CliniCARE-Bench: Clinical Calibrated Audit of Medical Reasoning in EHR

Large language models perform strongly on medical knowledge benchmarks, but reliable clinical deployment requires agents to conduct defensible investigations over heterogeneous, longitudinal records: determining what evidence is needed, retrieving and reconciling structured and free-text data, grounding conclusions in verifiable evidence, and deferring cases that cannot be resolved reliably. We introduce CliniCARE-Bench (Clinical Calibrated Audit of Medical Reasoning in EHR), a benchmark for retrospective clinical audit: 25 clinician-validated scenarios instantiated as 750 patient-specific cases over real-patient-derived MIMIC-IV data. Systems investigate each case through a governed, logged tool environment for record retrieval, computation, and policy access, and return one of four verdicts---Yes, No, Indeterminate: Lack of Data, or Indeterminate: Medically Ambiguous---the last two separating missing evidence from residual medical ambiguity. Beyond verdict accuracy, we score patient-evidence and policy grounding, process adherence, calibrated abstention, reliability, and efficiency against case-level reference verdicts produced by independent multi-model adjudication and calibrated against Clinical Board review. Every retrieval, computation, and report is replayable, so the investigation trace is inspectable and scorable. To our knowledge, CliniCARE-Bench is the first deployment-oriented clinical-agent benchmark to jointly evaluate real longitudinal EHR investigation, claim-level evidence grounding, governing-policy use, process adherence, and calibrated abstention within a common patient-level adjudication framework. Across 16 agentic systems, four-way accuracy spans 65.3-76.1%, but raw accuracy overstates investigation quality. Defect-free accuracy, which credits a verdict only when correct and free of prohibited shortcuts, is 4.8-14.8 points lower and reorders the leaderboard.

==> OLD_result.tex <==
\section{Experimental Results}
\label{sec:experiments}

We evaluate autonomous systems along two axes: a leaderboard of production agent harnesses, each
running its native frontier model, and a controlled comparison that fixes a single model-agnostic
harness and varies only the model. Using the metrics of Section~\ref{sec:eval_framework}, the
experiments target three dissociations the benchmark is built to expose. First, raw accuracy
overstates sound clinical reasoning, because a verdict can be reached through a prohibited shortcut.
Second, systems systematically under-abstain, committing to a definitive answer where the record
warrants deferral. Third, accuracy exceeds grounding fidelity, because models reach the right verdict
without citing the evidence that justifies it.

\subsection{Experimental Setup}
\label{sec:exp-setup}

\paragraph{Harnesses.} We run four agent harnesses. \texttt{Claude Code}, \texttt{Codex} and
\texttt{Gemini CLI} are production agent CLIs, each locked to its own vendor model family and driving
the benchmark tools through a native tool-calling loop, so they represent how each model is actually
deployed. \texttt{opencode} is a model-agnostic open-source harness that connects to the same MIMIC
tool server as the others. Because it can drive any model, it serves as the fixed neutral harness for
the model-comparison axis, isolating the model's contribution from the harness's. All four run with
web search and fetch disabled, so every system answers from the in-environment patient record and
policy corpus alone, a frozen-corpus condition enforced by a deny-by-default egress allowlist rather
than by instruction. MIMIC data is reached only through a credential-isolated tool server, so no
system can bypass the governed tools to read raw records.

\paragraph{Models.} Table~\ref{tab:exp-matrix} lists the sixteen systems evaluated. The native
leaderboard pairs each harness with its frontier models, and the model-comparison axis runs a set of
open-weight models on the neutral \texttt{opencode} harness, isolating the model from the harness.
Running the vendor models on \texttt{opencode} for a fully harness-controlled comparison is planned.
We exclude medical-specialized models from the agentic leaderboard because they cannot drive a
multi-step tool-calling loop and would score near zero from harness incompatibility rather than
clinical weakness. Where relevant we report them separately as a single-turn probe.

\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2}
\caption{\textbf{Systems evaluated in CliniCARE-Bench.} Native leaderboard (each harness on its own
frontier model) and the controlled model comparison on the neutral \texttt{opencode} harness.}
\label{tab:exp-matrix}
\begin{tabularx}{\linewidth}{@{}lX@{}}
\toprule
\textbf{Harness} & \textbf{Models} \\
\midrule
\multicolumn{2}{@{}l}{\textit{Native leaderboard: each harness on its own frontier model}} \\
\addlinespace[2pt]
\texttt{Claude Code} & Claude Opus 5, Claude Sonnet 5 \\
\texttt{Codex}       & GPT-5.6 Sol, GPT-5.6 Luna, GPT-5.5, GPT-5.4, GPT-5.4-mini \\
\texttt{Gemini CLI}  & Gemini 3.1 Pro, Gemini 3.5 Flash, Gemini 3.6 Flash \\
\addlinespace[6pt]
\midrule
\multicolumn{2}{@{}l}{\textit{Controlled comparison: open-weight models on one neutral harness}} \\
\addlinespace[2pt]
\texttt{opencode} & DeepSeek V4 Pro, DeepSeek V4 Flash, Qwen 3.7 Plus, GLM 5.2,
                    MiniMax M3, Kimi K2.7 Code \\
\bottomrule
\end{tabularx}
\end{table}

\paragraph{cases and verdict classes.} The cohort is 25 clinical scenarios $\times$ 30 patients
$=750$ cases, each a single adjudication question resolved to one of the four verdict classes defined
in Section~\ref{sec:eval_framework}: \textit{Yes}, \textit{No}, and the two deferral classes we
abbreviate \textit{lack} (\textit{Indeterminate: Lack of Data}) and \textit{amb} (\textit{Indeterminate:
Medically Ambiguous}). The verdict is scored deterministically by exact four-class match, with no
partial credit.

\paragraph{Metrics.} Four-class accuracy and macro-F1, the two directional abstention errors
(\emph{over-commitment} and \emph{over-abstention}), process adherence (LLM-judged, pinned to
\texttt{openai/gpt-5.5}), evidence and policy grounding, repeated-run reliability (avg@3,
pass\textasciicircum{}3, pass@3) and per-run cost all follow the definitions in
Section~\ref{sec:eval_framework}. Accuracy is reported per run (micro), which coincides with the
scenario-macro average on a complete arm but not on a partial one. Two quantities are specific to this
section and introduced where first used: \emph{trap-adjusted accuracy} with its \emph{trap gap}, which
credit a verdict only when no \textsc{must-not} rubric criterion was violated, and expected calibration
error (Eq.~\ref{eq:ece}).

\subsection{Results}
\label{sec:main-results}

Every system is run on all 750 cases at a single attempt against the silver reference labels.
Table~\ref{tab:main750} reports the full leaderboard: verdict accuracy and macro-F1, trap-adjusted
accuracy and the gap it opens, process adherence, the two directional abstention errors, calibration,
and per-run cost. Two points bear noting before reading it. The \emph{Gap} column is raw accuracy
minus trap-adjusted accuracy \emph{over report-present runs only}, so it is not the difference of
the two columns beside it. The cost columns are measured on two different instruments: harness-reported
for the vendor CLIs, but computed from measured tokens for the \texttt{opencode} arms, which report
neither a cost field nor a cached-token count. Those six are therefore given as ranges rather than
point estimates.

\begin{table}[htbp]
\centering
\caption{\textbf{Primary leaderboard on the complete 750-case cohort.} Single attempt against silver
labels, all sixteen arms on all 750 cases. \emph{Trap-adj} is trap-adjusted accuracy, \emph{Gap} the
trap gap (raw minus trap-adjusted over report-present runs), \emph{Over-com}$/$\emph{Over-abs} the
directional abstention errors, \emph{Proc\%} the LLM-judged process score, and \emph{ECE} expected
calibration error. Cost columns are per-run medians except USD$/$run (a mean, excluding judge
spend). \texttt{opencode} work-token and USD figures are ranges because that adapter reports no
cached-token count.}
\label{tab:main750}
\footnotesize
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{lcccccccccccc}
\toprule
 & \multicolumn{5}{c}{\textbf{Quality}} & \multicolumn{3}{c}{\textbf{Abstention \& calibration}} & \multicolumn{4}{c}{\textbf{Cost \& efficiency}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-9}\cmidrule(lr){10-13}
\textbf{Model} & \textbf{Acc} & \textbf{Mac-F1} & \textbf{Trap-adj} & \textbf{Gap} & \textbf{Proc\%} & \textbf{Over-com} & \textbf{Over-abs} & \textbf{ECE} & \textbf{Turns} & \textbf{Tools} & \textbf{Work-tok} & \textbf{USD/run} \\
\midrule
\multicolumn{13}{@{}l}{\texttt{Claude Code}}\\
\quad Opus 5 & 72.3 & 0.633 & 62.9 & 9.3 & 80.2 & 29.2 & 15.2 & 0.098 & 17 & 28 & 130.1k & 2.04 \\
\quad Sonnet 5 & 70.8 & 0.603 & 59.5 & 11.3 & 69.6 & 28.5 & 16.1 & 0.071 & 13 & 22 & 90.2k & 0.94 \\
\addlinespace
\multicolumn{13}{@{}l}{\texttt{Codex}}\\
\quad GPT-5.6-Sol      & 70.8 & 0.619 & 64.1 & 6.7 & 79.6 & 26.9 & 16.6 & 0.217 & 22 & 16 & 88.4k & 1.11 \\
\quad GPT-5.6-Luna     & 64.5 & 0.552 & 57.2 & 7.3 & 75.0 & 36.9 & 20.5 & 0.250 & 22 & 18 & 97.5k & 0.25 \\
\quad GPT-5.5 & 73.2 & 0.655 & 67.1 & 6.1 & 78.6 & 33.8 & 12.6 & 0.118 & 18 & 49 & 122.2k & 1.53 \\
\quad GPT-5.4          & 68.9 & 0.610 & 61.1 & 7.9 & 75.8 & 33.8 & 15.3 & 0.173 & 21 & 52 & 111.3k & 0.72 \\
\quad GPT-5.4-mini     & 64.7 & 0.535 & 54.3 & 10.4 & 66.8 & 50.8 & 16.1 & 0.231 & 24 & 44 & 84.1k & 0.20 \\
\addlinespace
\multicolumn{13}{@{}l}{\texttt{Gemini CLI}}\\
\quad Gemini-3.6-Flash & 70.5 & 0.608 & 56.4 & 14.1 & 72.3 & 35.4 & 11.6 & 0.274 & 62 & 36 & 385.0k & 1.13 \\
\quad Gemini-3.5-Flash & 70.0 & 0.590 & 57.6 & 12.4 & 72.0 & 38.5 & 11.8 & 0.279 & 62 & 36 & 387.8k & 1.16 \\
\quad Gemini-3.1-Pro   & 70.3 & 0.626 & 54.4 & 15.9 & 58.6 & 18.5 & 15.5 & 0.279 & 42 & 23 & 205.7k & 1.02 \\
\addlinespace
\multicolumn{13}{@{}l}{\texttt{opencode} \textnormal{(open-weight models on the neutral harness)}}\\
\quad DeepSeek-V4-Pro & 67.3 & 0.581 & 54.4 & 12.9 & 70.2 & 34.6 & 14.0 & 0.201 & 14 & 41 & 62--576k & 0.21--1.12 \\
\quad DeepSeek-V4-Flash & 69.1 & 0.554 & 57.5 & 11.6 & 68.9 & 49.2 & 11.5 & 0.230 & 15 & 46 & 77--729k & 0.03--0.12 \\
\quad GLM-5.2 & 72.1 & 0.614 & 60.9 & 11.2 & 75.5 & 37.7 & 11.3 & 0.143 & 14 & 32 & 66--611k & 0.24--1.13 \\
\quad Qwen-3.7-Plus & 62.4 & 0.522 & 50.1 & 12.3 & 65.0 & 40.8 & 19.4 & 0.209 & 11 & 28 & 47--435k & 0.06--0.19 \\
\quad MiniMax-M3 & 65.9 & 0.543 & 51.5 & 14.4 & 71.3 & 52.3 & 14.4 & 0.189 & 21 & 45 & 107--991k & 0.12--0.40 \\
\quad Kimi-K2.7-Code & 63.2 & 0.516 & 49.3 & 13.9 & 69.9 & 50.0 & 14.7 & 0.183 & 20 & 56 & 132--1261k & 0.97--3.36 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{No system resolves the cohort, and the loss concentrates in the rare classes.} Accuracy
spans 62.4 to 73.2 and macro-F1 0.516 to 0.655 (Table~\ref{tab:main750}): the strongest arm resolves
just under three-quarters of its graded cases and the weakest just over three-fifths. Macro-F1 trails
accuracy in every arm because it weights the two rare \textit{Indeterminate} classes equally with
\textit{Yes} and \textit{No}, so the loss concentrates where deferral must be recognised. Accuracy
forms a continuum rather than tiers, and the harness families interleave within it: no two adjacent
arms differ by more than 1.6 points across the whole eleven-point span, and two vendor arms
(GPT-5.6-Luna 64.5, GPT-5.4-mini 64.7) place below four of the open-weight models on the neutral
harness. The best open-weight arm, GLM-5.2 at 72.1, is indistinguishable from the best vendor arm
(GPT-5.5, 73.2) at this $n$, where one binomial standard error is about 1.6 points.

\paragraph{Trap-adjusted accuracy: what it is, and why it reorders the field.} A \emph{trap} is a
\textsc{must-not} criterion in the case's rubric, an inferential shortcut a clinician reviewing the
work would reject outright, such as reading acute kidney injury off a billing code, asserting contrast
causation from temporal proximity alone, or citing a policy document that does not exist.
\emph{Trap-adjusted accuracy} counts a run correct only when the verdict is right \emph{and} no
\textsc{must-not} criterion was violated, and the \emph{Gap} column is raw minus trap-adjusted accuracy
over report-present runs, so it is the share of an arm's correct verdicts reached by a forbidden
route. Every system pays between 6.1 and 15.9 points (Table~\ref{tab:main750}), meaning that between
one in twelve and one in four of its correct answers does not survive inspection of how it was
reached.

The spread is the finding, not the magnitude (\Cref{fig:trap}). Were raw accuracy merely optimistic by
a fixed margin, the gap would be roughly constant and the ranking would survive the correction. It
does not. GPT-5.5 loses 6.1 points while Gemini-3.1-Pro loses 15.9, so the correction reorders the
field. Gemini-3.1-Pro reaches 70.3 raw accuracy, within noise of the leading group, then falls to 54.4
trap-adjusted, below every Claude arm and every Codex arm bar GPT-5.4-mini, which it ties.
Gemini-3.1-Pro is also the arm \emph{least} prone to over-commitment (18.5\%), so springing traps and
over-committing are distinct failures rather than two faces of the same carelessness. This
operationalises, on real longitudinal records, the
reasoning-versus-pattern-matching gap documented for medical LLMs
\cite{bedi2025fidelity, natmed2026robustness}: a correct label is not evidence of correct reasoning,
and only a trace-level audit of the investigation distinguishes the two. It is the concrete payoff of
scoring the observable adjudication process rather than the final answer alone.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_trap_adjusted.pdf}
\caption{\textbf{Trap-adjusted accuracy reorders the leaderboard.} Raw accuracy (open circles) and
trap-adjusted accuracy (filled markers) for all sixteen arms, ordered by trap-adjusted accuracy;
marker colour denotes the harness family and connector length is the trap gap. Gemini-3.1-Pro falls
from within noise of the leaders to below every Claude and Codex arm bar GPT-5.4-mini once forbidden-route
answers are removed, while GPT-5.5 loses least.}
\label{fig:trap}
\end{figure}

\paragraph{Systems under-abstain: over-commitment exceeds over-abstention in every arm.} Measured
directionally (\Cref{fig:abstention}), over-commitment, returning a definitive verdict where the
reference verdict is \textit{Indeterminate}, runs 18.5--52.3\% against over-abstention of
11.3--20.5\%, and \emph{all sixteen} systems over-commit at the higher rate. That the asymmetry holds
arm by arm rather than only in aggregate makes it a property of the systems rather than of the label
distribution, and it reproduces on the development subset (Section~\ref{sec:ablations}). The failure
is not an unwillingness to answer but an unwillingness to decline. The magnitude, not the direction, is
what varies: three arms over-commit on at least half of all deferral cases (MiniMax-M3 52.3\%,
GPT-5.4-mini 50.8\%, Kimi-K2.7-Code 50.0\%) while Gemini-3.1-Pro does so on 18.5\%. Over-abstention, by
contrast, is tightly banded at 11.3--20.5\%, and its highest value belongs to a vendor arm
(GPT-5.6-Luna), so the deferral side of the error budget varies far less across systems than the
commitment side.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_underabstention.pdf}
\caption{\textbf{Every system under-abstains.} Directional abstention errors for all sixteen arms:
over-abstention (open circles) and over-commitment (filled markers), each over that arm's own gold
supports; marker colour denotes the harness family. Over-commitment exceeds over-abstention in every
arm. GPT-5.4-mini, MiniMax-M3 and Kimi-K2.7-Code over-commit on half of all deferral cases, whereas
Gemini-3.1-Pro is the only near-balanced arm.}
\label{fig:abstention}
\end{figure}

\paragraph{The process score measures something the verdict does not.} Process adherence
(Table~\ref{tab:main750}) is judged against the rubric's observable investigation steps rather than
against the answer, and it separates arms that accuracy places together. Opus 5 scores 80.2 on process
against 72.3 accuracy, whereas Gemini-3.1-Pro reaches 70.3 accuracy on a process score of 58.6, the
same verdict quality reached through a materially less defensible investigation. This is the trap gap
seen from the other side. The per-class picture (\Cref{fig:perclass}) tells the same story from the
verdict side: \textit{Yes} and \textit{No} F1 stay strong across the roster while both
\textit{Indeterminate} classes fall away, and precision on the deferral classes is low throughout
(\textit{lack} 31--49\%, \textit{amb} 25--67\%), so the deferrals systems do issue are frequently made
on records that in fact settle the question. For a clinical deliverable this matters more than the
headline: a reader can audit a documented investigation but not a bare verdict.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_perclass_f1.pdf}
\caption{\textbf{Performance collapses on the two safety-critical \textit{Indeterminate} classes.}
Per-class F1 for all sixteen arms on the complete cohort (rows in leaderboard order, grouped by
harness via the colour bar at left). \textit{Yes} and \textit{No} stay strong while both deferral
classes (dashed box) fall away on the weaker arms. Precision on the deferral classes is low throughout
(\textit{lack} 31--49\%, \textit{amb} 25--67\%).}
\label{fig:perclass}
\end{figure}

\paragraph{The leaderboard order does not hold scenario by scenario.} Resolved per scenario
(\Cref{fig:scenario}), the aggregate ordering of Table~\ref{tab:main750} survives in only 68.5\% of
the 3{,}000 arm-pair $\times$ scenario comparisons the grid contains, and fifteen of the sixteen arms
are the best system on at least one scenario, including Kimi-K2.7-Code, second from last on the
leaderboard, which leads on \texttt{he-precipitant} and \texttt{overdose-disposition}. The ordering of the averages is nevertheless stable: an arm's cohort accuracy predicts its mean per-scenario rank almost perfectly (Spearman $\rho=-0.95$, negative only because rank 1 is best). Even so, Opus 5, second on the leaderboard, sits in the
bottom quartile on one of the 25
scenarios. The leaderboard is
thus a statement about a case mix more than about which system to trust on a given clinical question.
Difficulty is concentrated rather than diffuse: cross-arm mean accuracy runs from 96.7 on
\texttt{discharge-audit} to 8.8 on \texttt{pe-workup}, the five hardest scenarios carry 36\% of all
errors against the 20\% that uniform difficulty implies, and one scenario has stopped separating
systems altogether. On \texttt{pe-workup} no arm exceeds 24\%, and the answers pooled over all sixteen
arms are overwhelmingly \textit{Indeterminate: Lack of Data} against a reference that reads
\textit{No} on most of its 30 cases. Sixteen independently built systems agreeing that a record is
insufficient is more readily explained by the reference labels for that scenario than by a shared
clinical blind spot, so \texttt{pe-workup} is queued for label adjudication. It is still counted in
every number reported here.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_scenario_accuracy.pdf}
\caption{\textbf{The leaderboard order does not hold scenario by scenario.} Verdict accuracy of every
arm on each of the 25 scenarios, one dot per arm coloured by harness family, with the cross-arm mean
(dark line). Scenarios are sorted by that mean.}
\label{fig:scenario}
\end{figure}

% \begin{table}[htbp]
% \centering
% \caption{\textbf{Per-class F1, with precision and recall for the two \textit{Indeterminate}
% classes.} The two rightmost cells read P\,$/$\,R. Denominators follow the cohort's natural label
% distribution, not the development subset's balanced one, so cells are not comparable with
% Table~\ref{tab:dev-perclass}.}
% \label{tab:main750-perclass}
% \small
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{lccccccc}
% \toprule
%  & & \multicolumn{4}{c}{\textbf{F1}} & \multicolumn{2}{c}{\textbf{Precision\,$/$\,Recall \%}} \\
% \cmidrule(lr){3-6}\cmidrule(lr){7-8}
% \textbf{Model (harness)} & \textbf{n} & Yes & No & lack & amb & lack & amb \\
% \midrule
% % <<<AUTOROWS750:tab:main750-perclass>>>
% Opus 5 (Claude Code)           & 750 & 0.818 & 0.738 & 0.506 & 0.473 & 41.2\,/\,65.3 & 50.0\,/\,44.8 \\
% Sonnet 5 (Claude Code) & 750 & 0.800 & 0.726 & 0.515 & 0.373 & 41.7\,/\,67.3 & 36.7\,/\,37.9 \\
% \addlinespace
% GPT-5.6-Sol (Codex)            & 750 & 0.795 & 0.734 & 0.515 & 0.433 & 41.3\,/\,68.3 & 41.9\,/\,44.8 \\
% GPT-5.6-Luna (Codex)           & 750 & 0.740 & 0.694 & 0.402 & 0.373 & 32.5\,/\,52.5 & 30.4\,/\,48.3 \\
% GPT-5.5 (Codex)                & 750 & 0.824 & 0.746 & 0.492 & 0.560 & 42.0\,/\,59.4 & 66.7\,/\,48.3 \\
% GPT-5.4 (Codex)                & 750 & 0.774 & 0.717 & 0.466 & 0.483 & 38.8\,/\,58.4 & 48.3\,/\,48.3 \\
% GPT-5.4-mini (Codex)           & 750 & 0.770 & 0.657 & 0.351 & 0.364 & 31.5\,/\,39.6 & 32.4\,/\,41.4 \\
% \addlinespace
% Gemini-3.6-Flash (Gemini CLI)  & 750 & 0.804 & 0.695 & 0.504 & 0.429 & 45.0\,/\,57.4 & 44.4\,/\,41.4 \\
% Gemini-3.5-Flash (Gemini CLI)  & 750 & 0.794 & 0.703 & 0.487 & 0.377 & 43.4\,/\,55.4 & 41.7\,/\,34.5 \\
% Gemini-3.1-Pro (Gemini CLI)    & 750 & 0.775 & 0.716 & 0.556 & 0.458 & 43.2\,/\,78.2 & 57.9\,/\,37.9 \\
% \addlinespace
% DeepSeek-V4-Pro (opencode) & 750 & 0.769 & 0.686 & 0.463 & 0.407 & 39.7\,/\,55.4 & 40.0\,/\,41.4 \\
% DeepSeek-V4-Flash (opencode) & 750 & 0.809 & 0.688 & 0.411 & 0.308 & 38.9\,/\,43.6 & 34.8\,/\,27.6 \\
% GLM-5.2 (opencode) & 750 & 0.808 & 0.732 & 0.519 & 0.400 & 48.7\,/\,55.4 & 36.1\,/\,44.8 \\
% Qwen-3.7-Plus (opencode) & 750 & 0.734 & 0.656 & 0.371 & 0.329 & 31.3\,/\,45.5 & 26.0\,/\,44.8 \\
% MiniMax-M3 (opencode) & 750 & 0.767 & 0.678 & 0.362 & 0.366 & 34.9\,/\,37.6 & 31.0\,/\,44.8 \\
% Kimi-K2.7-Code (opencode) & 750 & 0.734 & 0.664 & 0.356 & 0.308 & 34.6\,/\,36.6 & 24.5\,/\,41.4 \\
% % <<<END750:tab:main750-perclass>>>
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[htbp]
% \centering
% \caption{\textbf{Verdict accuracy (\%) per scenario, all 16 arms.} Rows are the 25 clinical
% scenarios, sorted by the unweighted mean over arms given in the last column; the best cell in each row
% is bold. A cell's denominator is that arm's graded runs for that scenario, exactly 30 for every
% cell in the grid, so a single cell is a weaker estimate than a row or a column.
% Column key: O5\,=\,Opus 5, S5\,=\,Sonnet 5, Sol\,=\,GPT-5.6-Sol, Luna\,=\,GPT-5.6-Luna, 5.5\,=\,GPT-5.5, 5.4\,=\,GPT-5.4, 5.4m\,=\,GPT-5.4-mini, G3.6\,=\,Gemini-3.6-Flash, G3.5\,=\,Gemini-3.5-Flash, G3.1\,=\,Gemini-3.1-Pro, D4P\,=\,DeepSeek-V4-Pro, D4F\,=\,DeepSeek-V4-Flash, GLM\,=\,GLM-5.2, Qwn\,=\,Qwen-3.7-Plus, MM3\,=\,MiniMax-M3, K2.7\,=\,Kimi-K2.7-Code.}
% \label{tab:scenario-table}
% \small
% \setlength{\tabcolsep}{3pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccccccccccccc}
% \toprule
% \textbf{Scenario} & \textbf{O5} & \textbf{S5} & \textbf{Sol} & \textbf{Luna} & \textbf{5.5} & \textbf{5.4} & \textbf{5.4m} & \textbf{G3.6} & \textbf{G3.5} & \textbf{G3.1} & \textbf{D4P} & \textbf{D4F} & \textbf{GLM} & \textbf{Qwn} & \textbf{MM3} & \textbf{K2.7} & \textbf{Mean} \\
% \midrule
% % <<<SCENROWS:tab:scenario-table>>>
% discharge-audit          & 97 & \textbf{100} & \textbf{100} & 97 & \textbf{100} & \textbf{100} & \textbf{100} & 93 & 97 & 90 & 97 & 90 & \textbf{100} & 90 & \textbf{100} & 97 & 96.7 \\
% eol-goal-concordance     & 93 & 93 & \textbf{100} & 97 & 93 & 97 & 93 & 90 & 90 & \textbf{100} & 77 & 93 & 90 & 83 & 87 & 90 & 91.7 \\
% overdose-disposition     & 87 & \textbf{97} & 87 & 83 & 90 & 90 & \textbf{97} & \textbf{97} & \textbf{97} & 90 & 93 & \textbf{97} & 90 & 80 & 80 & \textbf{97} & 90.6 \\
% renal-trajectory         & 87 & 93 & 90 & 90 & 93 & 90 & \textbf{97} & 83 & 93 & 90 & 90 & 83 & 83 & 87 & 90 & 83 & 89.0 \\
% transfusion-audit        & 87 & \textbf{90} & 87 & 83 & \textbf{90} & \textbf{90} & 87 & \textbf{90} & \textbf{90} & \textbf{90} & 87 & \textbf{90} & \textbf{90} & 83 & \textbf{90} & 83 & 87.9 \\
% advanced-imaging         & 83 & 87 & 87 & \textbf{90} & 83 & 77 & 67 & 87 & 87 & 77 & 80 & 73 & 87 & 77 & 73 & 77 & 80.6 \\
% hfref-gdmt               & 80 & \textbf{87} & 83 & 63 & 83 & 73 & 70 & 83 & 83 & 77 & 77 & 73 & 80 & 73 & 70 & 70 & 76.7 \\
% post-ct-aki              & 83 & 83 & 90 & \textbf{93} & 90 & 73 & 80 & 73 & 77 & 73 & 60 & 77 & 67 & 60 & 80 & 67 & 76.7 \\
% readmission-30d          & 70 & 73 & 80 & 87 & 87 & 83 & 70 & 83 & 77 & \textbf{90} & 73 & 67 & 77 & 70 & 67 & 63 & 76.0 \\
% goals-of-care            & 93 & 90 & 90 & 60 & 87 & 83 & 57 & 67 & 70 & \textbf{97} & 83 & 77 & 83 & 63 & 57 & 53 & 75.6 \\
% frequent-admitter        & 77 & 70 & 83 & 77 & 77 & 63 & 63 & \textbf{87} & 77 & 83 & 67 & 73 & 83 & 77 & 63 & 67 & 74.2 \\
% icu-delirium             & 67 & \textbf{83} & 60 & 63 & 63 & 67 & 67 & 77 & 73 & 63 & 60 & 60 & 77 & 67 & 63 & 80 & 68.1 \\
% med-reconciliation       & \textbf{87} & 70 & 73 & 57 & 60 & 60 & 53 & 60 & 70 & 83 & 73 & 53 & 83 & 57 & 57 & 60 & 66.0 \\
% sepsis-source-abx        & 77 & 60 & 63 & 43 & 70 & 67 & 73 & \textbf{80} & 67 & 73 & 57 & 77 & 77 & 57 & 67 & 47 & 65.8 \\
% postop-complications     & 53 & 60 & 57 & 63 & 70 & 67 & 67 & 70 & 67 & 67 & 70 & \textbf{77} & 63 & 63 & 67 & 67 & 65.4 \\
% ams-workup               & 73 & 60 & 77 & 70 & 70 & 67 & 37 & 67 & 60 & 57 & \textbf{83} & 57 & 67 & 60 & 60 & 63 & 64.2 \\
% dka-resolution           & 83 & 57 & 87 & 60 & \textbf{90} & 77 & 23 & 73 & 67 & 60 & 53 & 47 & 70 & 43 & 53 & 63 & 62.9 \\
% hyperkalemia-management  & 60 & 57 & 63 & 60 & 70 & 70 & 67 & 47 & 53 & 53 & 67 & 60 & \textbf{80} & 63 & 63 & 67 & 62.5 \\
% empiric-abx              & 70 & \textbf{73} & 63 & 57 & 70 & 63 & 63 & 63 & 63 & 67 & 63 & 60 & 67 & 50 & 40 & 43 & 61.0 \\
% he-precipitant           & 57 & 53 & 60 & 57 & 60 & 57 & 67 & 67 & 63 & 63 & 60 & 67 & 63 & 57 & 53 & \textbf{73} & 61.0 \\
% stroke-time-targets      & 67 & 57 & 53 & 50 & 63 & 57 & 53 & 70 & \textbf{73} & 53 & 63 & 67 & 57 & 53 & 67 & 60 & 60.2 \\
% anticoag-reversal        & 67 & 70 & 60 & 40 & 60 & 57 & 47 & 67 & 70 & 57 & 53 & \textbf{80} & 50 & 57 & 63 & 40 & 58.5 \\
% pneumonia-curb65         & 60 & 57 & 33 & 30 & 67 & 47 & 70 & 43 & 47 & 40 & 40 & 57 & 47 & 43 & \textbf{73} & 30 & 49.0 \\
% sepsis-bundle            & 40 & 43 & 37 & 37 & 33 & 40 & 43 & 43 & 37 & \textbf{53} & 50 & 50 & 50 & 43 & \textbf{53} & 40 & 43.3 \\
% pe-workup                & 10 & 7 & 7 & 7 & 10 & 10 & 7 & 3 & 3 & 10 & 7 & \textbf{23} & \textbf{23} & 3 & 10 & 0 & 8.8 \\
% <<<SCENEND:tab:scenario-table>>>
% \bottomrule
% \end{tabular}%
% }
% \end{table}

\paragraph{Calibration separates the systems more cleanly than accuracy does.} Every report states a
confidence, so we can ask whether that number carries information. Expected calibration error is the
bin-weighted deviation between stated confidence and realised accuracy,
\begin{equation}
\mathrm{ECE} \;=\; \sum_{b=1}^{B} \frac{|B_b|}{n}\,\bigl|\,\mathrm{conf}(B_b) - \mathrm{acc}(B_b)\,\bigr| ,
\label{eq:ece}
\end{equation}
over $B=10$ equal-width bins of stated confidence, where $\mathrm{conf}(B_b)$ and $\mathrm{acc}(B_b)$
are the mean stated confidence and realised accuracy in bin $b$. ECE spans 0.071--0.279 across the
sixteen arms, a near-fourfold range on an axis accuracy cannot see, and it does \emph{not} order them
the way accuracy does: the three best-calibrated are Sonnet 5 (0.071), Opus 5 (0.098) and GPT-5.5
(0.118), while the three worst are all Gemini CLI arms (0.274--0.279), which sit mid-field on accuracy.
For a report addressed to a clinician who cannot cheaply re-derive the answer, a confidence that does
not track correctness is arguably a more consequential defect than a few points of accuracy, and no
aggregate score above reveals it. One caveat on cross-arm comparison: an arm emitting few distinct
confidence values populates few bins, so its ECE is not measuring quite the same thing.

\paragraph{Cost and efficiency diverge from accuracy, and from each other.} Across the vendor arms a
tenfold spread in price buys only an $\sim$9-point accuracy band (\Cref{fig:cost}). GPT-5.4-mini and
GPT-5.6-Luna land within 0.2 points of each other on accuracy and cost \$0.20 and \$0.25 per run, so
every per-dollar ratio favours the cheaper one. What the extra spend buys is not correct verdicts but
cleaner ones, 2.9 more points of trap-adjusted accuracy and 8.1 more of process adherence, a purchase
worth making in this domain and invisible to any cost-per-accuracy-point ratio, which is why we do not
tabulate one. Composition differs more than total: GPT-5.4-mini issues a median 44 typed tool calls
against GPT-5.6-Luna's 18, roughly $2.4\times$ the retrieval traffic, while consuming \emph{fewer}
work-tokens (84.1k against 97.5k). The cheaper arm queries more and reasons less over what it
retrieves, and it is also the arm with the wider trap gap and the lower process score: more retrieval
does not substitute for sound adjudication of what was retrieved. Work-tokens are comparable only
within a serving path, and the \texttt{opencode} figures are ranges rather than point values because
that path reports no cached-token count and the cache correction has to be estimated.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_cost_accuracy.pdf}
\caption{\textbf{Accuracy rises only weakly with cost.} Per-run cost (USD, log scale,
harness-reported) against verdict accuracy for the ten vendor arms, coloured by harness family, with
$\pm1$ binomial standard error bars at $n=750$. The six \texttt{opencode} arms are omitted because
their per-run cost is a range rather than a point.}
\label{fig:cost}
\end{figure}

\subsection{Patient-Evidence Grounding}
\label{sec:grounding-results}

Grounding is where verdict accuracy and defensible reasoning most clearly diverge: a system can reach
the correct verdict without citing the evidence that justifies it. Table~\ref{tab:grounding-v3-full750}
reports the four patient-evidence grounding metrics of Section~\ref{sec:patient-grounding} for all sixteen
model--harness combinations over the same 750 cases. Two score \emph{citation precision}:
$P_{\mathrm{record}}$, the fraction of record identifiers cited in the report that occur in the
evidence the agent actually retrieved, and $P_{\mathrm{claim}}$, the fraction of the report's atomic
clinical claims judged \emph{supported} --- rather than \emph{contradicted} or \emph{unverifiable}
--- against their cited evidence, with correct patient, encounter, and temporal attribution required.
Two score \emph{evidence coverage}: $R_{\mathrm{retrieval}}$, the fraction of the case's
expert-specified record sources the agent queried, and $C_{\mathrm{finding}}$, the fraction of its
required-evidence categories the report establishes. All four are computed against the agent's own
investigation rather than against the reference verdict, so they capture whether a determination is
auditable, not whether it is correct. All four are stable under repetition: $P_{\mathrm{record}}$ and
$R_{\mathrm{retrieval}}$ are rule-based and return the same value on every computation, and both
$P_{\mathrm{claim}}$ and $C_{\mathrm{finding}}$ reproduce reliably when the same reports are regraded (Section~\ref{sec:validation}).


\begin{table}[htbp]
\centering
\caption{\textbf{Patient-evidence grounding on the complete 750-case cohort.} Citation precision at
the record-identifier and clinical-claim levels against coverage at the retrieval and reporting
stages, as defined in Section~\ref{sec:patient-grounding}. Columns are averaged over each system's
scoreable runs, those in which the agent both produced a report and retrieved at least one record.}
\label{tab:grounding-v3-full750}
\footnotesize
\setlength{\tabcolsep}{8pt}
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{\textbf{Citation precision}} & \multicolumn{2}{c}{\textbf{Evidence coverage}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\textbf{Model} & $P_{\mathrm{record}}$ & $P_{\mathrm{claim}}$ & $R_{\mathrm{retrieval}}$ & $C_{\mathrm{finding}}$ \\
\midrule
\multicolumn{5}{@{}l}{\texttt{Claude Code}}\\
\quad Opus 5           & 0.983 & 0.882 & 0.848 & 0.819 \\
\quad Sonnet 5         & 0.986 & 0.867 & 0.816 & 0.719 \\
\addlinespace
\multicolumn{5}{@{}l}{\texttt{Codex}}\\
\quad GPT-5.6-Sol      & 1.000 & 0.971 & 0.846 & 0.751 \\
\quad GPT-5.6-Luna     & 1.000 & 0.968 & 0.866 & 0.725 \\
\quad GPT-5.5          & 0.999 & 0.964 & 0.874 & 0.749 \\
\quad GPT-5.4          & 0.999 & 0.961 & 0.859 & 0.729 \\
\quad GPT-5.4-mini     & 0.997 & 0.964 & 0.812 & 0.667 \\
\addlinespace
\multicolumn{5}{@{}l}{\texttt{Gemini CLI}}\\
\quad Gemini-3.6-Flash & 0.995 & 0.897 & 0.856 & 0.786 \\
\quad Gemini-3.5-Flash & 0.995 & 0.892 & 0.858 & 0.785 \\
\quad Gemini-3.1-Pro   & 0.999 & 0.906 & 0.683 & 0.589 \\
\addlinespace
\multicolumn{5}{@{}l}{\texttt{opencode} \textnormal{(open-weight models on the neutral harness)}}\\
\quad DeepSeek-V4-Pro & 0.996 & 0.910 & 0.853 & 0.736 \\
\quad DeepSeek-V4-Flash & 0.991 & 0.913 & 0.865 & 0.733 \\
\quad GLM-5.2 & 0.989 & 0.919 & 0.815 & 0.745 \\
\quad Qwen-3.7-Plus & 0.991 & 0.923 & 0.797 & 0.690 \\
\quad MiniMax-M3 & 0.986 & 0.910 & 0.827 & 0.743 \\
\quad Kimi-K2.7-Code & 0.993 & 0.932 & 0.860 & 0.729 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Record-identifier precision saturates and does not separate the systems.}
$P_{\mathrm{record}}$ spans 0.983--1.000 across the systems. No system fabricates record identifiers
at a rate this check resolves, so the column establishes a lower bound on citation validity rather
than discriminating between systems. 

\paragraph{Claim-level precision tracks the harness, not model capability.} $P_{\mathrm{claim}}$
separates along harness families --- Codex 0.966, \texttt{opencode} 0.918, Gemini CLI 0.898, Claude
Code 0.875 --- yet is nearly flat within each. Substituting one model for another under a fixed
harness barely moves it: the five Codex systems agree to within 0.010 despite spanning that vendor's
mini-to-frontier range, and the six unrelated open-weight models on \texttt{opencode} agree to within
0.022. Across the sixteen systems the $P_{\mathrm{claim}}$ ranking shows no positive association with
the verdict-accuracy ranking of Table~\ref{tab:main750} (Spearman $\rho=-0.29$). This is the mirror
image of the harness ablation (Table~\ref{tab:ablation-harness}), where varying the harness at a fixed
model left verdict accuracy inside noise: whether a determination is traceable to retrieved evidence
is set largely by the scaffold that structures retrieval and report generation, whereas whether it is
correct is set by the model. 

\paragraph{Citation precision and evidence coverage are weakly opposed.} Across the sixteen systems,
$P_{\mathrm{claim}}$ correlates negatively with $C_{\mathrm{finding}}$ ($r=-0.20$) and only weakly
with $R_{\mathrm{retrieval}}$ ($r=+0.23$), while the two coverage metrics correlate strongly with each
other ($r=+0.80$). Both extremes occur within a single family: Claude Code records the lowest
family-level $P_{\mathrm{claim}}$ (0.875) together with the highest $C_{\mathrm{finding}}$ (0.769),
and Opus 5 attains the highest coverage of any system (0.819). The inverse configuration also occurs,
GPT-5.4-mini ranking third on precision and second-lowest on coverage (0.667). The claim classifications
indicate the mechanism: ungrounded claims are predominantly \emph{unverifiable} rather than
\emph{contradicted}, at ratios between 2.6:1 for Gemini CLI and 5.1:1 for Claude Code. Systems that
report more of the required evidence are therefore not misreading the record but exceeding what their
retrieved evidence supports. Under-substantiation rather than contradiction is the dominant grounding
failure across all sixteen systems, which motivates reporting the two axes separately
(Section~\ref{sec:patient-grounding}): a single averaged grounding score would assign the same value
to a report that is faithful but incomplete and to one that is complete but inadequately sourced,
and the two are not equivalent to a reviewer auditing the determination.

\subsection{Policy Grounding}
\label{sec:policy-results}

Policy grounding is scored separately from patient-evidence grounding
(Section~\ref{sec:policy-grounding-metrics}): whether the agent cites the governing guidance correctly
and whether it applies the passages a domain expert would consider controlling. We report
two axes plus the effect of corpus access itself (Tables~\ref{tab:main750-policy}
and~\ref{tab:ablation-policy}). Policy citation correctness combines a deterministic existence check
(the citation resolves to a real corpus document and line span) with an LLM-judged support check, and
policy relevance is an LLM-judged score against an expert-specified governing-document set. Comparing
the policy-on and policy-off conditions isolates whether corpus access changes verdicts, evidence that
a decision is documentary rather than parametric recall.

\paragraph{Systems cite the governing policy correctly but incompletely.} Policy grounding on the
cohort (Table~\ref{tab:main750-policy}) separates two failure modes a single grounding score
would merge. Take GPT-5.4-mini and GPT-5.6-Luna, two arms complete at 750 and within 0.2 accuracy
points of each other. Citations almost always resolve (0.991 and 1.000), and precision of the cited
document set against the clinical board's governing list is high (0.800 and 0.825). Recall of that
set is roughly half (0.483 and 0.522): systems cite documents that genuinely govern, then omit about
half of the others that also govern. Since a determination resting on part of the applicable standard
can be right for the wrong reason, this is the policy-axis analogue of the trap gap, and a combined
score would hide it because high precision offsets low recall. That failure shape is the one finding
here that reproduces across all sixteen arms, because these are rates rather than counts and each is
computed within an arm: resolution runs 0.953--1.000 and document precision 0.757--0.907, while
document recall never exceeds 0.682 and falls as low as 0.410. Every system in the roster cites real,
relevant policy and omits much of the rest.

\paragraph{Fabricated citations dissociate sharply between systems of equal accuracy.} The same two
arms emit 27 and 2 fabricated policy citations, references resolving to no corpus document, a
thirteen-fold difference between systems scoring identically on accuracy. Citation support, the
LLM-judged check that a cited passage entails the claim attached to it, moves the same way (0.643
against 0.817). With the trap gap and the confidence margins, this is the third axis on which these
two arms are clearly distinguishable while their headline accuracy is not, and it is the one a
clinician auditing the report would notice first.

\begin{table}[htbp]
\centering
\caption{\textbf{Policy grounding on the complete 750-case cohort.} Resolution deterministically checks
that a citation names a real corpus document and valid line span, Support is LLM-judged, and
Doc-P$/$R$/$F1 compare the cited document set against the expert-specified governing set. Columns are
averaged over each arm's policy-expected runs (Resolution and Support only over runs with at least
one citation). Fabricated citations are counted separately.}
\label{tab:main750-policy}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{Resolve} & \textbf{Support} & \textbf{Doc-P} & \textbf{Doc-R} & \textbf{Doc-F1} \\
\midrule
\multicolumn{6}{@{}l}{\texttt{Claude Code}}\\
\quad Opus 5           & 0.999 & 0.571 & 0.757 & 0.682 & 0.695 \\
\quad Sonnet 5 & 0.992 & 0.591 & 0.834 & 0.453 & 0.613 \\
\addlinespace
\multicolumn{6}{@{}l}{\texttt{Codex}}\\
\quad GPT-5.6-Sol      & 1.000 & 0.753 & 0.827 & 0.589 & 0.653 \\
\quad GPT-5.6-Luna     & 1.000 & 0.817 & 0.825 & 0.522 & 0.609 \\
\quad GPT-5.5          & 1.000 & 0.750 & 0.791 & 0.592 & 0.648 \\
\quad GPT-5.4          & 1.000 & 0.631 & 0.767 & 0.548 & 0.616 \\
\quad GPT-5.4-mini     & 0.991 & 0.643 & 0.800 & 0.483 & 0.605 \\
\addlinespace
\multicolumn{6}{@{}l}{\texttt{Gemini CLI}}\\
\quad Gemini-3.6-Flash & 0.988 & 0.469 & 0.770 & 0.629 & 0.664 \\
\quad Gemini-3.5-Flash & 0.987 & 0.457 & 0.765 & 0.624 & 0.659 \\
\quad Gemini-3.1-Pro   & 1.000 & 0.666 & 0.784 & 0.410 & 0.550 \\
\addlinespace
\multicolumn{6}{@{}l}{\texttt{opencode} \textnormal{(open-weight models on the neutral harness)}}\\
\quad DeepSeek-V4-Pro & 0.995 & 0.622 & 0.866 & 0.520 & 0.662 \\
\quad DeepSeek-V4-Flash & 0.953 & 0.578 & 0.851 & 0.455 & 0.627 \\
\quad GLM-5.2 & 0.986 & 0.596 & 0.825 & 0.580 & 0.652 \\
\quad Qwen-3.7-Plus & 0.997 & 0.567 & 0.907 & 0.445 & 0.678 \\
\quad MiniMax-M3 & 0.978 & 0.468 & 0.818 & 0.535 & 0.640 \\
\quad Kimi-K2.7-Code & 0.998 & 0.619 & 0.824 & 0.538 & 0.644 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Ablations}
\label{sec:ablations}
The ablations run on the 142-case \emph{development subset} defined in Section~\ref{sec:eval_framework}. All sixteen arms are closed there at $n=142$, which is
what makes per-pair significance and repeated runs possible: of the $\binom{16}{2}=120$ pairs, 58 reach
$p<0.05$ under a two-sided exact McNemar test and 21 survive Holm correction, and accuracy spans
47.2--71.1 with a genuine three-way tie at the top. Every comparison below is paired against the
subset's own baseline and never against Table~\ref{tab:main750}, because the subset over-samples the
two rare \textit{Indeterminate} classes and its Claude arm is Opus 4.8 rather than the cohort's Opus 5,
so absolute scores do not carry across. GPT-5.6-Luna, for instance, reads 56.3 here against 64.5 on the
cohort. At a support of 12, one \textit{amb} case moves that column by 8.3 points, so \textit{amb}
figures indicate a direction and never a ranking. The abstention asymmetry of
Section~\ref{sec:main-results} reproduces here on a deliberately different label distribution, with
over-commitment exceeding over-abstention in \emph{all sixteen} arms (23.4--48.9\% against
5.3--29.5\%), which is what makes it a property of the systems rather than of the cohort's label mix.
Full sixteen-arm scores on the subset appear in Appendix~\ref{app:dev-leaderboard}, together with the
per-pair tests and per-class breakdowns.

\paragraph{Withholding the policy corpus degrades deferral, not verdict-reaching.} With the corpus
withheld and nothing else changed, accuracy moves \emph{inconsistently}: three of five arms fall by
3.5--4.3 points and two rise by 0.7--4.2, and a two-sided exact McNemar test on the paired cases
separates \emph{no} arm's shift from zero ($p=0.26$--$1.00$). Corpus access is therefore not worth a
fixed number of points, and these deltas do not order the arms. Recall on \textit{amb} moves
consistently on four of the five, falling on three and unchanged on one, which is what one expects if
the corpus is what tells an agent a governing standard exists and does not settle the case. The
policy-enabled condition remains canonical. This is an ablation of the environment, not an alternative
configuration (Table~\ref{tab:ablation-policy}).

\begin{table}[htbp]
\centering
\caption{\textbf{Policy-corpus ablation.} \emph{Paired per case, web search disabled in both
conditions.} $\Delta$ is off $-$ on, so negative means withholding the corpus hurt. $p$ is a two-sided
exact McNemar test on the accuracy $\Delta$ over the paired cases (discordant counts 13--26 per arm,
too small for the $\chi^2$ approximation), and no arm's accuracy $\Delta$ is distinguishable from zero
($p=0.26$--$1.00$), so the deltas do not order the arms. \textit{amb} recall is against a support of
12, so one case is 8.3 points: read direction, not magnitude. The policy-off side is complete at 142 on
all five arms. Gemini-3.1-Pro carries 3 policy-on stub runs (no deliverable, no grade) dropped from
both sides, so its row is paired over 139 cases and every other over 142.}
\label{tab:ablation-policy}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{Accuracy}} & \multicolumn{3}{c}{\textbf{Recall \textit{amb} \%}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-8}
\textbf{Model (harness)} & on & off & $\Delta$ & $p$ & on & off & $\Delta$ \\
\midrule
GPT-5.6-Sol (Codex)         & 71.1 & 71.8 & $+0.7$ & 1.00 & 50.0 & 41.7 & $-8.3$ \\
GPT-5.5 (Codex)             & 71.1 & 66.9 & $-4.2$ & 0.26 & 50.0 & 41.7 & $-8.3$ \\
Gemini-3.1-Pro (Gemini CLI) & 72.7 & 68.3 & $-4.3$ & 0.33 & 33.3 & 41.7 & $+8.3$ \\
GPT-5.6-Luna (Codex)        & 56.3 & 60.6 & $+4.2$ & 0.29 & 58.3 & 50.0 & $-8.3$ \\
Opus 4.8 (Claude Code)      & 69.7 & 66.2 & $-3.5$ & 0.36 & 50.0 & 50.0 & $\pm0.0$ \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Single-attempt accuracy overstates consistent correctness, and the inconsistency is
systematic.} Across three independent attempts, pass\textasciicircum{}3 falls 8.2--12.7 points below
avg@3, and the residual agreement is on the \emph{same wrong} verdict, 16.9--26.8 points, and for
GPT-5.6-Luna 37\% of the cases on which it agreed with itself. Run-to-run variation is small next to
that shortfall, with the standard deviation of accuracy across the three attempts at 1.1--3.2 points,
so the gap is not attempt noise. High self-consistency is therefore not evidence of reliability: these
systems are mostly \emph{stably} wrong rather than randomly wrong, so repeating a query will not
surface the error. Reliability is also worst exactly where the benchmark is hardest, as \emph{every}
arm's lowest pass\textasciicircum{}3 falls on an \textit{Indeterminate} class
(Table~\ref{tab:passk-perclass}).

\begin{table}[htbp]
\centering
\caption{\textbf{Repeated-run reliability, development subset.} \emph{Three independent attempts.}
$n_{\mathrm{com}}$ counts cases gradeable in \emph{every} attempt, since pass\textasciicircum{}3 is
undefined otherwise, and all five arms cover the full subset. \emph{SD} is the sample standard
deviation (2 degrees of freedom) of the three per-attempt accuracies. \emph{Spread} is
pass@3 $-$ pass\textasciicircum{}3, the share of cases correct in some attempts but not others.
\emph{Overst.} is avg@3 $-$ pass\textasciicircum{}3. \emph{Agree} is the share on which all three
attempts returned the same verdict, and \emph{Agree-wr} the part of that on an \emph{incorrect}
verdict, so \textit{Agree} $=$ pass\textasciicircum{}3 $+$ \textit{Agree-wr} by construction (printed
values can differ by $0.1$ from independent rounding). pass\textasciicircum{}3 and pass@3 are
set-valued over the intersection and have no across-attempt SD, and their binomial standard error at
$n=142$ (4.1--4.2 and 3.3--3.9 points) is comparable to the range of \emph{Overst.}, so the columns
support the aggregate claim rather than an ordering of arms. avg@3 is not comparable with the Acc
column of Table~\ref{tab:dev-leaderboard} because the denominators differ. The eleven single-attempt
arms are omitted.}
\label{tab:passk}
\small
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lcccccccrr}
\toprule
\textbf{Model (harness)} & $n_{\mathrm{com}}$ & \textbf{avg@3} & \textbf{SD} & \textbf{pass\textasciicircum{}3} & \textbf{pass@3} & \textbf{Spread} & \textbf{Overst.} & \textbf{Agree} & \textbf{Agree-wr} \\
\midrule
Opus 4.8 (Claude Code)         & 142 & \textbf{70.9} & 1.5 & \textbf{62.0} & 79.6 & 17.6 & \phantom{0}8.9 & \textbf{79.6} & 17.6 \\
\addlinespace
GPT-5.5 (Codex)                & 142 & 70.2 & 1.1 & \textbf{62.0} & 78.2 & \textbf{16.2} & \textbf{\phantom{0}8.2} & \textbf{79.6} & 17.6 \\
GPT-5.6-Sol (Codex)            & 142 & 68.3 & 3.2 & 57.0 & 78.2 & 21.1 & 11.3 & 76.8 & 19.7 \\
GPT-5.6-Luna (Codex)           & 142 & 57.7 & 1.9 & 46.5 & 66.9 & 20.4 & 11.3 & 73.2 & 26.8 \\
\addlinespace
Gemini-3.1-Pro (Gemini CLI)    & 142 & 69.7 & 2.4 & 57.0 & \textbf{81.0} & 23.9 & 12.7 & 73.9 & 16.9 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Per-class repeated-run reliability.} \emph{Development subset, three attempts.}
pass\textasciicircum{}3 is the share of a class's cases correct in \emph{all three} attempts, pass@3
the share correct in \emph{at least one}, and $n$ is the per-class count gradeable in all three, so the
four supports sum to the arm's $n_{\mathrm{com}}$ in Table~\ref{tab:passk}. \emph{SD} is the sample
standard deviation of that class's accuracy across the three attempts (2 degrees of freedom), not of
pass\textasciicircum{}3 or pass@3, which are set-valued. \textbf{The \textsc{amb} support is 12 cases,
where one case moves a cell by 8.3 points, so that column indicates a direction and must not be read as
a ranking.} The per-case binomial standard error is about 6.9 points at $n=50$, 7.3 at $n=45$, 8.3 at
$n=35$ and 14.1 at $n=12$, so no single cell separates arms. All five arms cover the full subset
(\textsc{yes} 50, \textsc{no} 45, \textsc{lack} 35, \textsc{amb} 12).}
\label{tab:passk-perclass}
\begin{tabular}{lcccccccccccccccc}
\toprule
& \multicolumn{4}{c}{\textsc{yes}} & \multicolumn{4}{c}{\textsc{no}}
& \multicolumn{4}{c}{\textsc{lack}} & \multicolumn{4}{c}{\textsc{amb}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
\textbf{Model (harness)} & $n$ & \^{}3 & @3 & SD & $n$ & \^{}3 & @3 & SD & $n$ & \^{}3 & @3 & SD & $n$ & \^{}3 & @3 & SD \\
\midrule
Opus 4.8 (Claude Code)       & 50 & \textbf{74.0} & \textbf{94.0} & 1.2 & 45 & 57.8 & \textbf{82.2} & 3.4 & 35 & 54.3 & 60.0 & 0.0 & 12 & \textbf{50.0} & \textbf{66.7} & 4.8 \\
\addlinespace
GPT-5.5 (Codex)              & 50 & 64.0 & 86.0 & 2.0 & 45 & \textbf{71.1} & 80.0 & 2.6 & 35 & 54.3 & 74.3 & 1.6 & 12 & 41.7 & 50.0 & 4.8 \\
GPT-5.6-Sol (Codex)          & 50 & 62.0 & 84.0 & 3.5 & 45 & 60.0 & \textbf{82.2} & 6.7 & 35 & 51.4 & 74.3 & 1.6 & 12 & 41.7 & 50.0 & 4.8 \\
GPT-5.6-Luna (Codex)         & 50 & 48.0 & 64.0 & 4.6 & 45 & 48.9 & 71.1 & 2.2 & 35 & 42.9 & 68.6 & 1.6 & 12 & 41.7 & 58.3 & 8.3 \\
\addlinespace
Gemini-3.1-Pro (Gemini CLI)  & 50 & 60.0 & 86.0 & 4.2 & 45 & 62.2 & \textbf{82.2} & 6.8 & 35 & \textbf{60.0} & \textbf{82.9} & 2.9 & 12 & 16.7 & 50.0 & 4.8 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Prompt interventions for abstention.} We tested four case-agnostic interventions against an
unmodified baseline: a post-retrieval abstention decision-gate, a structured answer format separating
claims-and-evidence from the verdict, a self-critique pass, and an underspecification check. None
reliably lifts abstention. The gate and the structured format both \emph{lower} \textit{lack} recall,
self-critique nudges the stronger model's accuracy while committing more often, and the
underspecification check, the one positive, raises the weaker model's \textit{lack} recall at flat
accuracy but does not transfer to the stronger model. The effects are small, mixed and model-dependent,
which is itself evidence that under-abstention is a genuine benchmark axis rather than a shallow
prompting artefact. These four ran on an earlier build of the case prompts and grading stack, so their
absolute numbers are not comparable with the tables here. We report the direction and withhold the
table rather than invite a comparison the data does not support.

\paragraph{Harness versus model.} Holding the model fixed and varying the harness across three
model-agnostic harnesses moves accuracy little: the spread is smaller than the across-model spread
within a single harness, and no pairwise difference approaches significance on a paired test
(Table~\ref{tab:ablation-harness}). What separates the harnesses is cost, as median completion tokens
differ severalfold for accuracy differences inside noise, so at a fixed model the harness is an
efficiency choice more than a capability one.

\begin{table}[htbp]
\centering
\caption{\textbf{At a fixed model, the harness is not the dominant term.} DeepSeek-V4-Pro under three model-agnostic harnesses over the same 142 development cases. Accuracy spans 5.6 points --- no pair exceeding 1.0\,SE$_d$ (exact McNemar $p\geq0.17$) and well inside the across-model spread within one harness --- while median completion tokens differ 4.2-fold. Process adherence separates them no further (worst pair 1.5\,SE$_d$).}
\label{tab:ablation-harness}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lcccccc}
\toprule
\textbf{Harness} & \textbf{Acc \%} & $\Delta$ & $p$ & \textbf{Proc \%} & \textbf{Turns} & \textbf{Comp.\ tok} \\
\midrule
  \texttt{opencode} & 66.2\,$\pm$\,4.0 & --- & --- & 68.6\,$\pm$\,2.3 & 13 & 4\,874 \\
  \texttt{qwen-coder} & 60.6\,$\pm$\,4.1 & $-5.6$ & 0.17 & 63.6\,$\pm$\,2.4 & 15 & 9\,357 \\
  \texttt{mini-swe-agent} & 64.8\,$\pm$\,4.0 & $-1.4$ & 0.86 & 67.6\,$\pm$\,2.2 & 48 & 20\,370 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Test-time compute (reasoning effort).} A default-versus-\texttt{high} contrast measures
nothing here, for two separate reasons. The Codex adapter sets \texttt{reasoning\_effort} to
\texttt{high} unless told otherwise, so those two conditions are one. And Claude Code, which sets no
default, already runs at the top of the range: over the cases both arms completed, the median
\emph{within-case} ratio of default to \texttt{high} completion tokens is 1.000. We therefore compare
three explicit levels on one model over the same 142 cases (Table~\ref{tab:ablation-effort}). Compute
rises substantially, 39\% from \texttt{low} to \texttt{medium} and 74\% end to end, as median
within-case ratios rather than ratios of medians. Quality does not follow. Accuracy spans 1.4 points
with every pairwise difference inside 0.3 standard errors and both exact McNemar tests far from
significance, and process adherence separates the levels no further. Additional test-time compute buys
neither better verdicts nor a better-documented method, which is what one expects if the binding
constraint is retrieval elicitation and label discrimination rather than reasoning depth. One limit is
that the trajectories expose no reasoning-token count, so completion tokens are the only available
compute proxy and we cannot say \emph{where} the extra compute was spent.

\begin{table}[htbp]
\centering
\caption{\textbf{Test-time compute buys compute, not accuracy.} Opus 4.8 on Claude Code, three explicit reasoning-effort levels over the same 142 development cases. Completion tokens rise 41\% to \texttt{medium} and 74\% end to end, but no pairwise accuracy difference exceeds 0.3\,SE$_d$ (exact McNemar $p\geq0.80$) and no process difference exceeds 1.2\,SE$_d$. Reasoning depth is not the binding constraint on this benchmark.}
\label{tab:ablation-effort}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lcccccc}
\toprule
\textbf{Effort} & \textbf{Acc \%} & $\Delta$ & $p$ & \textbf{Proc \%} & \textbf{Comp.\ tok} & $\Delta$\,tok \\
\midrule
  \texttt{low} & 67.6\,$\pm$\,3.9 & -- & -- & 64.5\,$\pm$\,2.3 & 7\,030 & -- \\
  \texttt{medium} & 69.0\,$\pm$\,3.9 & $+1.4$ & 0.81 & 68.2\,$\pm$\,2.1 & 9\,776 & $+41$\% \\
  \texttt{high} & 69.0\,$\pm$\,3.9 & $+1.4$ & 0.80 & 68.5\,$\pm$\,2.4 & 12\,014 & $+74$\% \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Qualitative Analysis}
\label{sec:qualitative}
The aggregate scores hide a failure signature that trap-adjusted accuracy makes precise. A cirrhotic
patient is admitted with hepatic encephalopathy and moderate ascites, and no diagnostic paracentesis
appears anywhere in the admission, so spontaneous bacterial peritonitis can be neither confirmed nor
excluded and the reference verdict is \textit{Indeterminate: Lack of Data}. All five systems commit to
a definitive label, and four reach it through the same prohibited shortcut, asserting peritonitis
excluded with no ascitic-fluid result, the \textsc{must-not} criterion N4
(Table~\ref{tab:qual-he-precipitant}). The failure is not one of retrieval: every one of the five names
the missing paracentesis in its own report, and the process judge's justifications independently
describe the same mechanism, that the systems acknowledged the absent study and then treated the
diagnosis as effectively worked up. The sharpest case is GPT-5.6-Luna, which performs the deferral
reasoning correctly, earns the criterion rewarding escalation of an unresolved question, and avoids the
trap, yet still emits a definitive \textit{No}. Recognising an evidentiary gap is therefore not
sufficient. Here the failure occurs at label assignment, after the reasoning that should have prevented
it. This is why the benchmark scores the observable adjudication process separately from the verdict,
and why raw and trap-adjusted accuracy diverge.

\begin{table}[htbp]
\centering
\small
\caption{\textbf{Qualitative failure profile} (\texttt{he-precipitant-278ac1}). No diagnostic
paracentesis exists in the admission, so spontaneous bacterial peritonitis can be neither confirmed
nor excluded. Four of the five spring the same \textsc{must-not} criterion N4, ``Asserted SBP
excluded without an ascitic-fluid result''. GPT-5.6-Luna avoids the trap and earns the escalation
criterion, yet still commits.}
\label{tab:qual-he-precipitant}
\begin{tabular}{llcc}
\toprule
\textbf{System} & \textbf{Verdict} & \textbf{Stated conf.} & \textbf{Trap sprung} \\
\midrule
\emph{Gold} & \textit{Indeterminate: Lack of Data} & -- & -- \\
\midrule
Claude Sonnet 5 (Claude Code)   & Yes & \phantom{0}90\% & N4 \\
Claude Opus 4.8 (Claude Code)   & Yes & \phantom{0}90\% & N4 \\
GPT-5.5 (Codex)                 & Yes & \phantom{0}78\% & N4 \\
Gemini-3.5-Flash (Gemini CLI)   & Yes & 100\% & N4 \\
GPT-5.6-Luna (Codex)            & No  & \phantom{0}78\% & -- \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Benchmark Validation: Judge Reliability}
\label{sec:validation}
The process score and the reference labels both feed the rankings, so we validate each. The reference
labels are validated against independent clinician judgment in Section~\ref{sec:clinical-calibration}
(91\% agreement on the calibration sample, $\kappa=0.87$); here we validate the LLM-judged process and
policy scores.

\paragraph{Judge reliability and self-consistency.} The process rubric is LLM-adjudicated,
so we measure whether the grade is stable across judges rather than assuming it. A five-judge
panel grades every trajectory over the full rubric with three replicates each. We report
inter-judge agreement primarily as the mean pairwise disagreement. It flags 16\% of
criteria as contested, with the judges self-consistent across replicates and statistically
interchangeable on the aggregate score (companion Fleiss' $\kappa \approx 0.65$). The
most-contested criteria (for example, a hidden antibiotic de-escalation window and an
era-dependent heart-failure therapy) are exactly the cases an independent expert audit flagged
as under-specified, so judge disagreement acts as an automatic detector of ambiguous criteria,
which are then routed back for expert revision. This supports reporting the process score as a
real metric rather than judge noise.

\paragraph{Grounding-metric determinism and judge reliability.} The four patient-evidence grounding
metrics divide by construction, and each is validated according to what it produces.
$P_{\mathrm{record}}$ and $R_{\mathrm{retrieval}}$ are computed by rule from the trace and involve no
judge at all: recomputing them over a complete 750-case run returns every per-run value unchanged.
The other two are LLM-judged, so we grade the same reports twice and compare the two passes.
$C_{\mathrm{finding}}$ asks the judge one covered$/$not-covered question per rubric category. Because
those categories are fixed in advance, the two passes can be compared question by question: over 200
reports, 50 per harness family, they agree on 97.6\% of 1{,}310 category decisions (Cohen's
$\kappa=0.94$), 175 of the 200 reports receive an identical score, and no family average moves by
more than 0.005. $P_{\mathrm{claim}}$ gives no such fixed question list, because the judge must first
break the report into atomic claims and it does not divide it the same way twice; there is nothing to
align, so we report how far the score itself moves, which is at most 0.02 and in no consistent
direction. We therefore treat the two rule-based metrics as exact, $C_{\mathrm{finding}}$ as
reproducible, and differences of 0.02 or less on $P_{\mathrm{claim}}$ as noise.

\paragraph{Policy-judge reliability and self-consistency.} The policy rubric is mostly deterministic:
citation existence and policy relevance are computed by rule, while only citation support requires LLM
judgement. Accordingly, the two rule-based items achieve perfect agreement ($\kappa=1.0$) with no
replicate variation, and the remaining LLM judgement is stable across judges (companion Fleiss'
$\kappa\approx0.86$, within-judge noise 0.023--0.025 on a $0,1$ scale). The production judge is
therefore representative rather than unusually strict or lenient. The residual variation is systematic:
judges sometimes under-credit near-verbatim citations, making citation-correctness scores conservative
lower bounds, and we find no evidence of own-family favouritism. By defining policy relevance through
expert gold documents rather than LLM judgement, we remove a major source of ambiguity at the
rubric-design stage. This supports treating the policy score as a meaningful metric rather than judge
noise.

==> OLDresult_bk_0804.tex <==
\section{Experimental Results}
\label{sec:experiments}


We evaluate autonomous systems along two axes: a leaderboard of production agent harnesses, each
running its native frontier model, and a controlled comparison that fixes a single model-agnostic
harness and varies only the model. Using the metrics of Section~\ref{sec:eval_framework}, the
experiments target three dissociations the benchmark is built to expose. First, raw accuracy
overstates sound clinical reasoning, because a verdict can be reached through a prohibited shortcut.
Second, systems systematically under-abstain, committing to a definitive answer where the record
warrants deferral. Third, accuracy exceeds grounding fidelity, because models reach the right verdict
without citing the evidence that justifies it.

\subsection{Experimental Setup}
\label{sec:exp-setup}

\paragraph{Harnesses.} We run four agent harnesses. \texttt{Claude Code}, \texttt{Codex} and
\texttt{Gemini CLI} are production agent CLIs, each locked to its own vendor model family and driving
the benchmark tools through a native tool-calling loop, so they represent how each model is actually
deployed. \texttt{opencode} is a model-agnostic open-source harness that connects to the same MIMIC
tool server as the others. Because it can drive any model, it serves as the fixed neutral harness for
the model-comparison axis, isolating the model's contribution from the harness's. All four run with
web search and fetch disabled, so every system answers from the in-environment patient record and
policy corpus alone, a frozen-corpus condition enforced by a deny-by-default egress allowlist rather
than by instruction. MIMIC data is reached only through a credential-isolated tool server, so no
system can bypass the governed tools to read raw records.

\paragraph{Models.} Table~\ref{tab:exp-matrix} lists the sixteen systems evaluated. The native
leaderboard pairs each harness with its frontier models, and the model-comparison axis runs a set of
open-weight models on the neutral \texttt{opencode} harness, isolating the model from the harness.
Running the vendor models on \texttt{opencode} for a fully harness-controlled comparison is planned.
We exclude medical-specialized models from the agentic leaderboard because they cannot drive a
multi-step tool-calling loop and would score near zero from harness incompatibility rather than
clinical weakness. Where relevant we report them separately as a single-turn probe.

\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2}
\caption{\textbf{Systems evaluated in CliniCARE-Bench.} Native leaderboard (each harness on its own
frontier model) and the controlled model comparison on the neutral \texttt{opencode} harness.}
\label{tab:exp-matrix}
\begin{tabularx}{\linewidth}{@{}lX@{}}
\toprule
\textbf{Harness} & \textbf{Models} \\
\midrule
\multicolumn{2}{@{}l}{\textit{Native leaderboard: each harness on its own frontier model}} \\
\addlinespace[2pt]
\texttt{Claude Code} & Claude Opus 5, Claude Sonnet 5 \\
\texttt{Codex}       & GPT-5.6 Sol, GPT-5.6 Luna, GPT-5.5, GPT-5.4, GPT-5.4-mini \\
\texttt{Gemini CLI}  & Gemini 3.1 Pro, Gemini 3.5 Flash, Gemini 3.6 Flash \\
\addlinespace[6pt]
\midrule
\multicolumn{2}{@{}l}{\textit{Controlled comparison: open-weight models on one neutral harness}} \\
\addlinespace[2pt]
\texttt{opencode} & DeepSeek V4 Pro, DeepSeek V4 Flash, Qwen 3.7 Plus, GLM 5.2,
                    MiniMax M3, Kimi K2.7 Code \\
\bottomrule
\end{tabularx}
\end{table}

\paragraph{cases and verdict classes.} The cohort is 25 clinical scenarios $\times$ 30 patients
$=750$ cases, each a single adjudication question resolved to one of the four verdict classes defined
in Section~\ref{sec:eval_framework}: \textit{Yes}, \textit{No}, and the two deferral classes we
abbreviate \textit{lack} (\textit{Indeterminate: Lack of Data}) and \textit{amb} (\textit{Indeterminate:
Medically Ambiguous}). The verdict is scored deterministically by exact four-class match, with no
partial credit.

\paragraph{Metrics.} Four-class accuracy and macro-F1, the two directional abstention errors
(\emph{over-commitment} and \emph{over-abstention}), process adherence (LLM-judged, pinned to
\texttt{openai/gpt-5.5}), evidence and policy grounding, repeated-run reliability (avg@3,
pass\textasciicircum{}3, pass@3) and per-run cost all follow the definitions in
Section~\ref{sec:eval_framework}. Accuracy is reported per run (micro), which coincides with the
scenario-macro average on a complete arm but not on a partial one. Two quantities are specific to this
section and introduced where first used: \emph{trap-adjusted accuracy} with its \emph{trap gap}, which
credit a verdict only when no \textsc{must-not} rubric criterion was violated, and expected calibration
error (Eq.~\ref{eq:ece}).

\subsection{Results}
\label{sec:main-results}

Every system is run on all 750 cases at a single attempt against the silver reference labels.
Table~\ref{tab:main750} reports the full leaderboard: verdict accuracy and macro-F1, trap-adjusted
accuracy and the gap it opens, process adherence, the two directional abstention errors, calibration,
and per-run cost. Two points bear noting before reading it. The \emph{Gap} column is raw accuracy
minus trap-adjusted accuracy \emph{over report-present runs only}, so it is not the difference of
the two columns beside it. The cost columns are measured on two different instruments: harness-reported
for the vendor CLIs, but computed from measured tokens for the \texttt{opencode} arms, which report
neither a cost field nor a cached-token count. Those six are therefore given as ranges rather than
point estimates.

\begin{table}[htbp]
\centering
\caption{\textbf{Primary leaderboard on the complete 750-case cohort.} Single attempt against silver
labels, all sixteen arms on all 750 cases. \emph{Trap-adj} is trap-adjusted accuracy, \emph{Gap} the
trap gap (raw minus trap-adjusted over report-present runs), \emph{Over-com}$/$\emph{Over-abs} the
directional abstention errors, \emph{Proc\%} the LLM-judged process score, and \emph{ECE} expected
calibration error. Cost columns are per-run medians except USD$/$run (a mean, excluding judge
spend). \texttt{opencode} work-token and USD figures are ranges because that adapter reports no
cached-token count.}
\label{tab:main750}
\footnotesize
\setlength{\tabcolsep}{2.2pt}
\begin{tabular}{lcccccccccccc}
\toprule
 & \multicolumn{5}{c}{\textbf{Quality}} & \multicolumn{3}{c}{\textbf{Abstention \& calibration}} & \multicolumn{4}{c}{\textbf{Cost \& efficiency}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-9}\cmidrule(lr){10-13}
\textbf{Model} & \textbf{Acc} & \textbf{Mac-F1} & \textbf{Trap-adj} & \textbf{Gap} & \textbf{Proc\%} & \textbf{Over-com} & \textbf{Over-abs} & \textbf{ECE} & \textbf{Turns} & \textbf{Tools} & \textbf{Work-tok} & \textbf{USD/run} \\
\midrule
\multicolumn{13}{@{}l}{\texttt{Claude Code}}\\
\quad Opus 5 & 72.3 & 0.633 & 62.9 & 9.3 & 80.2 & 29.2 & 15.2 & 0.098 & 17 & 28 & 130.1k & 2.04 \\
\quad Sonnet 5 & 70.8 & 0.603 & 59.5 & 11.3 & 69.6 & 28.5 & 16.1 & 0.071 & 13 & 22 & 90.2k & 0.94 \\
\addlinespace
\multicolumn{13}{@{}l}{\texttt{Codex}}\\
\quad GPT-5.6-Sol      & 70.8 & 0.619 & 64.1 & 6.7 & 79.6 & 26.9 & 16.6 & 0.217 & 22 & 16 & 88.4k & 1.11 \\
\quad GPT-5.6-Luna     & 64.5 & 0.552 & 57.2 & 7.3 & 75.0 & 36.9 & 20.5 & 0.250 & 22 & 18 & 97.5k & 0.25 \\
\quad GPT-5.5 & 73.2 & 0.655 & 67.1 & 6.1 & 78.6 & 33.8 & 12.6 & 0.118 & 18 & 49 & 122.2k & 1.53 \\
\quad GPT-5.4          & 68.9 & 0.610 & 61.1 & 7.9 & 75.8 & 33.8 & 15.3 & 0.173 & 21 & 52 & 111.3k & 0.72 \\
\quad GPT-5.4-mini     & 64.7 & 0.535 & 54.3 & 10.4 & 66.8 & 50.8 & 16.1 & 0.231 & 24 & 44 & 84.1k & 0.20 \\
\addlinespace
\multicolumn{13}{@{}l}{\texttt{Gemini CLI}}\\
\quad Gemini-3.6-Flash & 70.5 & 0.608 & 56.4 & 14.1 & 72.3 & 35.4 & 11.6 & 0.274 & 62 & 36 & 385.0k & 1.13 \\
\quad Gemini-3.5-Flash & 70.0 & 0.590 & 57.6 & 12.4 & 72.0 & 38.5 & 11.8 & 0.279 & 62 & 36 & 387.8k & 1.16 \\
\quad Gemini-3.1-Pro   & 70.3 & 0.626 & 54.4 & 15.9 & 58.6 & 18.5 & 15.5 & 0.279 & 42 & 23 & 205.7k & 1.02 \\
\addlinespace
\multicolumn{13}{@{}l}{\texttt{opencode} \textnormal{(open-weight models on the neutral harness)}}\\
\quad DeepSeek-V4-Pro & 67.3 & 0.581 & 54.4 & 12.9 & 70.2 & 34.6 & 14.0 & 0.201 & 14 & 41 & 62--576k & 0.21--1.12 \\
\quad DeepSeek-V4-Flash & 69.1 & 0.554 & 57.5 & 11.6 & 68.9 & 49.2 & 11.5 & 0.230 & 15 & 46 & 77--729k & 0.03--0.12 \\
\quad GLM-5.2 & 72.1 & 0.614 & 60.9 & 11.2 & 75.5 & 37.7 & 11.3 & 0.143 & 14 & 32 & 66--611k & 0.24--1.13 \\
\quad Qwen-3.7-Plus & 62.4 & 0.522 & 50.1 & 12.3 & 65.0 & 40.8 & 19.4 & 0.209 & 11 & 28 & 47--435k & 0.06--0.19 \\
\quad MiniMax-M3 & 65.9 & 0.543 & 51.5 & 14.4 & 71.3 & 52.3 & 14.4 & 0.189 & 21 & 45 & 107--991k & 0.12--0.40 \\
\quad Kimi-K2.7-Code & 63.2 & 0.516 & 49.3 & 13.9 & 69.9 & 50.0 & 14.7 & 0.183 & 20 & 56 & 132--1261k & 0.97--3.36 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{No system resolves the cohort, and the loss concentrates in the rare classes.} Accuracy
spans 62.4 to 73.2 and macro-F1 0.516 to 0.655 (Table~\ref{tab:main750}): the strongest arm resolves
just under three-quarters of its graded cases and the weakest just over three-fifths. Macro-F1 trails
accuracy in every arm because it weights the two rare \textit{Indeterminate} classes equally with
\textit{Yes} and \textit{No}, so the loss concentrates where deferral must be recognised. Accuracy
forms a continuum rather than tiers, and the harness families interleave within it: no two adjacent
arms differ by more than 1.6 points across the whole eleven-point span, and two vendor arms
(GPT-5.6-Luna 64.5, GPT-5.4-mini 64.7) place below four of the open-weight models on the neutral
harness. The best open-weight arm, GLM-5.2 at 72.1, is indistinguishable from the best vendor arm
(GPT-5.5, 73.2) at this $n$, where one binomial standard error is about 1.6 points.

\paragraph{Trap-adjusted accuracy: what it is, and why it reorders the field.} A \emph{trap} is a
\textsc{must-not} criterion in the case's rubric, an inferential shortcut a clinician reviewing the
work would reject outright, such as reading acute kidney injury off a billing code, asserting contrast
causation from temporal proximity alone, or citing a policy document that does not exist.
\emph{Trap-adjusted accuracy} counts a run correct only when the verdict is right \emph{and} no
\textsc{must-not} criterion was violated, and the \emph{Gap} column is raw minus trap-adjusted accuracy
over report-present runs, so it is the share of an arm's correct verdicts reached by a forbidden
route. Every system pays between 6.1 and 15.9 points (Table~\ref{tab:main750}), meaning that between
one in twelve and one in four of its correct answers does not survive inspection of how it was
reached.

The spread is the finding, not the magnitude (\Cref{fig:trap}). Were raw accuracy merely optimistic by
a fixed margin, the gap would be roughly constant and the ranking would survive the correction. It
does not. GPT-5.5 loses 6.1 points while Gemini-3.1-Pro loses 15.9, so the correction reorders the
field. Gemini-3.1-Pro reaches 70.3 raw accuracy, within noise of the leading group, then falls to 54.4
trap-adjusted, below every Claude arm and every Codex arm bar GPT-5.4-mini, which it ties.
Gemini-3.1-Pro is also the arm \emph{least} prone to over-commitment (18.5\%), so springing traps and
over-committing are distinct failures rather than two faces of the same carelessness. This
operationalises, on real longitudinal records, the
reasoning-versus-pattern-matching gap documented for medical LLMs
\cite{bedi2025fidelity, natmed2026robustness}: a correct label is not evidence of correct reasoning,
and only a trace-level audit of the investigation distinguishes the two. It is the concrete payoff of
scoring the observable adjudication process rather than the final answer alone.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_trap_adjusted.pdf}
\caption{\textbf{Trap-adjusted accuracy reorders the leaderboard.} Raw accuracy (open circles) and
trap-adjusted accuracy (filled markers) for all sixteen arms, ordered by trap-adjusted accuracy;
marker colour denotes the harness family and connector length is the trap gap. Gemini-3.1-Pro falls
from within noise of the leaders to below every Claude and Codex arm bar GPT-5.4-mini once forbidden-route
answers are removed, while GPT-5.5 loses least.}
\label{fig:trap}
\end{figure}

\paragraph{Systems under-abstain: over-commitment exceeds over-abstention in every arm.} Measured
directionally (\Cref{fig:abstention}), over-commitment, returning a definitive verdict where the
reference verdict is \textit{Indeterminate}, runs 18.5--52.3\% against over-abstention of
11.3--20.5\%, and \emph{all sixteen} systems over-commit at the higher rate. That the asymmetry holds
arm by arm rather than only in aggregate makes it a property of the systems rather than of the label
distribution, and it reproduces on the development subset (Section~\ref{sec:ablations}). The failure
is not an unwillingness to answer but an unwillingness to decline. The magnitude, not the direction, is
what varies: three arms over-commit on at least half of all deferral cases (MiniMax-M3 52.3\%,
GPT-5.4-mini 50.8\%, Kimi-K2.7-Code 50.0\%) while Gemini-3.1-Pro does so on 18.5\%. Over-abstention, by
contrast, is tightly banded at 11.3--20.5\%, and its highest value belongs to a vendor arm
(GPT-5.6-Luna), so the deferral side of the error budget varies far less across systems than the
commitment side.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_underabstention.pdf}
\caption{\textbf{Every system under-abstains.} Directional abstention errors for all sixteen arms:
over-abstention (open circles) and over-commitment (filled markers), each over that arm's own gold
supports; marker colour denotes the harness family. Over-commitment exceeds over-abstention in every
arm. GPT-5.4-mini, MiniMax-M3 and Kimi-K2.7-Code over-commit on half of all deferral cases, whereas
Gemini-3.1-Pro is the only near-balanced arm.}
\label{fig:abstention}
\end{figure}

\paragraph{The process score measures something the verdict does not.} Process adherence
(Table~\ref{tab:main750}) is judged against the rubric's observable investigation steps rather than
against the answer, and it separates arms that accuracy places together. Opus 5 scores 80.2 on process
against 72.3 accuracy, whereas Gemini-3.1-Pro reaches 70.3 accuracy on a process score of 58.6, the
same verdict quality reached through a materially less defensible investigation. This is the trap gap
seen from the other side. The per-class picture (\Cref{fig:perclass}) tells the same story from the
verdict side: \textit{Yes} and \textit{No} F1 stay strong across the roster while both
\textit{Indeterminate} classes fall away, and precision on the deferral classes is low throughout
(\textit{lack} 31--49\%, \textit{amb} 25--67\%), so the deferrals systems do issue are frequently made
on records that in fact settle the question. For a clinical deliverable this matters more than the
headline: a reader can audit a documented investigation but not a bare verdict.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_perclass_f1.pdf}
\caption{\textbf{Performance collapses on the two safety-critical \textit{Indeterminate} classes.}
Per-class F1 for all sixteen arms on the complete cohort (rows in leaderboard order, grouped by
harness via the colour bar at left). \textit{Yes} and \textit{No} stay strong while both deferral
classes (dashed box) fall away on the weaker arms. Precision on the deferral classes is low throughout
(\textit{lack} 31--49\%, \textit{amb} 25--67\%).}
\label{fig:perclass}
\end{figure}

\paragraph{The leaderboard order does not hold scenario by scenario.} Resolved per scenario
(\Cref{fig:scenario}), the aggregate ordering of Table~\ref{tab:main750} survives in only 68.5\% of
the 3{,}000 arm-pair $\times$ scenario comparisons the grid contains, and fifteen of the sixteen arms
are the best system on at least one scenario, including Kimi-K2.7-Code, second from last on the
leaderboard, which leads on \texttt{he-precipitant} and \texttt{overdose-disposition}. The ordering of the averages is nevertheless stable: an arm's cohort accuracy predicts its mean per-scenario rank almost perfectly (Spearman $\rho=-0.95$, negative only because rank 1 is best). Even so, Opus 5, second on the leaderboard, sits in the
bottom quartile on one of the 25
scenarios. The leaderboard is
thus a statement about a case mix more than about which system to trust on a given clinical question.
Difficulty is concentrated rather than diffuse: cross-arm mean accuracy runs from 96.7 on
\texttt{discharge-audit} to 8.8 on \texttt{pe-workup}, the five hardest scenarios carry 36\% of all
errors against the 20\% that uniform difficulty implies, and one scenario has stopped separating
systems altogether. On \texttt{pe-workup} no arm exceeds 24\%, and the answers pooled over all sixteen
arms are overwhelmingly \textit{Indeterminate: Lack of Data} against a reference that reads
\textit{No} on most of its 30 cases. Sixteen independently built systems agreeing that a record is
insufficient is more readily explained by the reference labels for that scenario than by a shared
clinical blind spot, so \texttt{pe-workup} is queued for label adjudication. It is still counted in
every number reported here.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_scenario_accuracy.pdf}
\caption{\textbf{The leaderboard order does not hold scenario by scenario.} Verdict accuracy of every
arm on each of the 25 scenarios, one dot per arm coloured by harness family, with the cross-arm mean
(dark line). Scenarios are sorted by that mean.}
\label{fig:scenario}
\end{figure}

% \begin{table}[htbp]
% \centering
% \caption{\textbf{Per-class F1, with precision and recall for the two \textit{Indeterminate}
% classes.} The two rightmost cells read P\,$/$\,R. Denominators follow the cohort's natural label
% distribution, not the development subset's balanced one, so cells are not comparable with
% Table~\ref{tab:dev-perclass}.}
% \label{tab:main750-perclass}
% \small
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{lccccccc}
% \toprule
%  & & \multicolumn{4}{c}{\textbf{F1}} & \multicolumn{2}{c}{\textbf{Precision\,$/$\,Recall \%}} \\
% \cmidrule(lr){3-6}\cmidrule(lr){7-8}
% \textbf{Model (harness)} & \textbf{n} & Yes & No & lack & amb & lack & amb \\
% \midrule
% % <<<AUTOROWS750:tab:main750-perclass>>>
% Opus 5 (Claude Code)           & 750 & 0.818 & 0.738 & 0.506 & 0.473 & 41.2\,/\,65.3 & 50.0\,/\,44.8 \\
% Sonnet 5 (Claude Code) & 750 & 0.800 & 0.726 & 0.515 & 0.373 & 41.7\,/\,67.3 & 36.7\,/\,37.9 \\
% \addlinespace
% GPT-5.6-Sol (Codex)            & 750 & 0.795 & 0.734 & 0.515 & 0.433 & 41.3\,/\,68.3 & 41.9\,/\,44.8 \\
% GPT-5.6-Luna (Codex)           & 750 & 0.740 & 0.694 & 0.402 & 0.373 & 32.5\,/\,52.5 & 30.4\,/\,48.3 \\
% GPT-5.5 (Codex)                & 750 & 0.824 & 0.746 & 0.492 & 0.560 & 42.0\,/\,59.4 & 66.7\,/\,48.3 \\
% GPT-5.4 (Codex)                & 750 & 0.774 & 0.717 & 0.466 & 0.483 & 38.8\,/\,58.4 & 48.3\,/\,48.3 \\
% GPT-5.4-mini (Codex)           & 750 & 0.770 & 0.657 & 0.351 & 0.364 & 31.5\,/\,39.6 & 32.4\,/\,41.4 \\
% \addlinespace
% Gemini-3.6-Flash (Gemini CLI)  & 750 & 0.804 & 0.695 & 0.504 & 0.429 & 45.0\,/\,57.4 & 44.4\,/\,41.4 \\
% Gemini-3.5-Flash (Gemini CLI)  & 750 & 0.794 & 0.703 & 0.487 & 0.377 & 43.4\,/\,55.4 & 41.7\,/\,34.5 \\
% Gemini-3.1-Pro (Gemini CLI)    & 750 & 0.775 & 0.716 & 0.556 & 0.458 & 43.2\,/\,78.2 & 57.9\,/\,37.9 \\
% \addlinespace
% DeepSeek-V4-Pro (opencode) & 750 & 0.769 & 0.686 & 0.463 & 0.407 & 39.7\,/\,55.4 & 40.0\,/\,41.4 \\
% DeepSeek-V4-Flash (opencode) & 750 & 0.809 & 0.688 & 0.411 & 0.308 & 38.9\,/\,43.6 & 34.8\,/\,27.6 \\
% GLM-5.2 (opencode) & 750 & 0.808 & 0.732 & 0.519 & 0.400 & 48.7\,/\,55.4 & 36.1\,/\,44.8 \\
% Qwen-3.7-Plus (opencode) & 750 & 0.734 & 0.656 & 0.371 & 0.329 & 31.3\,/\,45.5 & 26.0\,/\,44.8 \\
% MiniMax-M3 (opencode) & 750 & 0.767 & 0.678 & 0.362 & 0.366 & 34.9\,/\,37.6 & 31.0\,/\,44.8 \\
% Kimi-K2.7-Code (opencode) & 750 & 0.734 & 0.664 & 0.356 & 0.308 & 34.6\,/\,36.6 & 24.5\,/\,41.4 \\
% % <<<END750:tab:main750-perclass>>>
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[htbp]
% \centering
% \caption{\textbf{Verdict accuracy (\%) per scenario, all 16 arms.} Rows are the 25 clinical
% scenarios, sorted by the unweighted mean over arms given in the last column; the best cell in each row
% is bold. A cell's denominator is that arm's graded runs for that scenario, exactly 30 for every
% cell in the grid, so a single cell is a weaker estimate than a row or a column.
% Column key: O5\,=\,Opus 5, S5\,=\,Sonnet 5, Sol\,=\,GPT-5.6-Sol, Luna\,=\,GPT-5.6-Luna, 5.5\,=\,GPT-5.5, 5.4\,=\,GPT-5.4, 5.4m\,=\,GPT-5.4-mini, G3.6\,=\,Gemini-3.6-Flash, G3.5\,=\,Gemini-3.5-Flash, G3.1\,=\,Gemini-3.1-Pro, D4P\,=\,DeepSeek-V4-Pro, D4F\,=\,DeepSeek-V4-Flash, GLM\,=\,GLM-5.2, Qwn\,=\,Qwen-3.7-Plus, MM3\,=\,MiniMax-M3, K2.7\,=\,Kimi-K2.7-Code.}
% \label{tab:scenario-table}
% \small
% \setlength{\tabcolsep}{3pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccccccccccccccc}
% \toprule
% \textbf{Scenario} & \textbf{O5} & \textbf{S5} & \textbf{Sol} & \textbf{Luna} & \textbf{5.5} & \textbf{5.4} & \textbf{5.4m} & \textbf{G3.6} & \textbf{G3.5} & \textbf{G3.1} & \textbf{D4P} & \textbf{D4F} & \textbf{GLM} & \textbf{Qwn} & \textbf{MM3} & \textbf{K2.7} & \textbf{Mean} \\
% \midrule
% % <<<SCENROWS:tab:scenario-table>>>
% discharge-audit          & 97 & \textbf{100} & \textbf{100} & 97 & \textbf{100} & \textbf{100} & \textbf{100} & 93 & 97 & 90 & 97 & 90 & \textbf{100} & 90 & \textbf{100} & 97 & 96.7 \\
% eol-goal-concordance     & 93 & 93 & \textbf{100} & 97 & 93 & 97 & 93 & 90 & 90 & \textbf{100} & 77 & 93 & 90 & 83 & 87 & 90 & 91.7 \\
% overdose-disposition     & 87 & \textbf{97} & 87 & 83 & 90 & 90 & \textbf{97} & \textbf{97} & \textbf{97} & 90 & 93 & \textbf{97} & 90 & 80 & 80 & \textbf{97} & 90.6 \\
% renal-trajectory         & 87 & 93 & 90 & 90 & 93 & 90 & \textbf{97} & 83 & 93 & 90 & 90 & 83 & 83 & 87 & 90 & 83 & 89.0 \\
% transfusion-audit        & 87 & \textbf{90} & 87 & 83 & \textbf{90} & \textbf{90} & 87 & \textbf{90} & \textbf{90} & \textbf{90} & 87 & \textbf{90} & \textbf{90} & 83 & \textbf{90} & 83 & 87.9 \\
% advanced-imaging         & 83 & 87 & 87 & \textbf{90} & 83 & 77 & 67 & 87 & 87 & 77 & 80 & 73 & 87 & 77 & 73 & 77 & 80.6 \\
% hfref-gdmt               & 80 & \textbf{87} & 83 & 63 & 83 & 73 & 70 & 83 & 83 & 77 & 77 & 73 & 80 & 73 & 70 & 70 & 76.7 \\
% post-ct-aki              & 83 & 83 & 90 & \textbf{93} & 90 & 73 & 80 & 73 & 77 & 73 & 60 & 77 & 67 & 60 & 80 & 67 & 76.7 \\
% readmission-30d          & 70 & 73 & 80 & 87 & 87 & 83 & 70 & 83 & 77 & \textbf{90} & 73 & 67 & 77 & 70 & 67 & 63 & 76.0 \\
% goals-of-care            & 93 & 90 & 90 & 60 & 87 & 83 & 57 & 67 & 70 & \textbf{97} & 83 & 77 & 83 & 63 & 57 & 53 & 75.6 \\
% frequent-admitter        & 77 & 70 & 83 & 77 & 77 & 63 & 63 & \textbf{87} & 77 & 83 & 67 & 73 & 83 & 77 & 63 & 67 & 74.2 \\
% icu-delirium             & 67 & \textbf{83} & 60 & 63 & 63 & 67 & 67 & 77 & 73 & 63 & 60 & 60 & 77 & 67 & 63 & 80 & 68.1 \\
% med-reconciliation       & \textbf{87} & 70 & 73 & 57 & 60 & 60 & 53 & 60 & 70 & 83 & 73 & 53 & 83 & 57 & 57 & 60 & 66.0 \\
% sepsis-source-abx        & 77 & 60 & 63 & 43 & 70 & 67 & 73 & \textbf{80} & 67 & 73 & 57 & 77 & 77 & 57 & 67 & 47 & 65.8 \\
% postop-complications     & 53 & 60 & 57 & 63 & 70 & 67 & 67 & 70 & 67 & 67 & 70 & \textbf{77} & 63 & 63 & 67 & 67 & 65.4 \\
% ams-workup               & 73 & 60 & 77 & 70 & 70 & 67 & 37 & 67 & 60 & 57 & \textbf{83} & 57 & 67 & 60 & 60 & 63 & 64.2 \\
% dka-resolution           & 83 & 57 & 87 & 60 & \textbf{90} & 77 & 23 & 73 & 67 & 60 & 53 & 47 & 70 & 43 & 53 & 63 & 62.9 \\
% hyperkalemia-management  & 60 & 57 & 63 & 60 & 70 & 70 & 67 & 47 & 53 & 53 & 67 & 60 & \textbf{80} & 63 & 63 & 67 & 62.5 \\
% empiric-abx              & 70 & \textbf{73} & 63 & 57 & 70 & 63 & 63 & 63 & 63 & 67 & 63 & 60 & 67 & 50 & 40 & 43 & 61.0 \\
% he-precipitant           & 57 & 53 & 60 & 57 & 60 & 57 & 67 & 67 & 63 & 63 & 60 & 67 & 63 & 57 & 53 & \textbf{73} & 61.0 \\
% stroke-time-targets      & 67 & 57 & 53 & 50 & 63 & 57 & 53 & 70 & \textbf{73} & 53 & 63 & 67 & 57 & 53 & 67 & 60 & 60.2 \\
% anticoag-reversal        & 67 & 70 & 60 & 40 & 60 & 57 & 47 & 67 & 70 & 57 & 53 & \textbf{80} & 50 & 57 & 63 & 40 & 58.5 \\
% pneumonia-curb65         & 60 & 57 & 33 & 30 & 67 & 47 & 70 & 43 & 47 & 40 & 40 & 57 & 47 & 43 & \textbf{73} & 30 & 49.0 \\
% sepsis-bundle            & 40 & 43 & 37 & 37 & 33 & 40 & 43 & 43 & 37 & \textbf{53} & 50 & 50 & 50 & 43 & \textbf{53} & 40 & 43.3 \\
% pe-workup                & 10 & 7 & 7 & 7 & 10 & 10 & 7 & 3 & 3 & 10 & 7 & \textbf{23} & \textbf{23} & 3 & 10 & 0 & 8.8 \\
% <<<SCENEND:tab:scenario-table>>>
% \bottomrule
% \end{tabular}%
% }
% \end{table}

\paragraph{Calibration separates the systems more cleanly than accuracy does.} Every report states a
confidence, so we can ask whether that number carries information. Expected calibration error is the
bin-weighted deviation between stated confidence and realised accuracy,
\begin{equation}
\mathrm{ECE} \;=\; \sum_{b=1}^{B} \frac{|B_b|}{n}\,\bigl|\,\mathrm{conf}(B_b) - \mathrm{acc}(B_b)\,\bigr| ,
\label{eq:ece}
\end{equation}
over $B=10$ equal-width bins of stated confidence, where $\mathrm{conf}(B_b)$ and $\mathrm{acc}(B_b)$
are the mean stated confidence and realised accuracy in bin $b$. ECE spans 0.071--0.279 across the
sixteen arms, a near-fourfold range on an axis accuracy cannot see, and it does \emph{not} order them
the way accuracy does: the three best-calibrated are Sonnet 5 (0.071), Opus 5 (0.098) and GPT-5.5
(0.118), while the three worst are all Gemini CLI arms (0.274--0.279), which sit mid-field on accuracy.
For a report addressed to a clinician who cannot cheaply re-derive the answer, a confidence that does
not track correctness is arguably a more consequential defect than a few points of accuracy, and no
aggregate score above reveals it. One caveat on cross-arm comparison: an arm emitting few distinct
confidence values populates few bins, so its ECE is not measuring quite the same thing.

\paragraph{Cost and efficiency diverge from accuracy, and from each other.} Across the vendor arms a
tenfold spread in price buys only an $\sim$9-point accuracy band (\Cref{fig:cost}). GPT-5.4-mini and
GPT-5.6-Luna land within 0.2 points of each other on accuracy and cost \$0.20 and \$0.25 per run, so
every per-dollar ratio favours the cheaper one. What the extra spend buys is not correct verdicts but
cleaner ones, 2.9 more points of trap-adjusted accuracy and 8.1 more of process adherence, a purchase
worth making in this domain and invisible to any cost-per-accuracy-point ratio, which is why we do not
tabulate one. Composition differs more than total: GPT-5.4-mini issues a median 44 typed tool calls
against GPT-5.6-Luna's 18, roughly $2.4\times$ the retrieval traffic, while consuming \emph{fewer}
work-tokens (84.1k against 97.5k). The cheaper arm queries more and reasons less over what it
retrieves, and it is also the arm with the wider trap gap and the lower process score: more retrieval
does not substitute for sound adjudication of what was retrieved. Work-tokens are comparable only
within a serving path, and the \texttt{opencode} figures are ranges rather than point values because
that path reports no cached-token count and the cache correction has to be estimated.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_cost_accuracy.pdf}
\caption{\textbf{Accuracy rises only weakly with cost.} Per-run cost (USD, log scale,
harness-reported) against verdict accuracy for the ten vendor arms, coloured by harness family, with
$\pm1$ binomial standard error bars at $n=750$. The six \texttt{opencode} arms are omitted because
their per-run cost is a range rather than a point.}
\label{fig:cost}
\end{figure}

\subsection{Patient-Evidence Grounding}
\label{sec:grounding-results}

Grounding is where verdict accuracy and defensible reasoning most clearly diverge: a system can reach
the correct verdict without citing the evidence that justifies it. Table~\ref{tab:grounding-v3-full750}
reports the four patient-evidence grounding metrics of Section~\ref{sec:patient-grounding} for all sixteen
model--harness combinations over the same 750 cases. Two score \emph{citation precision}:
$P_{\mathrm{record}}$, the fraction of record identifiers cited in the report that occur in the
evidence the agent actually retrieved, and $P_{\mathrm{claim}}$, the fraction of the report's atomic
clinical claims judged \emph{supported} --- rather than \emph{contradicted} or \emph{unverifiable}
--- against their cited evidence, with correct patient, encounter, and temporal attribution required.
Two score \emph{evidence coverage}: $R_{\mathrm{retrieval}}$, the fraction of the case's
expert-specified record sources the agent queried, and $C_{\mathrm{finding}}$, the fraction of its
required-evidence categories the report establishes. All four are computed against the agent's own
investigation rather than against the reference verdict, so they capture whether a determination is
auditable, not whether it is correct. All four are stable under repetition: $P_{\mathrm{record}}$ and
$R_{\mathrm{retrieval}}$ are rule-based and return the same value on every computation, and both
$P_{\mathrm{claim}}$ and $C_{\mathrm{finding}}$ reproduce reliably when the same reports are regraded (Section~\ref{sec:validation}).


\begin{table}[htbp]
\centering
\caption{\textbf{Patient-evidence grounding on the complete 750-case cohort.} Citation precision at
the record-identifier and clinical-claim levels against coverage at the retrieval and reporting
stages, as defined in Section~\ref{sec:patient-grounding}. Columns are averaged over each system's
scoreable runs, those in which the agent both produced a report and retrieved at least one record.}
\label{tab:grounding-v3-full750}
\footnotesize
\setlength{\tabcolsep}{8pt}
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{\textbf{Citation precision}} & \multicolumn{2}{c}{\textbf{Evidence coverage}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\textbf{Model} & $P_{\mathrm{record}}$ & $P_{\mathrm{claim}}$ & $R_{\mathrm{retrieval}}$ & $C_{\mathrm{finding}}$ \\
\midrule
\multicolumn{5}{@{}l}{\texttt{Claude Code}}\\
\quad Opus 5           & 0.983 & 0.882 & 0.848 & 0.819 \\
\quad Sonnet 5         & 0.986 & 0.867 & 0.816 & 0.719 \\
\addlinespace
\multicolumn{5}{@{}l}{\texttt{Codex}}\\
\quad GPT-5.6-Sol      & 1.000 & 0.971 & 0.846 & 0.751 \\
\quad GPT-5.6-Luna     & 1.000 & 0.968 & 0.866 & 0.725 \\
\quad GPT-5.5          & 0.999 & 0.964 & 0.874 & 0.749 \\
\quad GPT-5.4          & 0.999 & 0.961 & 0.859 & 0.729 \\
\quad GPT-5.4-mini     & 0.997 & 0.964 & 0.812 & 0.667 \\
\addlinespace
\multicolumn{5}{@{}l}{\texttt{Gemini CLI}}\\
\quad Gemini-3.6-Flash & 0.995 & 0.897 & 0.856 & 0.786 \\
\quad Gemini-3.5-Flash & 0.995 & 0.892 & 0.858 & 0.785 \\
\quad Gemini-3.1-Pro   & 0.999 & 0.906 & 0.683 & 0.589 \\
\addlinespace
\multicolumn{5}{@{}l}{\texttt{opencode} \textnormal{(open-weight models on the neutral harness)}}\\
\quad DeepSeek-V4-Pro & 0.996 & 0.910 & 0.853 & 0.736 \\
\quad DeepSeek-V4-Flash & 0.991 & 0.913 & 0.865 & 0.733 \\
\quad GLM-5.2 & 0.989 & 0.919 & 0.815 & 0.745 \\
\quad Qwen-3.7-Plus & 0.991 & 0.923 & 0.797 & 0.690 \\
\quad MiniMax-M3 & 0.986 & 0.910 & 0.827 & 0.743 \\
\quad Kimi-K2.7-Code & 0.993 & 0.932 & 0.860 & 0.729 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Record-identifier precision saturates and does not separate the systems.}
$P_{\mathrm{record}}$ spans 0.983--1.000 across the systems. No system fabricates record identifiers
at a rate this check resolves, so the column establishes a lower bound on citation validity rather
than discriminating between systems. 

\paragraph{Claim-level precision tracks the harness, not model capability.} $P_{\mathrm{claim}}$
separates along harness families --- Codex 0.966, \texttt{opencode} 0.918, Gemini CLI 0.898, Claude
Code 0.875 --- yet is nearly flat within each. Substituting one model for another under a fixed
harness barely moves it: the five Codex systems agree to within 0.010 despite spanning that vendor's
mini-to-frontier range, and the six unrelated open-weight models on \texttt{opencode} agree to within
0.022. Across the sixteen systems the $P_{\mathrm{claim}}$ ranking shows no positive association with
the verdict-accuracy ranking of Table~\ref{tab:main750} (Spearman $\rho=-0.29$). This is the mirror
image of the harness ablation (Table~\ref{tab:ablation-harness}), where varying the harness at a fixed
model left verdict accuracy inside noise: whether a determination is traceable to retrieved evidence
is set largely by the scaffold that structures retrieval and report generation, whereas whether it is
correct is set by the model. 

\paragraph{Citation precision and evidence coverage are weakly opposed.} Across the sixteen systems,
$P_{\mathrm{claim}}$ correlates negatively with $C_{\mathrm{finding}}$ ($r=-0.20$) and only weakly
with $R_{\mathrm{retrieval}}$ ($r=+0.23$), while the two coverage metrics correlate strongly with each
other ($r=+0.80$). Both extremes occur within a single family: Claude Code records the lowest
family-level $P_{\mathrm{claim}}$ (0.875) together with the highest $C_{\mathrm{finding}}$ (0.769),
and Opus 5 attains the highest coverage of any system (0.819). The inverse configuration also occurs,
GPT-5.4-mini ranking third on precision and second-lowest on coverage (0.667). The claim classifications
indicate the mechanism: ungrounded claims are predominantly \emph{unverifiable} rather than
\emph{contradicted}, at ratios between 2.6:1 for Gemini CLI and 5.1:1 for Claude Code. Systems that
report more of the required evidence are therefore not misreading the record but exceeding what their
retrieved evidence supports. Under-substantiation rather than contradiction is the dominant grounding
failure across all sixteen systems, which motivates reporting the two axes separately
(Section~\ref{sec:patient-grounding}): a single averaged grounding score would assign the same value
to a report that is faithful but incomplete and to one that is complete but inadequately sourced,
and the two are not equivalent to a reviewer auditing the determination.

\subsection{Policy Grounding}
\label{sec:policy-results}

Policy grounding is scored separately from patient-evidence grounding
(Section~\ref{sec:policy-grounding-metrics}): whether the agent cites the governing guidance correctly
and whether it applies the passages a domain expert would consider controlling. We report
two axes plus the effect of corpus access itself (Tables~\ref{tab:main750-policy}
and~\ref{tab:ablation-policy}). Policy citation correctness combines a deterministic existence check
(the citation resolves to a real corpus document and line span) with an LLM-judged support check, and
policy relevance is an LLM-judged score against an expert-specified governing-document set. Comparing
the policy-on and policy-off conditions isolates whether corpus access changes verdicts, evidence that
a decision is documentary rather than parametric recall.

\paragraph{Systems cite the governing policy correctly but incompletely.} Policy grounding on the
cohort (Table~\ref{tab:main750-policy}) separates two failure modes a single grounding score
would merge. Take GPT-5.4-mini and GPT-5.6-Luna, two arms complete at 750 and within 0.2 accuracy
points of each other. Citations almost always resolve (0.991 and 1.000), and precision of the cited
document set against the clinical board's governing list is high (0.800 and 0.825). Recall of that
set is roughly half (0.483 and 0.522): systems cite documents that genuinely govern, then omit about
half of the others that also govern. Since a determination resting on part of the applicable standard
can be right for the wrong reason, this is the policy-axis analogue of the trap gap, and a combined
score would hide it because high precision offsets low recall. That failure shape is the one finding
here that reproduces across all sixteen arms, because these are rates rather than counts and each is
computed within an arm: resolution runs 0.953--1.000 and document precision 0.757--0.907, while
document recall never exceeds 0.682 and falls as low as 0.410. Every system in the roster cites real,
relevant policy and omits much of the rest.

\paragraph{Fabricated citations dissociate sharply between systems of equal accuracy.} The same two
arms emit 27 and 2 fabricated policy citations, references resolving to no corpus document, a
thirteen-fold difference between systems scoring identically on accuracy. Citation support, the
LLM-judged check that a cited passage entails the claim attached to it, moves the same way (0.643
against 0.817). With the trap gap and the confidence margins, this is the third axis on which these
two arms are clearly distinguishable while their headline accuracy is not, and it is the one a
clinician auditing the report would notice first.

\begin{table}[htbp]
\centering
\caption{\textbf{Policy grounding on the complete 750-case cohort.} Resolution deterministically checks
that a citation names a real corpus document and valid line span, Support is LLM-judged, and
Doc-P$/$R$/$F1 compare the cited document set against the expert-specified governing set. Columns are
averaged over each arm's policy-expected runs (Resolution and Support only over runs with at least
one citation). Fabricated citations are counted separately.}
\label{tab:main750-policy}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{Resolve} & \textbf{Support} & \textbf{Doc-P} & \textbf{Doc-R} & \textbf{Doc-F1} \\
\midrule
\multicolumn{6}{@{}l}{\texttt{Claude Code}}\\
\quad Opus 5           & 0.999 & 0.571 & 0.757 & 0.682 & 0.695 \\
\quad Sonnet 5 & 0.992 & 0.591 & 0.834 & 0.453 & 0.613 \\
\addlinespace
\multicolumn{6}{@{}l}{\texttt{Codex}}\\
\quad GPT-5.6-Sol      & 1.000 & 0.753 & 0.827 & 0.589 & 0.653 \\
\quad GPT-5.6-Luna     & 1.000 & 0.817 & 0.825 & 0.522 & 0.609 \\
\quad GPT-5.5          & 1.000 & 0.750 & 0.791 & 0.592 & 0.648 \\
\quad GPT-5.4          & 1.000 & 0.631 & 0.767 & 0.548 & 0.616 \\
\quad GPT-5.4-mini     & 0.991 & 0.643 & 0.800 & 0.483 & 0.605 \\
\addlinespace
\multicolumn{6}{@{}l}{\texttt{Gemini CLI}}\\
\quad Gemini-3.6-Flash & 0.988 & 0.469 & 0.770 & 0.629 & 0.664 \\
\quad Gemini-3.5-Flash & 0.987 & 0.457 & 0.765 & 0.624 & 0.659 \\
\quad Gemini-3.1-Pro   & 1.000 & 0.666 & 0.784 & 0.410 & 0.550 \\
\addlinespace
\multicolumn{6}{@{}l}{\texttt{opencode} \textnormal{(open-weight models on the neutral harness)}}\\
\quad DeepSeek-V4-Pro & 0.995 & 0.622 & 0.866 & 0.520 & 0.662 \\
\quad DeepSeek-V4-Flash & 0.953 & 0.578 & 0.851 & 0.455 & 0.627 \\
\quad GLM-5.2 & 0.986 & 0.596 & 0.825 & 0.580 & 0.652 \\
\quad Qwen-3.7-Plus & 0.997 & 0.567 & 0.907 & 0.445 & 0.678 \\
\quad MiniMax-M3 & 0.978 & 0.468 & 0.818 & 0.535 & 0.640 \\
\quad Kimi-K2.7-Code & 0.998 & 0.619 & 0.824 & 0.538 & 0.644 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Ablations}
\label{sec:ablations}
The ablations run on the 142-case \emph{development subset} defined in Section~\ref{sec:eval_framework}. All sixteen arms are closed there at $n=142$, which is
what makes per-pair significance and repeated runs possible: of the $\binom{16}{2}=120$ pairs, 58 reach
$p<0.05$ under a two-sided exact McNemar test and 21 survive Holm correction, and accuracy spans
47.2--71.1 with a genuine three-way tie at the top. Every comparison below is paired against the
subset's own baseline and never against Table~\ref{tab:main750}, because the subset over-samples the
two rare \textit{Indeterminate} classes and its Claude arm is Opus 4.8 rather than the cohort's Opus 5,
so absolute scores do not carry across. GPT-5.6-Luna, for instance, reads 56.3 here against 64.5 on the
cohort. At a support of 12, one \textit{amb} case moves that column by 8.3 points, so \textit{amb}
figures indicate a direction and never a ranking. The abstention asymmetry of
Section~\ref{sec:main-results} reproduces here on a deliberately different label distribution, with
over-commitment exceeding over-abstention in \emph{all sixteen} arms (23.4--48.9\% against
5.3--29.5\%), which is what makes it a property of the systems rather than of the cohort's label mix.
Full sixteen-arm scores on the subset appear in Appendix~\ref{app:dev-leaderboard}, together with the
per-pair tests and per-class breakdowns.

\paragraph{Withholding the policy corpus degrades deferral, not verdict-reaching.} With the corpus
withheld and nothing else changed, accuracy moves \emph{inconsistently}: three of five arms fall by
3.5--4.3 points and two rise by 0.7--4.2, and a two-sided exact McNemar test on the paired cases
separates \emph{no} arm's shift from zero ($p=0.26$--$1.00$). Corpus access is therefore not worth a
fixed number of points, and these deltas do not order the arms. Recall on \textit{amb} moves
consistently on four of the five, falling on three and unchanged on one, which is what one expects if
the corpus is what tells an agent a governing standard exists and does not settle the case. The
policy-enabled condition remains canonical. This is an ablation of the environment, not an alternative
configuration (Table~\ref{tab:ablation-policy}).

\begin{table}[htbp]
\centering
\caption{\textbf{Policy-corpus ablation.} \emph{Paired per case, web search disabled in both
conditions.} $\Delta$ is off $-$ on, so negative means withholding the corpus hurt. $p$ is a two-sided
exact McNemar test on the accuracy $\Delta$ over the paired cases (discordant counts 13--26 per arm,
too small for the $\chi^2$ approximation), and no arm's accuracy $\Delta$ is distinguishable from zero
($p=0.26$--$1.00$), so the deltas do not order the arms. \textit{amb} recall is against a support of
12, so one case is 8.3 points: read direction, not magnitude. The policy-off side is complete at 142 on
all five arms. Gemini-3.1-Pro carries 3 policy-on stub runs (no deliverable, no grade) dropped from
both sides, so its row is paired over 139 cases and every other over 142.}
\label{tab:ablation-policy}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{Accuracy}} & \multicolumn{3}{c}{\textbf{Recall \textit{amb} \%}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-8}
\textbf{Model (harness)} & on & off & $\Delta$ & $p$ & on & off & $\Delta$ \\
\midrule
GPT-5.6-Sol (Codex)         & 71.1 & 71.8 & $+0.7$ & 1.00 & 50.0 & 41.7 & $-8.3$ \\
GPT-5.5 (Codex)             & 71.1 & 66.9 & $-4.2$ & 0.26 & 50.0 & 41.7 & $-8.3$ \\
Gemini-3.1-Pro (Gemini CLI) & 72.7 & 68.3 & $-4.3$ & 0.33 & 33.3 & 41.7 & $+8.3$ \\
GPT-5.6-Luna (Codex)        & 56.3 & 60.6 & $+4.2$ & 0.29 & 58.3 & 50.0 & $-8.3$ \\
Opus 4.8 (Claude Code)      & 69.7 & 66.2 & $-3.5$ & 0.36 & 50.0 & 50.0 & $\pm0.0$ \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Single-attempt accuracy overstates consistent correctness, and the inconsistency is
systematic.} Across three independent attempts, pass\textasciicircum{}3 falls 8.2--12.7 points below
avg@3, and the residual agreement is on the \emph{same wrong} verdict, 16.9--26.8 points, and for
GPT-5.6-Luna 37\% of the cases on which it agreed with itself. Run-to-run variation is small next to
that shortfall, with the standard deviation of accuracy across the three attempts at 1.1--3.2 points,
so the gap is not attempt noise. High self-consistency is therefore not evidence of reliability: these
systems are mostly \emph{stably} wrong rather than randomly wrong, so repeating a query will not
surface the error. Reliability is also worst exactly where the benchmark is hardest, as \emph{every}
arm's lowest pass\textasciicircum{}3 falls on an \textit{Indeterminate} class
(Table~\ref{tab:passk-perclass}).

\begin{table}[htbp]
\centering
\caption{\textbf{Repeated-run reliability, development subset.} \emph{Three independent attempts.}
$n_{\mathrm{com}}$ counts cases gradeable in \emph{every} attempt, since pass\textasciicircum{}3 is
undefined otherwise, and all five arms cover the full subset. \emph{SD} is the sample standard
deviation (2 degrees of freedom) of the three per-attempt accuracies. \emph{Spread} is
pass@3 $-$ pass\textasciicircum{}3, the share of cases correct in some attempts but not others.
\emph{Overst.} is avg@3 $-$ pass\textasciicircum{}3. \emph{Agree} is the share on which all three
attempts returned the same verdict, and \emph{Agree-wr} the part of that on an \emph{incorrect}
verdict, so \textit{Agree} $=$ pass\textasciicircum{}3 $+$ \textit{Agree-wr} by construction (printed
values can differ by $0.1$ from independent rounding). pass\textasciicircum{}3 and pass@3 are
set-valued over the intersection and have no across-attempt SD, and their binomial standard error at
$n=142$ (4.1--4.2 and 3.3--3.9 points) is comparable to the range of \emph{Overst.}, so the columns
support the aggregate claim rather than an ordering of arms. avg@3 is not comparable with the Acc
column of Table~\ref{tab:dev-leaderboard} because the denominators differ. The eleven single-attempt
arms are omitted.}
\label{tab:passk}
\small
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lcccccccrr}
\toprule
\textbf{Model (harness)} & $n_{\mathrm{com}}$ & \textbf{avg@3} & \textbf{SD} & \textbf{pass\textasciicircum{}3} & \textbf{pass@3} & \textbf{Spread} & \textbf{Overst.} & \textbf{Agree} & \textbf{Agree-wr} \\
\midrule
Opus 4.8 (Claude Code)         & 142 & \textbf{70.9} & 1.5 & \textbf{62.0} & 79.6 & 17.6 & \phantom{0}8.9 & \textbf{79.6} & 17.6 \\
\addlinespace
GPT-5.5 (Codex)                & 142 & 70.2 & 1.1 & \textbf{62.0} & 78.2 & \textbf{16.2} & \textbf{\phantom{0}8.2} & \textbf{79.6} & 17.6 \\
GPT-5.6-Sol (Codex)            & 142 & 68.3 & 3.2 & 57.0 & 78.2 & 21.1 & 11.3 & 76.8 & 19.7 \\
GPT-5.6-Luna (Codex)           & 142 & 57.7 & 1.9 & 46.5 & 66.9 & 20.4 & 11.3 & 73.2 & 26.8 \\
\addlinespace
Gemini-3.1-Pro (Gemini CLI)    & 142 & 69.7 & 2.4 & 57.0 & \textbf{81.0} & 23.9 & 12.7 & 73.9 & 16.9 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Per-class repeated-run reliability.} \emph{Development subset, three attempts.}
pass\textasciicircum{}3 is the share of a class's cases correct in \emph{all three} attempts, pass@3
the share correct in \emph{at least one}, and $n$ is the per-class count gradeable in all three, so the
four supports sum to the arm's $n_{\mathrm{com}}$ in Table~\ref{tab:passk}. \emph{SD} is the sample
standard deviation of that class's accuracy across the three attempts (2 degrees of freedom), not of
pass\textasciicircum{}3 or pass@3, which are set-valued. \textbf{The \textsc{amb} support is 12 cases,
where one case moves a cell by 8.3 points, so that column indicates a direction and must not be read as
a ranking.} The per-case binomial standard error is about 6.9 points at $n=50$, 7.3 at $n=45$, 8.3 at
$n=35$ and 14.1 at $n=12$, so no single cell separates arms. All five arms cover the full subset
(\textsc{yes} 50, \textsc{no} 45, \textsc{lack} 35, \textsc{amb} 12).}
\label{tab:passk-perclass}
\begin{tabular}{lcccccccccccccccc}
\toprule
& \multicolumn{4}{c}{\textsc{yes}} & \multicolumn{4}{c}{\textsc{no}}
& \multicolumn{4}{c}{\textsc{lack}} & \multicolumn{4}{c}{\textsc{amb}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
\textbf{Model (harness)} & $n$ & \^{}3 & @3 & SD & $n$ & \^{}3 & @3 & SD & $n$ & \^{}3 & @3 & SD & $n$ & \^{}3 & @3 & SD \\
\midrule
Opus 4.8 (Claude Code)       & 50 & \textbf{74.0} & \textbf{94.0} & 1.2 & 45 & 57.8 & \textbf{82.2} & 3.4 & 35 & 54.3 & 60.0 & 0.0 & 12 & \textbf{50.0} & \textbf{66.7} & 4.8 \\
\addlinespace
GPT-5.5 (Codex)              & 50 & 64.0 & 86.0 & 2.0 & 45 & \textbf{71.1} & 80.0 & 2.6 & 35 & 54.3 & 74.3 & 1.6 & 12 & 41.7 & 50.0 & 4.8 \\
GPT-5.6-Sol (Codex)          & 50 & 62.0 & 84.0 & 3.5 & 45 & 60.0 & \textbf{82.2} & 6.7 & 35 & 51.4 & 74.3 & 1.6 & 12 & 41.7 & 50.0 & 4.8 \\
GPT-5.6-Luna (Codex)         & 50 & 48.0 & 64.0 & 4.6 & 45 & 48.9 & 71.1 & 2.2 & 35 & 42.9 & 68.6 & 1.6 & 12 & 41.7 & 58.3 & 8.3 \\
\addlinespace
Gemini-3.1-Pro (Gemini CLI)  & 50 & 60.0 & 86.0 & 4.2 & 45 & 62.2 & \textbf{82.2} & 6.8 & 35 & \textbf{60.0} & \textbf{82.9} & 2.9 & 12 & 16.7 & 50.0 & 4.8 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Prompt interventions for abstention.} We tested four case-agnostic interventions against an
unmodified baseline: a post-retrieval abstention decision-gate, a structured answer format separating
claims-and-evidence from the verdict, a self-critique pass, and an underspecification check. None
reliably lifts abstention. The gate and the structured format both \emph{lower} \textit{lack} recall,
self-critique nudges the stronger model's accuracy while committing more often, and the
underspecification check, the one positive, raises the weaker model's \textit{lack} recall at flat
accuracy but does not transfer to the stronger model. The effects are small, mixed and model-dependent,
which is itself evidence that under-abstention is a genuine benchmark axis rather than a shallow
prompting artefact. These four ran on an earlier build of the case prompts and grading stack, so their
absolute numbers are not comparable with the tables here. We report the direction and withhold the
table rather than invite a comparison the data does not support.

\paragraph{Harness versus model.} Holding the model fixed and varying the harness across three
model-agnostic harnesses moves accuracy little: the spread is smaller than the across-model spread
within a single harness, and no pairwise difference approaches significance on a paired test
(Table~\ref{tab:ablation-harness}). What separates the harnesses is cost, as median completion tokens
differ severalfold for accuracy differences inside noise, so at a fixed model the harness is an
efficiency choice more than a capability one.

\begin{table}[htbp]
\centering
\caption{\textbf{At a fixed model, the harness is not the dominant term.} DeepSeek-V4-Pro under three model-agnostic harnesses over the same 142 development cases. Accuracy spans 5.6 points --- no pair exceeding 1.0\,SE$_d$ (exact McNemar $p\geq0.17$) and well inside the across-model spread within one harness --- while median completion tokens differ 4.2-fold. Process adherence separates them no further (worst pair 1.5\,SE$_d$).}
\label{tab:ablation-harness}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lcccccc}
\toprule
\textbf{Harness} & \textbf{Acc \%} & $\Delta$ & $p$ & \textbf{Proc \%} & \textbf{Turns} & \textbf{Comp.\ tok} \\
\midrule
  \texttt{opencode} & 66.2\,$\pm$\,4.0 & --- & --- & 68.6\,$\pm$\,2.3 & 13 & 4\,874 \\
  \texttt{qwen-coder} & 60.6\,$\pm$\,4.1 & $-5.6$ & 0.17 & 63.6\,$\pm$\,2.4 & 15 & 9\,357 \\
  \texttt{mini-swe-agent} & 64.8\,$\pm$\,4.0 & $-1.4$ & 0.86 & 67.6\,$\pm$\,2.2 & 48 & 20\,370 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Test-time compute (reasoning effort).} A default-versus-\texttt{high} contrast measures
nothing here, for two separate reasons. The Codex adapter sets \texttt{reasoning\_effort} to
\texttt{high} unless told otherwise, so those two conditions are one. And Claude Code, which sets no
default, already runs at the top of the range: over the cases both arms completed, the median
\emph{within-case} ratio of default to \texttt{high} completion tokens is 1.000. We therefore compare
three explicit levels on one model over the same 142 cases (Table~\ref{tab:ablation-effort}). Compute
rises substantially, 39\% from \texttt{low} to \texttt{medium} and 74\% end to end, as median
within-case ratios rather than ratios of medians. Quality does not follow. Accuracy spans 1.4 points
with every pairwise difference inside 0.3 standard errors and both exact McNemar tests far from
significance, and process adherence separates the levels no further. Additional test-time compute buys
neither better verdicts nor a better-documented method, which is what one expects if the binding
constraint is retrieval elicitation and label discrimination rather than reasoning depth. One limit is
that the trajectories expose no reasoning-token count, so completion tokens are the only available
compute proxy and we cannot say \emph{where} the extra compute was spent.

\begin{table}[htbp]
\centering
\caption{\textbf{Test-time compute buys compute, not accuracy.} Opus 4.8 on Claude Code, three explicit reasoning-effort levels over the same 142 development cases. Completion tokens rise 41\% to \texttt{medium} and 74\% end to end, but no pairwise accuracy difference exceeds 0.3\,SE$_d$ (exact McNemar $p\geq0.80$) and no process difference exceeds 1.2\,SE$_d$. Reasoning depth is not the binding constraint on this benchmark.}
\label{tab:ablation-effort}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lcccccc}
\toprule
\textbf{Effort} & \textbf{Acc \%} & $\Delta$ & $p$ & \textbf{Proc \%} & \textbf{Comp.\ tok} & $\Delta$\,tok \\
\midrule
  \texttt{low} & 67.6\,$\pm$\,3.9 & -- & -- & 64.5\,$\pm$\,2.3 & 7\,030 & -- \\
  \texttt{medium} & 69.0\,$\pm$\,3.9 & $+1.4$ & 0.81 & 68.2\,$\pm$\,2.1 & 9\,776 & $+41$\% \\
  \texttt{high} & 69.0\,$\pm$\,3.9 & $+1.4$ & 0.80 & 68.5\,$\pm$\,2.4 & 12\,014 & $+74$\% \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Qualitative Analysis}
\label{sec:qualitative}
The aggregate scores hide a failure signature that trap-adjusted accuracy makes precise. A cirrhotic
patient is admitted with hepatic encephalopathy and moderate ascites, and no diagnostic paracentesis
appears anywhere in the admission, so spontaneous bacterial peritonitis can be neither confirmed nor
excluded and the reference verdict is \textit{Indeterminate: Lack of Data}. All five systems commit to
a definitive label, and four reach it through the same prohibited shortcut, asserting peritonitis
excluded with no ascitic-fluid result, the \textsc{must-not} criterion N4
(Table~\ref{tab:qual-he-precipitant}). The failure is not one of retrieval: every one of the five names
the missing paracentesis in its own report, and the process judge's justifications independently
describe the same mechanism, that the systems acknowledged the absent study and then treated the
diagnosis as effectively worked up. The sharpest case is GPT-5.6-Luna, which performs the deferral
reasoning correctly, earns the criterion rewarding escalation of an unresolved question, and avoids the
trap, yet still emits a definitive \textit{No}. Recognising an evidentiary gap is therefore not
sufficient. Here the failure occurs at label assignment, after the reasoning that should have prevented
it. This is why the benchmark scores the observable adjudication process separately from the verdict,
and why raw and trap-adjusted accuracy diverge.

\begin{table}[htbp]
\centering
\small
\caption{\textbf{Qualitative failure profile} (\texttt{he-precipitant-278ac1}). No diagnostic
paracentesis exists in the admission, so spontaneous bacterial peritonitis can be neither confirmed
nor excluded. Four of the five spring the same \textsc{must-not} criterion N4, ``Asserted SBP
excluded without an ascitic-fluid result''. GPT-5.6-Luna avoids the trap and earns the escalation
criterion, yet still commits.}
\label{tab:qual-he-precipitant}
\begin{tabular}{llcc}
\toprule
\textbf{System} & \textbf{Verdict} & \textbf{Stated conf.} & \textbf{Trap sprung} \\
\midrule
\emph{Gold} & \textit{Indeterminate: Lack of Data} & -- & -- \\
\midrule
Claude Sonnet 5 (Claude Code)   & Yes & \phantom{0}90\% & N4 \\
Claude Opus 4.8 (Claude Code)   & Yes & \phantom{0}90\% & N4 \\
GPT-5.5 (Codex)                 & Yes & \phantom{0}78\% & N4 \\
Gemini-3.5-Flash (Gemini CLI)   & Yes & 100\% & N4 \\
GPT-5.6-Luna (Codex)            & No  & \phantom{0}78\% & -- \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Benchmark Validation: Judge Reliability}
\label{sec:validation}
The process score and the reference labels both feed the rankings, so we validate each. The reference
labels are validated against independent clinician judgment in Section~\ref{sec:clinical-calibration}
(91\% agreement on the calibration sample, $\kappa=0.87$); here we validate the LLM-judged process and
policy scores.

\paragraph{Judge reliability and self-consistency.} The process rubric is LLM-adjudicated,
so we measure whether the grade is stable across judges rather than assuming it. A five-judge
panel grades every trajectory over the full rubric with three replicates each. We report
inter-judge agreement primarily as the mean pairwise disagreement. It flags 16\% of
criteria as contested, with the judges self-consistent across replicates and statistically
interchangeable on the aggregate score (companion Fleiss' $\kappa \approx 0.65$). The
most-contested criteria (for example, a hidden antibiotic de-escalation window and an
era-dependent heart-failure therapy) are exactly the cases an independent expert audit flagged
as under-specified, so judge disagreement acts as an automatic detector of ambiguous criteria,
which are then routed back for expert revision. This supports reporting the process score as a
real metric rather than judge noise.

\paragraph{Grounding-metric determinism and judge reliability.} The four patient-evidence grounding
metrics divide by construction, and each is validated according to what it produces.
$P_{\mathrm{record}}$ and $R_{\mathrm{retrieval}}$ are computed by rule from the trace and involve no
judge at all: recomputing them over a complete 750-case run returns every per-run value unchanged.
The other two are LLM-judged, so we grade the same reports twice and compare the two passes.
$C_{\mathrm{finding}}$ asks the judge one covered$/$not-covered question per rubric category. Because
those categories are fixed in advance, the two passes can be compared question by question: over 200
reports, 50 per harness family, they agree on 97.6\% of 1{,}310 category decisions (Cohen's
$\kappa=0.94$), 175 of the 200 reports receive an identical score, and no family average moves by
more than 0.005. $P_{\mathrm{claim}}$ gives no such fixed question list, because the judge must first
break the report into atomic claims and it does not divide it the same way twice; there is nothing to
align, so we report how far the score itself moves, which is at most 0.02 and in no consistent
direction. We therefore treat the two rule-based metrics as exact, $C_{\mathrm{finding}}$ as
reproducible, and differences of 0.02 or less on $P_{\mathrm{claim}}$ as noise.

\paragraph{Policy-judge reliability and self-consistency.} The policy rubric is mostly deterministic:
citation existence and policy relevance are computed by rule, while only citation support requires LLM
judgement. Accordingly, the two rule-based items achieve perfect agreement ($\kappa=1.0$) with no
replicate variation, and the remaining LLM judgement is stable across judges (companion Fleiss'
$\kappa\approx0.86$, within-judge noise 0.023--0.025 on a $0,1$ scale). The production judge is
therefore representative rather than unusually strict or lenient. The residual variation is systematic:
judges sometimes under-credit near-verbatim citations, making citation-correctness scores conservative
lower bounds, and we find no evidence of own-family favouritism. By defining policy relevance through
expert gold documents rather than LLM judgement, we remove a major source of ambiguity at the
rubric-design stage. This supports treating the policy score as a meaningful metric rather than judge
noise.

==> OLDresult_old.tex <==
\section{Experimental Results}
\label{sec:experiments}

We evaluate autonomous systems along two axes: a leaderboard of production agent harnesses, each
running its native frontier model, and a controlled comparison that fixes a single model-agnostic
harness and varies only the model. Using the metrics of Section~\ref{sec:eval}, the experiments are
designed to expose three dissociations the benchmark targets: (i) raw accuracy overstates sound
clinical reasoning, since a verdict can be reached through a prohibited shortcut; (ii) systems
systematically under-abstain, committing to a definitive answer where the record warrants deferral;
and (iii) accuracy exceeds grounding fidelity, as models reach the right verdict without citing the
evidence that justifies it.

\subsection{Experimental Setup}
\label{sec:eval}
\label{sec:exp-setup}

\paragraph{Harnesses.} We run four agent harnesses. \texttt{Claude Code}, \texttt{Codex} and
\texttt{Gemini CLI} are production agent CLIs, each locked to its own vendor model family and driving
the benchmark tools through a native tool-calling loop, so they represent how each model is actually
deployed. \texttt{opencode} is a model-agnostic open-source harness that connects to the same MIMIC
tool server as the others; because it can drive any model, it serves as the fixed neutral harness for
the model-comparison axis, isolating the model's contribution from the harness's. All four run with
web search and fetch disabled, so every system answers from the in-environment patient record and
policy corpus alone --- a frozen-corpus condition enforced by a deny-by-default egress allowlist
rather than by instruction. MIMIC data is reached only through a credential-isolated tool server, so
no system can bypass the governed tools to read raw records.

\paragraph{Models.} Table~\ref{tab:exp-matrix} lists the sixteen systems evaluated. The native
leaderboard pairs each harness with its frontier models. The model-comparison axis runs a set of
open-weight models on the neutral \texttt{opencode} harness, isolating the model from the harness.
Running the vendor models on \texttt{opencode} as well, for a fully harness-controlled comparison, is
planned. Medical-specialized models are excluded from the agentic leaderboard because they cannot
drive a multi-step tool-calling loop: under an agentic harness they would score near zero from
harness incompatibility rather than clinical weakness. Where relevant we report them separately as a
single-turn probe.

\begin{table}[htbp]
\centering
\small
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2}
\caption{\textbf{Systems evaluated in CliniCARE-Bench.} Native leaderboard
(each harness on its own frontier model) and the controlled model comparison
(a common model set on the neutral \texttt{opencode} harness). All sixteen appear in every
leaderboard table.}
\label{tab:exp-matrix}
\begin{tabularx}{\linewidth}{@{}lX@{}}
\toprule
\textbf{Harness} & \textbf{Models} \\
\midrule
\multicolumn{2}{@{}l}{\textit{Native leaderboard: each harness on its own frontier model}} \\
\addlinespace[2pt]
\texttt{Claude Code} & Claude Opus 5; Claude Sonnet 5 \\
\texttt{Codex}       & GPT-5.6 Sol; GPT-5.6 Luna; GPT-5.5; GPT-5.4; GPT-5.4-mini \\
\texttt{Gemini CLI}  & Gemini 3.1 Pro; Gemini 3.5 Flash; Gemini 3.6 Flash \\
\addlinespace[6pt]
\midrule
\multicolumn{2}{@{}l}{\textit{Controlled comparison: open-weight models on one neutral harness}} \\
\addlinespace[2pt]
\texttt{opencode} & DeepSeek V4 Pro; DeepSeek V4 Flash; Qwen 3.7 Plus; GLM 5.2;
                    MiniMax M3; Kimi K2.7 Code \\
\bottomrule
\end{tabularx}
\end{table}

\paragraph{cases and verdict classes.} The cohort is 25 clinical scenarios $\times$ 30 patients
$=750$ cases. Each case asks a single adjudication question against one patient's longitudinal record
and the governing policy corpus, and the answer is one of four classes: \textit{Yes}
(\texttt{YES}), \textit{No} (\texttt{NO}), \textit{Indeterminate: Lack of Data}
(\texttt{INDETERMINATE\_LACK\_OF\_DATA}) and \textit{Indeterminate: Medically Ambiguous}
(\texttt{INDETERMINATE\_MEDICAL\_AMBIGUITY}). The two deferral classes are distinct on purpose:
\textit{lack} means the record does not contain the study or observation that would settle the
question, whereas \textit{amb} means the record is complete and the governing standard still does not
determine an answer. Throughout we abbreviate them as \textit{lack} and \textit{amb}. The verdict is
scored deterministically by exact four-class match; there is no partial credit and no
free-text equivalence judgement.

\paragraph{Development subset.} A frozen subset of 142 of the 750 cases, built by taking up to two
patients per verdict class from each scenario, so it over-samples the two rare \textit{Indeterminate}
classes (gold supports \textit{Yes}~50, \textit{No}~45, \textit{lack}~35, \textit{amb}~12) and an
intervention aimed at deferral can move a measurable number of cases. Its case ids are pinned and form a
verified subset of the 750 with byte-identical rubrics, and all sixteen arms have graded all 142, so it
is closed --- which is why per-pair significance and repeated-run reliability are reported there rather
than on the cohort. Its Claude arm is Opus 4.8, not the cohort's Opus 5, so those rows are different
systems. Appendix~\ref{app:dev-subset} carries the detail.

\paragraph{Metrics.} Verdict quality is four-class accuracy and macro-F1 over the four classes, the
latter weighting the two rare \textit{Indeterminate} classes equally with \textit{Yes} and
\textit{No}. Accuracy is reported per trial (micro); because every scenario holds exactly 30
patients, the scenario-macro average coincides with it exactly on an arm complete at 750 but not on a
partial one, and we say which we use wherever it matters. A \emph{trap} is a \textsc{must-not}
criterion in the case's rubric --- an inferential shortcut a clinician reviewing the work would
reject outright. \emph{Trap-adjusted accuracy} counts a trial correct only when the verdict is right
\emph{and} no \textsc{must-not} criterion was violated. The \emph{trap gap} is raw accuracy
\emph{restricted to trials that produced a report} minus trap-adjusted accuracy; it is deliberately
not overall accuracy minus trap-adjusted accuracy, because those two are taken over different
denominators and their difference is not interpretable. Abstention is measured directionally rather
than as a single hedging rate: \emph{over-commitment} is returning a definitive verdict where the
reference verdict is \textit{Indeterminate}, and \emph{over-abstention} is deferring where the record
supports a determination, each taken over that arm's own gold supports (47 deferral and 95 definitive
cases on the development subset). \emph{Process adherence} is an LLM-judged score over the rubric's
observable investigation steps, independent of the verdict; the judge is pinned to
\texttt{openai/gpt-5.5}. Calibration is expected calibration error over the confidence each report
states, defined at Eq.~\ref{eq:ece} where it is first used. Evidence grounding and policy grounding
each carry their own axes and are defined where they are reported
(Sections~\ref{sec:grounding-results} and~\ref{sec:policy-results}). Repeated-run reliability uses
avg@3 (mean accuracy across three independent attempts), pass\textasciicircum{}3 (correct in
\emph{every} attempt), pass@3 (correct in \emph{at least one}) and verdict agreement (all three
attempts returning the same verdict, correct or not). Cost and efficiency are per-trial turns, typed
tool calls, work-tokens (prompt $-$ cached $+$ completion) and USD/trial, the last comparable only
within a harness family.




\subsection{Results}
\label{sec:main-results}

Every system is run on all 750 cases at a single attempt against the silver reference labels.
Table~\ref{tab:main750} reports the full leaderboard: verdict accuracy and macro-F1, trap-adjusted
accuracy and the gap it opens, process adherence, the two directional abstention errors, calibration,
and per-trial cost. Two things are worth fixing in mind before reading it. The \emph{Gap} column is
raw accuracy minus trap-adjusted accuracy \emph{over report-present trials only}, so it is not the
difference of the two columns beside it. And the cost columns are measured on two different instruments: harness-reported for the vendor
CLIs, but computed from measured tokens for the \texttt{opencode} arms, which report neither a cost
field nor a cached-token count. Those six are therefore given as ranges rather than point estimates.

\begin{table}[htbp]
\centering
\caption{\textbf{Primary leaderboard} Every arm was run and scored on all 750 cases. \emph{Over-com} and \emph{Over-abs} are the directional abstention
errors of Section~\ref{sec:eval}, each taken over that arm's own gold deferral and definitive
supports. \emph{Proc \%} is the LLM-judged process-rubric score. The four cost columns are per-trial
medians (work-tokens $=$ prompt $-$ cached $+$ completion) except USD/trial, which is a mean excluding
judge spend; totals are not reported, since the per-trial figure is the comparable unit. The six \texttt{opencode} arms show a \emph{range} for work-tokens and USD because the
\texttt{opencode} adapter does not report a cached-token count --- the same Fireworks-served model reports
one normally under a different harness, so this is an instrumentation gap in the adapter and not a
property of the serving path: the upper end assumes no prompt caching, the lower end applies the 0.90 cache rate measured across the ten arms that do report it (range 0.84--0.93) at each model's own cache-read price. The true value lies between; the vendor arms are harness-reported with caching already netted out. \emph{Acc} is the
per-trial (micro) average, which coincides with the scenario-macro average only on an arm complete at
750. Turns and tool calls are comparable only within a harness family and work-tokens only within a
serving path; tool calls count typed MCP calls only, so a harness reaching the tool server through a
shell is undercounted.}
\label{tab:main750}
\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccc}
\toprule
 & & \multicolumn{5}{c}{\textbf{Quality}} & \multicolumn{3}{c}{\textbf{Abstention \& calibration}} & \multicolumn{4}{c}{\textbf{Cost \& efficiency}} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-10}\cmidrule(lr){11-14}
\textbf{Model (harness)} & \textbf{n} & \textbf{Acc} & \textbf{Macro-F1} & \textbf{Trap-adj} & \textbf{Gap} & \textbf{Proc \%} & \textbf{Over-com} & \textbf{Over-abs} & \textbf{ECE} & \textbf{Turns} & \textbf{Tools} & \textbf{Work-tok} & \textbf{USD/trial} \\
\midrule
% <<<AUTOROWS750:tab:main750>>>
Opus 5 (Claude Code)           & 750 & \textbf{72.3} & 0.633 & 62.9 & 9.3 & 80.2 & 29.2 & 15.2 & 0.098 & 17 & 28 & 130.2k & 2.05 \\
Sonnet 5 (Claude Code)         & 750 & 70.8 & 0.603 & 59.5 & 11.3 & 69.5 & 28.5 & 16.3 & 0.072 & 13 & 22 & 90.2k & 0.94 \\
\addlinespace
GPT-5.6-Sol (Codex)            & 750 & 70.8 & 0.619 & 64.1 & 6.7 & 79.6 & 26.9 & 16.6 & 0.217 & 22 & 16 & 90.5k & 1.11 \\
GPT-5.6-Luna (Codex)           & 750 & 64.5 & 0.552 & 57.2 & 7.3 & 75.0 & 36.9 & 20.5 & 0.250 & 22 & 18 & 97.5k & 0.25 \\
GPT-5.5 (Codex)                & 750 & 71.7 & 0.639 & 65.6 & 6.1 & 77.0 & 32.3 & 14.5 & 0.119 & 18 & 49 & 126.2k & 1.50 \\
GPT-5.4 (Codex)                & 750 & 68.9 & 0.612 & 61.1 & 7.9 & 75.7 & 33.8 & 15.3 & 0.174 & 21 & 52 & 110.7k & 0.72 \\
GPT-5.4-mini (Codex)           & 750 & 64.7 & 0.535 & 54.3 & 10.4 & 66.8 & 50.8 & 16.1 & 0.231 & 24 & 44 & 84.1k & 0.20 \\
\addlinespace
Gemini-3.6-Flash (Gemini CLI)  & 750 & 70.5 & 0.608 & 56.4 & 14.1 & 72.3 & 35.4 & 11.6 & 0.274 & 62 & 36 & 384.5k & 1.14 \\
Gemini-3.5-Flash (Gemini CLI)  & 750 & 70.0 & 0.590 & 57.6 & 12.4 & 72.0 & 38.5 & 11.8 & 0.279 & 62 & 36 & 387.8k & 1.16 \\
Gemini-3.1-Pro (Gemini CLI)    & 750 & 70.3 & 0.626 & 54.4 & 15.9 & 58.6 & 18.5 & 15.5 & 0.279 & 42 & 23 & 206.7k & 1.02 \\
\addlinespace
DeepSeek-V4-Pro (opencode)     & 750 & 63.1 & 0.547 & 51.6 & 11.5 & 65.3 & 31.5 & 21.0 & 0.209 & 14 & 39 & 59--552k & 0.20--1.08 \\
DeepSeek-V4-Flash (opencode)   & 750 & 63.3 & 0.514 & 52.5 & 10.8 & 63.6 & 44.6 & 20.5 & 0.252 & 15 & 46 & 79--747k & 0.04--0.12 \\
GLM-5.2 (opencode)             & 750 & 62.9 & 0.542 & 53.5 & 9.5 & 67.2 & 33.8 & 24.5 & 0.243 & 13 & 29 & 57--528k & 0.21--0.97 \\
Qwen-3.7-Plus (opencode)       & 750 & 58.1 & 0.492 & 46.8 & 11.3 & 59.8 & 36.2 & 27.6 & 0.200 & 11 & 28 & 45--415k & 0.06--0.19 \\
MiniMax-M3 (opencode)          & 750 & 59.7 & 0.492 & 47.3 & 12.4 & 67.0 & 50.8 & 22.7 & 0.198 & 22 & 46 & 106--1001k & 0.13--0.42 \\
Kimi-K2.7-Code (opencode)      & 750 & 52.7 & 0.427 & 41.5 & 11.2 & 61.4 & 45.4 & 29.4 & 0.199 & 18 & 49 & 106--1032k & 0.73--2.50 \\
% <<<END750:tab:main750>>>
\bottomrule
\end{tabular}%
}
\end{table}

\paragraph{No system resolves the cohort, and the loss concentrates in the rare classes.} Accuracy
spans 52.7 to 72.3 and macro-F1 0.427 to 0.639 (Table~\ref{tab:main750}): the strongest arm resolves
just under three-quarters of its graded cases and the weakest barely more than half. Macro-F1 trails accuracy
in every arm, because it weights the two rare \textit{Indeterminate} classes equally with \textit{Yes}
and \textit{No}, so the loss is concentrated where deferral must be recognised. Accuracy forms a
continuum rather than tiers: the three weakest arms (Kimi-K2.7-Code 52.7, Qwen-3.7-Plus 58.1,
MiniMax-M3 59.7) sit below the rest, but only 3.2 points separate the third weakest from the fourth, so
we read the ordering as a gradient and not as a set of separable groups. Differences of a few points
anywhere in the table are not separable at these $n$ and we do not treat them as a ranking.

\paragraph{Trap-adjusted accuracy: what it is, and why it reorders the field.} A \emph{trap} is a
\textsc{must-not} criterion in the case's rubric --- an inferential shortcut a clinician reviewing the
work would reject outright, such as reading acute kidney injury off a billing code, asserting contrast
causation from temporal proximity alone, or citing a policy document that does not exist.
\emph{Trap-adjusted accuracy} counts a trial correct only when the verdict is right \emph{and} no
\textsc{must-not} criterion was violated; the \emph{Gap} column is raw minus trap-adjusted accuracy over
report-present trials, so it is the share of an arm's correct verdicts that were reached by a
forbidden route. Every system pays between 6.1 and 15.9 points (Table~\ref{tab:main750}), meaning that
between one in twelve and one in four of its correct answers does not survive inspection of how it was
reached.

The spread is the finding, not the magnitude. Were raw accuracy merely optimistic by a fixed margin,
the gap would be roughly constant and the ranking would survive the correction. It does not: GPT-5.5
loses 6.1 points while Gemini-3.1-Pro loses 15.9, so the correction reorders the field ---
Gemini-3.1-Pro reaches 70.3 raw accuracy, level with the leaders, and falls to 54.4 trap-adjusted,
below every Claude arm and every Codex arm bar GPT-5.4-mini, which it merely ties. Gemini-3.1-Pro is also the arm \emph{least} prone to over-commitment
(18.5\%), so springing traps and over-committing are distinct failures rather than two faces of the
same carelessness. This operationalises, on real longitudinal records, the
reasoning-versus-pattern-matching gap documented for medical LLMs
\cite{bedi2025fidelity, natmed2026robustness}: a correct label is not evidence of correct reasoning,
and only a trace-level audit of the investigation distinguishes the two. It is the concrete payoff of
scoring the observable adjudication process rather than the final answer alone.

\paragraph{Systems under-abstain: over-commitment exceeds over-abstention in every arm.} Measured
directionally (Table~\ref{tab:main750}), over-commitment --- returning a definitive verdict where the
reference verdict is \textit{Indeterminate} --- runs 18.5--50.8\% against over-abstention of
11.6--29.4\%, and \emph{all sixteen} systems over-commit at the higher rate. That the asymmetry holds
arm by arm rather than only in aggregate is what makes it a property of the systems rather than of the
label distribution, and it reproduces on the development subset (Section~\ref{sec:ablations}). The failure is not an unwillingness to
answer but an unwillingness to decline. The magnitude, not the direction, is what varies: GPT-5.4-mini
and MiniMax-M3 over-commit on exactly half of all deferral cases (50.8\% each) while
Gemini-3.1-Pro does so on 18.5\%.

\paragraph{The process score measures something the verdict does not.} Process adherence
(Table~\ref{tab:main750}) is judged against the rubric's observable investigation steps rather than
against the answer, and it separates arms that accuracy places together. Opus 5 scores 80.2 on process
against 72.3 accuracy, whereas Gemini-3.1-Pro reaches 70.3 accuracy on a process score of 58.6 --- the
same verdict quality reached through a materially less defensible investigation, which is the trap gap
(the \textbf{Gap} column of Table~\ref{tab:main750}) seen from the other side. Read against per-class precision
(Table~\ref{tab:main750-perclass}), the pattern is that precision on \textit{Yes} stays high while
precision on both \textit{Indeterminate} classes is far lower, so the deferrals systems do issue are
frequently issued on records that in fact settle the question. For a clinical deliverable this matters
more than the headline: a reader can audit a documented investigation and cannot audit a bare
verdict.

\begin{table}[htbp]
\centering
\caption{\textbf{Per-class F1, with precision and recall for the two \textit{Indeterminate}
classes.} The two rightmost cells read P\,$/$\,R. Denominators follow the cohort's natural label
distribution, not the development subset's balanced one, so cells are not comparable with
Table~\ref{tab:dev-perclass}.}
\label{tab:main750-perclass}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccccccc}
\toprule
 & & \multicolumn{4}{c}{\textbf{F1}} & \multicolumn{2}{c}{\textbf{Precision\,$/$\,Recall \%}} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-8}
\textbf{Model (harness)} & \textbf{n} & Yes & No & lack & amb & lack & amb \\
\midrule
% <<<AUTOROWS750:tab:main750-perclass>>>
Opus 5 (Claude Code)           & 750 & 0.818 & 0.738 & 0.506 & 0.473 & 41.2\,/\,65.3 & 50.0\,/\,44.8 \\
Sonnet 5 (Claude Code)         & 750 & 0.800 & 0.727 & 0.513 & 0.373 & 41.5\,/\,67.3 & 36.7\,/\,37.9 \\
\addlinespace
GPT-5.6-Sol (Codex)            & 750 & 0.795 & 0.734 & 0.515 & 0.433 & 41.3\,/\,68.3 & 41.9\,/\,44.8 \\
GPT-5.6-Luna (Codex)           & 750 & 0.740 & 0.694 & 0.402 & 0.373 & 32.5\,/\,52.5 & 30.4\,/\,48.3 \\
GPT-5.5 (Codex)                & 750 & 0.811 & 0.737 & 0.479 & 0.531 & 39.2\,/\,61.4 & 65.0\,/\,44.8 \\
GPT-5.4 (Codex)                & 750 & 0.774 & 0.717 & 0.465 & 0.491 & 38.6\,/\,58.4 & 50.0\,/\,48.3 \\
GPT-5.4-mini (Codex)           & 750 & 0.770 & 0.657 & 0.351 & 0.364 & 31.5\,/\,39.6 & 32.4\,/\,41.4 \\
\addlinespace
Gemini-3.6-Flash (Gemini CLI)  & 750 & 0.804 & 0.695 & 0.504 & 0.429 & 45.0\,/\,57.4 & 44.4\,/\,41.4 \\
Gemini-3.5-Flash (Gemini CLI)  & 750 & 0.794 & 0.703 & 0.487 & 0.377 & 43.4\,/\,55.4 & 41.7\,/\,34.5 \\
Gemini-3.1-Pro (Gemini CLI)    & 750 & 0.775 & 0.716 & 0.556 & 0.458 & 43.2\,/\,78.2 & 57.9\,/\,37.9 \\
\addlinespace
DeepSeek-V4-Pro (opencode)     & 750 & 0.746 & 0.642 & 0.409 & 0.392 & 31.0\,/\,60.4 & 45.5\,/\,34.5 \\
DeepSeek-V4-Flash (opencode)   & 750 & 0.774 & 0.635 & 0.357 & 0.292 & 27.9\,/\,49.5 & 36.8\,/\,24.1 \\
GLM-5.2 (opencode)             & 750 & 0.739 & 0.669 & 0.388 & 0.373 & 28.8\,/\,59.4 & 36.7\,/\,37.9 \\
Qwen-3.7-Plus (opencode)       & 750 & 0.702 & 0.631 & 0.333 & 0.303 & 24.4\,/\,52.5 & 27.0\,/\,34.5 \\
MiniMax-M3 (opencode)          & 750 & 0.719 & 0.646 & 0.287 & 0.317 & 22.8\,/\,38.6 & 29.4\,/\,34.5 \\
Kimi-K2.7-Code (opencode)      & 750 & 0.654 & 0.584 & 0.268 & 0.200 & 19.8\,/\,41.6 & 17.1\,/\,24.1 \\
% <<<END750:tab:main750-perclass>>>
\bottomrule
\end{tabular}
\end{table}

\paragraph{The leaderboard order does not hold scenario by scenario.} Resolved per
scenario (Table~\ref{tab:scenario-table}), the aggregate ordering of Table~\ref{tab:main750} survives
in only 65.5\% of the 3{,}000 arm-pair $\times$ scenario comparisons the grid contains, and thirteen of
the sixteen arms are the best system on at least one scenario --- including Kimi-K2.7-Code, last on the
leaderboard, which leads on \texttt{he-precipitant} and \texttt{overdose-disposition}. The ordering of
the averages is nevertheless stable (Spearman 0.94 between an arm's cohort accuracy and its mean
per-scenario rank), and the leader, GPT-5.5, still sits in the bottom quartile of arms on 4 of the 25
scenarios: the leaderboard is a statement about a case mix rather than about which system to trust on a
given clinical question. Difficulty is concentrated rather than diffuse --- cross-arm mean accuracy runs
from 91.7 on \texttt{discharge-audit} to 6.4 on \texttt{pe-workup}, and the five hardest scenarios
carry a third of all errors against the fifth that uniform difficulty implies --- and one scenario has
stopped separating systems altogether. On \texttt{pe-workup} no arm exceeds 24\%, and 342 of the 370
graded answers pooled over all sixteen arms are \textit{Indeterminate: Lack of Data} against a
reference that reads \textit{No} in 19 of its 30 cases. Sixteen independently built systems agreeing
that a record is insufficient is more readily explained by the reference labels for that scenario than
by a shared clinical blind spot, so \texttt{pe-workup} is queued for label adjudication; it is still
counted in every number reported here.

\begin{table}[htbp]
\centering
\caption{\textbf{Verdict accuracy (\%) per scenario, all 16 arms.} Rows are the 25 clinical
scenarios, sorted by the unweighted mean over arms given in the last column; the best cell in each row
is bold. A cell's denominator is that arm's graded trials for that scenario, now 30
across the row (minimum 12), so a single cell is a weaker estimate than a row or a column.
Column key: O5\,=\,Opus 5, S5\,=\,Sonnet 5, Sol\,=\,GPT-5.6-Sol, Luna\,=\,GPT-5.6-Luna, 5.5\,=\,GPT-5.5, 5.4\,=\,GPT-5.4, 5.4m\,=\,GPT-5.4-mini, G3.6\,=\,Gemini-3.6-Flash, G3.5\,=\,Gemini-3.5-Flash, G3.1\,=\,Gemini-3.1-Pro, D4P\,=\,DeepSeek-V4-Pro, D4F\,=\,DeepSeek-V4-Flash, GLM\,=\,GLM-5.2, Qwn\,=\,Qwen-3.7-Plus, MM3\,=\,MiniMax-M3, K2.7\,=\,Kimi-K2.7-Code.}
\label{tab:scenario-table}
\small
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccccc}
\toprule
\textbf{Scenario} & \textbf{O5} & \textbf{S5} & \textbf{Sol} & \textbf{Luna} & \textbf{5.5} & \textbf{5.4} & \textbf{5.4m} & \textbf{G3.6} & \textbf{G3.5} & \textbf{G3.1} & \textbf{D4P} & \textbf{D4F} & \textbf{GLM} & \textbf{Qwn} & \textbf{MM3} & \textbf{K2.7} & \textbf{Mean} \\
\midrule
% <<<SCENROWS:tab:scenario-table>>>
discharge-audit          & 97 & \textbf{100} & \textbf{100} & 97 & 89 & \textbf{100} & \textbf{100} & 92 & 96 & 92 & 90 & 70 & 87 & 90 & 89 & 80 & 91.7 \\
overdose-disposition     & 87 & 97 & 79 & 83 & 78 & 89 & 97 & 96 & 96 & 89 & 92 & 89 & 90 & 80 & 83 & \textbf{100} & 89.0 \\
eol-goal-concordance     & 93 & 93 & \textbf{100} & 97 & 88 & 95 & 93 & 86 & 88 & \textbf{100} & 79 & 84 & 80 & 77 & 73 & 76 & 87.7 \\
renal-trajectory         & 87 & 93 & 87 & 90 & 90 & 88 & \textbf{97} & 86 & 93 & 90 & 75 & 79 & 67 & 77 & 78 & 83 & 84.9 \\
transfusion-audit        & 87 & \textbf{90} & 86 & 83 & 83 & 84 & 87 & 89 & 89 & 89 & 86 & 80 & 77 & 73 & 86 & 65 & 83.3 \\
advanced-imaging         & 83 & 87 & \textbf{92} & 90 & \textbf{92} & 73 & 67 & 83 & 85 & 73 & 80 & 62 & 87 & 70 & 73 & 65 & 78.8 \\
hfref-gdmt               & 80 & 87 & \textbf{95} & 63 & 90 & 76 & 70 & 88 & 88 & 80 & 71 & 67 & 67 & 77 & 67 & 62 & 76.7 \\
post-ct-aki              & 83 & 83 & 81 & \textbf{93} & 87 & 67 & 80 & 79 & 83 & 72 & 57 & 68 & 53 & 66 & 86 & 56 & 74.6 \\
goals-of-care            & 93 & 90 & 95 & 60 & 95 & 83 & 57 & 67 & 74 & \textbf{96} & 75 & 62 & 80 & 70 & 50 & 45 & 74.6 \\
readmission-30d          & 70 & 73 & 73 & 87 & 87 & 85 & 70 & 83 & 79 & \textbf{92} & 63 & 65 & 73 & 67 & 62 & 44 & 73.3 \\
frequent-admitter        & 77 & 70 & \textbf{87} & 77 & 85 & 56 & 63 & 85 & 74 & 86 & 67 & 72 & 67 & 70 & 58 & 77 & 73.1 \\
med-reconciliation       & \textbf{87} & 70 & 84 & 57 & 59 & 62 & 53 & 63 & 69 & 86 & 80 & 65 & 73 & 50 & 56 & 60 & 67.1 \\
icu-delirium             & 67 & \textbf{83} & 56 & 63 & 50 & 62 & 67 & 77 & 70 & 62 & 55 & 55 & 67 & 60 & 54 & 62 & 63.0 \\
postop-complications     & 53 & 60 & 61 & 63 & 64 & 65 & 67 & \textbf{73} & 69 & 65 & 67 & 65 & 60 & 52 & 58 & 58 & 62.5 \\
dka-resolution           & 83 & 57 & 83 & 60 & \textbf{94} & 87 & 23 & 75 & 69 & 59 & 45 & 48 & 67 & 50 & 41 & 38 & 61.2 \\
sepsis-source-abx        & 77 & 60 & 59 & 43 & 73 & 64 & 73 & \textbf{79} & 67 & 71 & 46 & 67 & 67 & 47 & 59 & 26 & 61.0 \\
he-precipitant           & 57 & 53 & 71 & 57 & 67 & 54 & 66 & 67 & 62 & 61 & 69 & 68 & 57 & 50 & 45 & \textbf{74} & 61.0 \\
ams-workup               & 73 & 60 & \textbf{85} & 70 & 78 & 68 & 37 & 65 & 62 & 59 & 67 & 54 & 40 & 50 & 52 & 55 & 60.9 \\
hyperkalemia-management  & 60 & 57 & 68 & 60 & 69 & \textbf{72} & 67 & 50 & 57 & 54 & 61 & 52 & 70 & 50 & 52 & 57 & 59.7 \\
stroke-time-targets      & 67 & 57 & 52 & 50 & 68 & 58 & 53 & 67 & \textbf{70} & 54 & 57 & 67 & 47 & 48 & 59 & 40 & 57.1 \\
empiric-abx              & 70 & 73 & 58 & 57 & \textbf{74} & 65 & 63 & 59 & 61 & 63 & 61 & 48 & 50 & 39 & 30 & 27 & 56.1 \\
anticoag-reversal        & 67 & \textbf{70} & 56 & 40 & 44 & 50 & 47 & 63 & 67 & 56 & 57 & 68 & 57 & 52 & 57 & 45 & 55.8 \\
pneumonia-curb65         & 60 & 57 & 38 & 30 & 60 & 40 & \textbf{70} & 38 & 46 & 31 & 33 & 47 & 27 & 37 & 63 & 32 & 44.3 \\
sepsis-bundle            & 40 & 43 & 36 & 37 & 41 & 48 & 43 & 48 & 40 & 58 & \textbf{59} & 55 & 43 & 50 & 36 & 30 & 44.3 \\
pe-workup                & 10 & 7 & 0 & 7 & 0 & 0 & 7 & 4 & 4 & 12 & 0 & 12 & \textbf{23} & 3 & 14 & 0 & 6.4 \\
% <<<SCENEND:tab:scenario-table>>>
\bottomrule
\end{tabular}%
}
\end{table}

\paragraph{Calibration separates the systems more cleanly than accuracy does.} Every report states a
confidence, so we can ask whether that number carries information. Expected calibration error is the
bin-weighted deviation between stated confidence and realised accuracy,
\begin{equation}
\mathrm{ECE} \;=\; \sum_{b=1}^{B} \frac{|B_b|}{n}\,\bigl|\,\mathrm{conf}(B_b) - \mathrm{acc}(B_b)\,\bigr| ,
\label{eq:ece}
\end{equation}
over $B=10$ equal-width bins of stated confidence, where $\mathrm{conf}(B_b)$ and $\mathrm{acc}(B_b)$
are the mean stated confidence and realised accuracy in bin $b$. ECE spans 0.072--0.279 across the
sixteen arms --- a near-fourfold range on an axis accuracy cannot see --- and it does \emph{not} order
them the way accuracy does: the three best-calibrated are Sonnet 5 (0.072), Opus 5 (0.098) and GPT-5.5
(0.119), while the three worst are all Gemini CLI arms (0.274--0.279), which sit mid-field on accuracy.
For a report addressed to a clinician who cannot cheaply re-derive the answer, a confidence that does
not track correctness is arguably a more consequential defect than a few points of accuracy, and no
aggregate score above reveals it. One bound on cross-arm comparison: an arm emitting few distinct
confidence values populates few bins, so its ECE is not measuring quite the same thing.


\paragraph{Cost and efficiency diverge from accuracy, and from each other.} GPT-5.4-mini and
GPT-5.6-Luna land within 0.2 points of each other on accuracy and cost \$0.20 and \$0.25 per trial, so every per-dollar ratio favours the cheaper one.
What the extra spend buys is not correct verdicts but cleaner ones --- 2.9 more points of trap-adjusted
accuracy and 8.2 more of process adherence --- a purchase worth making in this domain and invisible to
any cost-per-accuracy-point ratio, which is why we do not tabulate one. Composition differs more than
total: GPT-5.4-mini issues a median 44 typed tool calls against GPT-5.6-Luna's 18, roughly
$2.4\times$ the retrieval traffic, while consuming \emph{fewer} work-tokens (84.1k against 97.5k). The
cheaper arm queries more and reasons less over what it retrieves, and it is also the arm with the wider
trap gap and the lower process score: more retrieval does not substitute for sound adjudication of what
was retrieved. Work-tokens are comparable only within a serving path: the \texttt{opencode} figures
are ranges rather than point values, because that path reports no cached-token count and the cache
correction has to be estimated.



\subsection{Grounding Fidelity}
\label{sec:grounding-results}
\george{TODO: Update with latest numbers on full split}
Grounding is where accuracy and reasoning most clearly diverge: a system can select the
correct verdict without citing the evidence that justifies it. Following the two axes of
Section~\ref{sec:eval}, we report grounding fidelity per system in Table~\ref{tab:grounding}.
Citation precision is reported at the record-identifier level ($P_{\mathrm{record}}$: a cited
patient, admission, order, or note must appear in what the agent retrieved) and the
clinical-claim level ($P_{\mathrm{claim}}$: each atomic assertion judged supported,
contradicted, or unverifiable, with entity and temporal attribution required); evidence
recall is reported as retrieval recall ($R_{\mathrm{retrieval}}$: the fraction of the case's
expert-specified required source tables the agent examined) and insight coverage
($C_{\mathrm{insight}}$: the fraction of required findings the report addresses).



\begin{table}[htbp]
\centering
\caption{Evidence grounding (full v3).}
\label{tab:grounding-v3-full750}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Model (harness)} & done & Record-ID & Claim-lvl & Retrieval & Insight-cov \\
\midrule
Opus 5 (Claude Code)              & 413 & 0.968 & 0.862 & 0.814 & \textbf{0.808} \\
Sonnet 5 (Claude Code)            & 402 & 0.977 & 0.818 & 0.822 & 0.691 \\
\addlinespace
GPT-5.6-Sol (Codex)               & 721 & \textbf{1.000} & 0.967 & 0.851 & 0.751 \\
GPT-5.5 (Codex)                   & 719 & 0.999 & 0.963 & 0.846 & 0.748 \\
GPT-5.4 (Codex)                   & 473 & 0.998 & 0.963 & 0.861 & 0.735 \\
GPT-5.4-mini (Codex)              & 750 & 0.997 & 0.964 & 0.812 & 0.667 \\
GPT-5.6-Luna (Codex)              & 750 & \textbf{1.000} & \textbf{0.968} & \textbf{0.866} & 0.725 \\
\addlinespace
Gemini-3.1-Pro (Gemini CLI)       & 326 & \textbf{1.000} & 0.917 & 0.686 & 0.612 \\
Gemini-3.5-Flash (Gemini CLI)     & 295 & 0.994 &       & 0.859 & 0.784 \\
Gemini-3.6-Flash (Gemini CLI)     & 288 & 0.992 &       & 0.853 & 0.796 \\
\addlinespace
DeepSeek-V4-Pro (opencode)        & 246 & 0.964 &       & 0.654 & 0.614 \\
DeepSeek-V4-Flash (opencode)      & 289 & 0.930 &       & 0.653 & 0.640 \\
GLM-5.2 (opencode)                & 342 & 0.914 &       & 0.565 & 0.601 \\
\addlinespace
Qwen-3.7-Plus (opencode)          & 232 & 0.968 &       & 0.504 & 0.496 \\
MiniMax-M3 (opencode)             & 192 & 0.858 &       & 0.452 & 0.552 \\
Kimi-K2.7-Code (opencode)         & 165 & 0.921 &       & 0.492 & 0.495 \\
\bottomrule
\end{tabular}
\end{table}

\newpage
\subsection{Policy Grounding}
\label{sec:policy-results}

Policy grounding is scored separately from patient-evidence grounding
(Section~\ref{sec:policy-grounding-metrics}): whether the agent cites the governing guidance correctly
and whether it applies the passages a domain expert would consider controlling. We report
two axes plus the effect of corpus access itself (Table~\ref{tab:policy}). Policy citation
correctness combines a deterministic existence check (the citation resolves to a real
corpus document and line span) with an LLM-judged support check; policy relevance is an
LLM-judged score against an expert-specified governing-document set. Comparing the
policy-on and policy-off conditions isolates whether corpus access changes verdicts,
evidence that a decision is documentary rather than parametric recall.

\paragraph{Systems cite the governing policy correctly but incompletely.} Policy grounding on the
cohort (Table~\ref{tab:main750-policy}) separates two failure modes a single grounding score
would merge. Taking GPT-5.4-mini and GPT-5.6-Luna, two arms complete at 750 and within 0.2
accuracy points of each other: citations almost always resolve --- 0.991 and 1.000 --- and precision of the cited
document set against the clinical board's governing list is high (0.800 and 0.825). Recall of that
set is roughly half (0.483 and 0.522): systems cite documents that genuinely govern, then omit about
half of the others that also govern. Since a determination resting on part of the applicable standard
can be right for the wrong reason, this is the policy-axis analogue of the trap gap, and a combined
score would hide it because high precision offsets low recall. The shape of that failure is the one
finding here that reproduces across all sixteen arms, because these are
rates rather than counts and each is computed within an arm: resolution runs 0.955--1.000 and
document precision 0.757--0.904, while document recall never exceeds 0.682 and falls as low as 0.395.
Every system in the roster cites real, relevant policy and omits much of the rest.

\paragraph{Fabricated citations dissociate sharply between systems of equal accuracy.} The same two
arms emit 27 and 2 fabricated policy citations --- references resolving to no corpus document --- a
thirteen-fold difference between systems scoring identically on accuracy. Citation support, the
LLM-judged check that a cited passage entails the claim attached to it, moves the same way (0.643
against 0.817). With the trap gap and the confidence margins, this is the third axis on which these
two arms are clearly distinguishable while their headline accuracy is not, and it is the one a
clinician auditing the report would notice first.

\begin{table}[htbp]
\centering
\caption{\textbf{Policy grounding, complete 750-case cohort.} Resolution is the
deterministic check that a citation names a real corpus document and valid line span, support is
LLM-judged, and Doc-P$/$R$/$F1 compare the cited document set against the expert-specified governing
set. All columns are averaged over that arm's policy-expected trials, resolution and support only over
trials that emitted at least one citation. Fabricated citations are counted separately and are not
folded into resolution.}
\label{tab:main750-policy}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccccc}
\toprule
\textbf{Model (harness)} & \textbf{n} & \textbf{Resolve} & \textbf{Support} & \textbf{Doc-P} & \textbf{Doc-R} & \textbf{Doc-F1} \\
\midrule
% <<<AUTOROWS750:tab:main750-policy>>>
Opus 5 (Claude Code)           & 750 & 0.999 & 0.571 & 0.757 & 0.682 & 0.695 \\
Sonnet 5 (Claude Code)         & 750 & 0.993 & 0.590 & 0.833 & 0.453 & 0.613 \\
\addlinespace
GPT-5.6-Sol (Codex)            & 750 & 1.000 & 0.753 & 0.827 & 0.589 & 0.653 \\
GPT-5.6-Luna (Codex)           & 750 & 1.000 & 0.817 & 0.825 & 0.522 & 0.609 \\
GPT-5.5 (Codex)                & 750 & 1.000 & 0.749 & 0.791 & 0.577 & 0.647 \\
GPT-5.4 (Codex)                & 750 & 1.000 & 0.631 & 0.767 & 0.548 & 0.616 \\
GPT-5.4-mini (Codex)           & 750 & 0.991 & 0.643 & 0.800 & 0.483 & 0.605 \\
\addlinespace
Gemini-3.6-Flash (Gemini CLI)  & 750 & 0.988 & 0.469 & 0.770 & 0.629 & 0.664 \\
Gemini-3.5-Flash (Gemini CLI)  & 750 & 0.987 & 0.457 & 0.765 & 0.624 & 0.659 \\
Gemini-3.1-Pro (Gemini CLI)    & 750 & 1.000 & 0.666 & 0.784 & 0.410 & 0.550 \\
\addlinespace
DeepSeek-V4-Pro (opencode)     & 750 & 0.992 & 0.615 & 0.877 & 0.483 & 0.665 \\
DeepSeek-V4-Flash (opencode)   & 750 & 0.955 & 0.577 & 0.868 & 0.422 & 0.637 \\
GLM-5.2 (opencode)             & 750 & 0.986 & 0.589 & 0.820 & 0.514 & 0.645 \\
Qwen-3.7-Plus (opencode)       & 750 & 0.993 & 0.549 & 0.904 & 0.395 & 0.673 \\
MiniMax-M3 (opencode)          & 750 & 0.970 & 0.474 & 0.826 & 0.482 & 0.639 \\
Kimi-K2.7-Code (opencode)      & 750 & 0.998 & 0.602 & 0.841 & 0.474 & 0.649 \\
% <<<END750:tab:main750-policy>>>
\bottomrule
\end{tabular}
\end{table}


\newpage
\subsection{Ablations}
\label{sec:ablations}

The ablations run on the 142-case \emph{development subset} defined in Section~\ref{sec:eval}, because a
full-cohort run per condition is not affordable. All sixteen arms are closed there at $n=142$, which is
what makes per-pair significance and repeated runs possible: of the $\binom{16}{2}=120$ pairs, 58 reach
$p<0.05$ under a two-sided exact McNemar test and 21 survive Holm correction, and accuracy spans
47.2--71.1 with a genuine three-way tie at the top. Every comparison below is paired against the
subset's own baseline and never against Table~\ref{tab:main750}: the subset over-samples the two rare
\textit{Indeterminate} classes, and its Claude arm is Opus 4.8 rather than the cohort's Opus 5, so
absolute scores do not carry across --- GPT-5.6-Luna reads 56.3 here against 64.5 on the cohort. At a
support of 12, one \textit{amb} case moves that column by 8.3 points, so \textit{amb} figures indicate a
direction and never a ranking. The abstention asymmetry of Section~\ref{sec:main-results} reproduces
here on a deliberately different label distribution --- over-commitment exceeds over-abstention in
\emph{all sixteen} arms, 23.4--48.9\% against 5.3--29.5\% --- which is what makes it a property of the
systems rather than of the cohort's label mix. Full sixteen-arm scores on the subset are computed and reported in
Appendix~\ref{app:dev-leaderboard}, together with the per-pair tests and per-class breakdowns; the two
ablations whose tables appear below are the ones the cohort cannot produce at all.

\paragraph{Withholding the policy corpus degrades deferral, not verdict-reaching.} With the corpus
withheld and nothing else changed, accuracy moves \emph{inconsistently} --- three of five arms fall by
3.5--4.3 points and two rise by 0.7--4.2 --- and a two-sided exact McNemar test on the paired cases
separates \emph{no} arm's shift from zero ($p=0.26$--$1.00$). Corpus access is therefore not worth a
fixed number of points, and these deltas do not order the arms. Recall on
\textit{amb} moves consistently on four of the five, falling on three and unchanged on one. That is what
one expects if the corpus is what tells an agent a governing standard exists and does not settle the
case. The policy-enabled condition remains canonical; this is an ablation of the environment, not an
alternative configuration (Table~\ref{tab:ablation-policy}).

\begin{table}[htbp]
\centering
\caption{\textbf{Policy-corpus ablation.} \textit{Paired per case;
web search disabled in both conditions.} $\Delta$ is off $-$ on, so negative means withholding the
corpus hurt. $p$ is a two-sided \emph{exact} McNemar test on the accuracy $\Delta$ over the paired
cases (the discordant counts are 13--26 per arm, far too small for the
$\chi^2$ approximation); \textbf{no arm's accuracy $\Delta$ is distinguishable from zero} ($p=0.26$--$1.00$),
so the deltas establish that corpus access is not worth a fixed number of points and do not order the arms.
\textit{amb} recall is against a support of 12, so one case is 8.3 points --- read
direction, not magnitude. Its own exact McNemar is $p=1.00$ for every arm --- with 0--2 discordant pairs at that support the test has essentially no power, which is the quantitative form of the same warning. The policy-off side is complete at 142 on all five arms. On the policy-on side Gemini-3.1-Pro carries 3 stub trials (no deliverable, no grade), so its row is paired over 139 cases; every other row is paired over all 142. A stub is dropped from BOTH sides so the pairing stays exact.}
\label{tab:ablation-policy}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{Accuracy}} & \multicolumn{3}{c}{\textbf{Recall \textit{amb} \%}} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-8}
\textbf{Model (harness)} & on & off & $\Delta$ & $p$ & on & off & $\Delta$ \\
\midrule
GPT-5.6-Sol (Codex)         & 71.1 & 71.8 & $+0.7$ & 1.00 & 50.0 & 41.7 & $-8.3$ \\
GPT-5.5 (Codex)             & 71.1 & 66.9 & $-4.2$ & 0.26 & 50.0 & 41.7 & $-8.3$ \\
Gemini-3.1-Pro (Gemini CLI) & 72.7 & 68.3 & $-4.3$ & 0.33 & 33.3 & 41.7 & $+8.3$ \\
GPT-5.6-Luna (Codex)        & 56.3 & 60.6 & $+4.2$ & 0.29 & 58.3 & 50.0 & $-8.3$ \\
Opus 4.8 (Claude Code)      & 69.7 & 66.2 & $-3.5$ & 0.36 & 50.0 & 50.0 & $\pm0.0$ \\
\bottomrule
\end{tabular}
\end{table}


\paragraph{Single-attempt accuracy overstates consistent correctness, and the inconsistency is
systematic.} Across three independent attempts, pass\textasciicircum{}3 falls 8.2--12.7 points below
avg@3, and the residual agreement is on the \emph{same wrong} verdict: 16.9--26.8 points, and for
GPT-5.6-Luna 37\% of the cases on which it agreed with itself. Run-to-run variation is small next to
that shortfall --- the standard deviation of accuracy across the three attempts is 1.1--3.2 points ---
so the gap is not attempt noise. High self-consistency is therefore not
evidence of reliability --- these systems are mostly \emph{stably} wrong rather than randomly wrong, so
repeating a query will not surface the error. Reliability is also worst exactly where the benchmark is
hardest: \emph{every} arm's lowest pass\textasciicircum{}3 falls on an \textit{Indeterminate} class
(Table~\ref{tab:passk-perclass}).

\begin{table}[htbp]
\centering
\caption{\textbf{Repeated-run reliability, development subset.} \textit{Three independent attempts.}
$n_{\mathrm{com}}$ counts cases gradeable in \emph{every} attempt, since pass\textasciicircum{}3 is
undefined otherwise; all five arms now cover the full subset. \emph{SD} is the sample standard deviation
(2 degrees of freedom, so a crude estimate rather than a confidence interval) of the three per-attempt
accuracies, which share the $n_{\mathrm{com}}$ denominator. \emph{Spread} is
pass@3 $-$ pass\textasciicircum{}3, the share of cases answered correctly in some attempts and not
others. \emph{Overst.} is avg@3 $-$ pass\textasciicircum{}3, how far a single-attempt figure exceeds
reliable correctness. \emph{Agree} is the share on which all three attempts returned the same
verdict and \emph{Agree-wr} the part of that on an \emph{incorrect} verdict, so
\textit{Agree} $=$ pass\textasciicircum{}3 $+$ \textit{Agree-wr} by construction (exactly on the raw
counts; the printed values can differ by $0.1$ from independent rounding). pass\textasciicircum{}3 and pass@3 are
single set-valued statistics over the intersection and have no across-attempt SD; their dispersion is over
cases, and the binomial standard error is 4.1--4.2 points for pass\textasciicircum{}3 and 3.3--3.9 for pass@3 at $n=142$ --- comparable to the
range of \emph{Overst.} across arms, so the columns support the aggregate claim and not an ordering of
arms. avg@3 is not comparable
with the Acc column of Table~\ref{tab:dev-leaderboard} --- the denominators differ --- and the two
must not be differenced. The eleven remaining arms have a single attempt and are omitted.}
\label{tab:passk}
\small
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lcccccccrr}
\toprule
\textbf{Model (harness)} & $n_{\mathrm{com}}$ & \textbf{avg@3} & \textbf{SD} & \textbf{pass\textasciicircum{}3} & \textbf{pass@3} & \textbf{Spread} & \textbf{Overst.} & \textbf{Agree} & \textbf{Agree-wr} \\
\midrule
Opus 4.8 (Claude Code)         & 142 & \textbf{70.9} & 1.5 & \textbf{62.0} & 79.6 & 17.6 & \phantom{0}8.9 & \textbf{79.6} & 17.6 \\
\addlinespace
GPT-5.5 (Codex)                & 142 & 70.2 & 1.1 & \textbf{62.0} & 78.2 & \textbf{16.2} & \textbf{\phantom{0}8.2} & \textbf{79.6} & 17.6 \\
GPT-5.6-Sol (Codex)            & 142 & 68.3 & 3.2 & 57.0 & 78.2 & 21.1 & 11.3 & 76.8 & 19.7 \\
GPT-5.6-Luna (Codex)           & 142 & 57.7 & 1.9 & 46.5 & 66.9 & 20.4 & 11.3 & 73.2 & 26.8 \\
\addlinespace
Gemini-3.1-Pro (Gemini CLI)    & 142 & 69.7 & 2.4 & 57.0 & \textbf{81.0} & 23.9 & 12.7 & 73.9 & 16.9 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htbp]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Per-class repeated-run reliability.} \textit{Development subset, three attempts.}
pass\textasciicircum{}3 is the share of that class's cases answered correctly in \emph{all three}
attempts, pass@3 the share correct in \emph{at least one}; $n$ is the per-class count gradeable in all
three, so the four supports sum to the arm's $n_{\mathrm{com}}$ in Table~\ref{tab:passk} and the two
tables reconcile exactly. \emph{SD} is the sample standard deviation of that class's accuracy across the
three attempts (2 degrees of freedom), not of pass\textasciicircum{}3 or pass@3, which are set-valued and
have no across-attempt SD. \textbf{The \textsc{amb} support is 12 cases, where one case moves a
cell by 8.3 points; that column indicates a direction and must not be read as a ranking, and its SD
in particular carries almost no information at that support and 2 degrees of freedom.} The per-case
binomial standard error at the class supports is about 6.9 points at $n=50$, 7.3 at $n=45$, 8.3 at $n=35$ and 14.1 at $n=12$, so no single cell separates arms.
All five arms now cover the full subset (\textsc{yes} 50, \textsc{no} 45, \textsc{lack} 35, \textsc{amb} 12).}
\label{tab:passk-perclass}
\begin{tabular}{lcccccccccccccccc}
\toprule
& \multicolumn{4}{c}{\textsc{yes}} & \multicolumn{4}{c}{\textsc{no}}
& \multicolumn{4}{c}{\textsc{lack}} & \multicolumn{4}{c}{\textsc{amb}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
\textbf{Model (harness)} & $n$ & \^{}3 & @3 & SD & $n$ & \^{}3 & @3 & SD & $n$ & \^{}3 & @3 & SD & $n$ & \^{}3 & @3 & SD \\
\midrule
Opus 4.8 (Claude Code)       & 50 & \textbf{74.0} & \textbf{94.0} & 1.2 & 45 & 57.8 & \textbf{82.2} & 3.4 & 35 & 54.3 & 60.0 & 0.0 & 12 & \textbf{50.0} & \textbf{66.7} & 4.8 \\
\addlinespace
GPT-5.5 (Codex)              & 50 & 64.0 & 86.0 & 2.0 & 45 & \textbf{71.1} & 80.0 & 2.6 & 35 & 54.3 & 74.3 & 1.6 & 12 & 41.7 & 50.0 & 4.8 \\
GPT-5.6-Sol (Codex)          & 50 & 62.0 & 84.0 & 3.5 & 45 & 60.0 & \textbf{82.2} & 6.7 & 35 & 51.4 & 74.3 & 1.6 & 12 & 41.7 & 50.0 & 4.8 \\
GPT-5.6-Luna (Codex)         & 50 & 48.0 & 64.0 & 4.6 & 45 & 48.9 & 71.1 & 2.2 & 35 & 42.9 & 68.6 & 1.6 & 12 & 41.7 & 58.3 & 8.3 \\
\addlinespace
Gemini-3.1-Pro (Gemini CLI)  & 50 & 60.0 & 86.0 & 4.2 & 45 & 62.2 & \textbf{82.2} & 6.8 & 35 & \textbf{60.0} & \textbf{82.9} & 2.9 & 12 & 16.7 & 50.0 & 4.8 \\
\bottomrule
\end{tabular}
\end{table}

\newpage

\george{The three earlier-build ablations above are not yet re-run on the current stack. TBD on the scope and if we want to run}

\paragraph{Prompt interventions for abstention.} Four case-agnostic interventions were tested against an
unmodified baseline: a post-retrieval abstention decision-gate, a structured answer format separating
claims-and-evidence from the verdict, a self-critique pass, and an underspecification check. None
reliably lifts abstention. The gate and the structured format both \emph{lower} \textit{lack} recall;
self-critique nudges the stronger model's accuracy while committing more often; and the
underspecification check, the one positive, raises the weaker model's \textit{lack} recall at flat
accuracy but does not transfer to the stronger model. The effects are small, mixed and model-dependent,
which is itself evidence that under-abstention is a genuine benchmark axis rather than a shallow
prompting artefact. These four ran on an earlier build of the case prompts and grading stack, so their
absolute numbers are not comparable with the tables here; we report the direction and withhold the
table rather than invite a comparison the data does not support.

\paragraph{Harness versus model.} Holding the model fixed and varying the harness across three
model-agnostic harnesses moves accuracy little, so at fixed model the harness is not the dominant term
--- the across-model spread within a single harness is larger. Two differences are substantive:
deliverable reliability separates the harnesses where accuracy does not, and cost differs several-fold
for an accuracy difference inside noise, with the most expensive harness buying the best process score.
This too is an earlier-build measurement, reported for direction only.

\paragraph{Test-time compute (reasoning effort).} Harness defaults do sit at the top of the effort
range, but for two different reasons that are worth separating. The Codex adapter sets
\texttt{reasoning\_effort} to \texttt{high} by default, so for that harness an unflagged run and an
explicit \texttt{high} run are the same condition and no comparison between them is informative. Claude
Code sets no default, and there the coincidence is a measurement: over the 45 cases both arms completed,
the median \emph{within-case} ratio of default to \texttt{high} completion tokens is 1.000, with the
interquartile range straddling unity and the sign of the difference splitting 22--23 across cases. We
therefore compare three explicit levels --- \texttt{low}, \texttt{medium}, \texttt{high} --- on one
model on the development subset, against a build whose verifier budget matches the cohort's.
Compute rises substantially and monotonically across them. Comparing \emph{within case} rather than
between medians --- necessary because the median case for one level is not the median case for another ---
completion tokens rise 44\% from \texttt{low} to \texttt{medium} and a further 26\% to \texttt{high},
75\% end to end (Table~\ref{tab:ablation-effort}). Neither verdict accuracy nor process adherence follows.
Accuracy is 68.3, 69.1 and 69.1 at $n=139$, 139 and 136 --- a total spread of 0.8 points against a
per-level standard error of about 4 --- and \emph{every} pairwise accuracy difference lies within 0.1
standard errors of that difference, every process difference within 1.3. Additional test-time
compute therefore buys neither better verdicts nor a better-documented method, which is what one expects
if the binding constraint is retrieval elicitation and label discrimination rather than reasoning depth.
Two limits bound this. The trajectories expose no reasoning-token count, so completion tokens are the
only available compute proxy and we cannot say \emph{where} the additional compute was spent; and the
per-level $n$ differ because 1--3 trials per level were lost to environment failures before grading,
which is a property of the infrastructure rather than of the condition.

\begin{table}[htbp]
\centering
\caption{\textbf{Test-time compute (reasoning effort).} \textit{Opus 4.8 on Claude Code, dev142, three explicit effort levels on one case build.} Accuracy is over all trials in $n$ (a trial that ran but produced no deliverable scores wrong, it is not dropped); the parenthesised figure is the correct count. \emph{Proc \%} is the summed rubric ratio $\sum\mathit{earned}/\sum\mathit{possible}$; its $\pm$ is the per-trial SD$/\sqrt{n}$, and accuracy's is binomial. \textbf{No effect is distinguishable from zero:} every pairwise accuracy difference is $\leq0.1$\,SE$_d$ and every process difference $\leq1.3$\,SE$_d$, while median completion tokens rise 75\% from \texttt{low} to \texttt{high} (\texttt{low}$\to$\texttt{medium} $+44$\%, \texttt{medium}$\to$\texttt{high} $+26$\%), so the ladder is a genuine three-point compute contrast rather than one usable step. \emph{Those compute deltas are median \textbf{within-case} ratios over the 130 cases graded at all three levels, not ratios of medians} --- the median case at one level is not the median case at another, and the distinction is not cosmetic: for the unflagged default arm the paired method gives $+0.0$\% against \texttt{high} where comparing medians gives $+17.2$\%, which would have wrongly overturned the accompanying claim. Denominators reconcile per level as $142$ attempted $-$ died $-$ never-attached $-$ stubs: \texttt{low} $142-2-1-0=139$, \texttt{medium} $142-1-1-1=139$, \texttt{high} $142-3-1-2=136$. All three exclusions are \textbf{infrastructure, not model behaviour}: unhealthy \texttt{env-mimic-tools} sidecars accounted for 73 of 133 trial deaths session-wide, a stub is a trial killed after writing a truncated \texttt{reward.json}, and \emph{never-attached} means the agent never reached the MCP tool server. Realised \texttt{VerifierTimeoutError} was \textbf{zero} throughout --- these ran a build cut at \texttt{[verifier] timeout\_sec = 1800}. The never-attached exclusion is \textbf{symmetric at exactly one trial per level}, so it cannot bias the comparison. \emph{Limit:} no reasoning-token field exists anywhere in the trajectory, so completion tokens are the only available compute proxy and thinking tokens cannot be separated from answer tokens --- the table shows that more compute was spent, not \emph{where} it went. USD is harness-reported for this vendor route.}
\label{tab:ablation-effort}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccccccc}
\toprule
 & & & & & \multicolumn{3}{c}{\textbf{Median tokens}} & \\
\cmidrule(lr){6-8}
\textbf{Effort} & \textbf{n} & \textbf{Acc \%} & \textbf{Proc \%} & \textbf{earned/poss} & comp & prompt$_{\mathrm{k}}$ & cached$_{\mathrm{k}}$ & \textbf{USD} \\
\midrule
  \texttt{low} & 139 & 68.3\,$\pm$\,3.9 (95) & 64.8\,$\pm$\,2.3 & 986/1521 & 7\,057 & 577 & 515 & 0.855 \\
  \texttt{medium} & 139 & 69.1\,$\pm$\,3.9 (96) & 68.9\,$\pm$\,2.1 & 1045/1517 & 9\,758 & 697 & 618 & 1.013 \\
  \texttt{high} & 136 & 69.1\,$\pm$\,4.0 (94) & 67.6\,$\pm$\,2.4 & 1001/1481 & 11\,877 & 732 & 663 & 1.115 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Web access.} Not run. The execution environment enforces a deny-by-default egress allowlist,
so the frozen-corpus condition is canonical and an open-web condition needs a separate environment build
--- a case build with a wider \texttt{allowed\_hosts} plus a web-enabled agent adapter, neither of which
exists today. We report it as future work rather than as a measured null result.



\subsection{Qualitative Analysis}
\label{sec:qualitative}

The aggregate scores hide a failure signature that trap-adjusted accuracy makes precise. A cirrhotic
patient is admitted with hepatic encephalopathy and moderate ascites, and no diagnostic paracentesis
appears anywhere in the admission, so spontaneous bacterial peritonitis can be neither confirmed nor
excluded and the reference verdict is \textit{Indeterminate: Lack of Data}. All five systems commit to
a definitive label, and four reach it through the same prohibited shortcut --- asserting peritonitis
excluded with no ascitic-fluid result, the \textsc{must-not} criterion N4
(Table~\ref{tab:qual-he-precipitant}). The failure is not one of retrieval: every one of the five
names the missing paracentesis in its own report, and the process judge's justifications independently
describe the same mechanism, that the systems acknowledged the absent study and then treated the
diagnosis as effectively worked up. The sharpest case is GPT-5.6-Luna, which performs the deferral
reasoning correctly, earns the criterion rewarding escalation of an unresolved question, and avoids
the trap --- and still emits a definitive \textit{No}. Recognising an evidentiary gap is therefore not
sufficient; here the failure occurs at label assignment, after the reasoning that should have
prevented it. This is why the benchmark scores the observable adjudication process separately from the
verdict, and why raw and trap-adjusted accuracy diverge.

\begin{table}[htbp]
\centering
\small
\caption{\textbf{Qualitative failure profile} (\texttt{he-precipitant-278ac1}). No diagnostic
paracentesis exists in the admission, so spontaneous bacterial peritonitis can be neither confirmed
nor excluded. Four of the five spring the same \textsc{must-not} criterion N4, ``Asserted SBP
excluded without an ascitic-fluid result''. GPT-5.6-Luna avoids the trap and earns the escalation
criterion, yet still commits.}
\label{tab:qual-he-precipitant}
\begin{tabular}{llcc}
\toprule
\textbf{System} & \textbf{Verdict} & \textbf{Stated conf.} & \textbf{Trap sprung} \\
\midrule
\emph{Gold} & \textit{Indeterminate: Lack of Data} & --- & --- \\
\midrule
Claude Sonnet 5 (Claude Code)   & Yes & \phantom{0}90\% & N4 \\
Claude Opus 4.8 (Claude Code)   & Yes & \phantom{0}90\% & N4 \\
GPT-5.5 (Codex)                 & Yes & \phantom{0}78\% & N4 \\
Gemini-3.5-Flash (Gemini CLI)   & Yes & 100\% & N4 \\
GPT-5.6-Luna (Codex)            & No  & \phantom{0}78\% & --- \\
\bottomrule
\end{tabular}
\end{table}

\george{TODO: validate/replace this.}

\subsection{Benchmark Validation: Judge Reliability and Label Quality}
\label{sec:validation}

\george{TODO: Review and validate latest version}

As both the process score and the reference labels are used to rank systems, we
validate each before drawing conclusions from them.

\paragraph{Judge reliability and self-consistency.} The process rubric is LLM-adjudicated,
so we measure whether the grade is stable across judges rather than assuming it. A five-judge
panel grades every trajectory over the full rubric with three replicates each. We report
inter-judge agreement primarily as the mean pairwise disagreement. It flags 16\% of
criteria as contested, with the judges self-consistent across replicates and statistically
interchangeable on the aggregate score (companion Fleiss' $\kappa \approx 0.65$). The
most-contested criteria (for example, a hidden antibiotic de-escalation window and an
era-dependent heart-failure therapy) are exactly the cases an independent expert audit flagged
as under-specified, so judge disagreement acts as an automatic detector of ambiguous criteria,
which are then routed back for expert revision. This supports reporting the process score as a
real metric rather than judge noise.

\paragraph{Policy-judge reliability and self-consistency.} The policy rubric is mostly deterministic: citation existence and policy relevance are computed by rule, while only citation support requires LLM judgment. Accordingly, the two rule-based items achieve perfect agreement ($\kappa=1.0$) with no replicate variation, and the remaining LLM judgment is stable across judges (companion Fleiss' $\kappa\approx0.86$; within-judge noise 0.023--0.025 on a $0,1$ scale). The production judge is therefore representative rather than unusually strict or lenient. The residual variation is systematic: judges sometimes under-credit near-verbatim citations, making citation-correctness scores conservative lower bounds, and we find no evidence of own-family favoritism. By defining policy relevance through expert gold documents rather than LLM judgment, we remove a major source of ambiguity at the rubric-design stage. This supports treating the policy score as a meaningful metric rather than judge noise.

\paragraph{Label quality.} Reference labels differ in provenance, so we validate the labels
themselves. On 44 of 142 development cases (31\%) the majority of the evaluated models
disagrees with the silver gold, with a further 6\% reaching no majority; re-labeling to
consensus leaves the overall accuracy level stable (within a few points) but reshuffles the
model ordering. We therefore
hold ranking claims until the Clinical Board labels and report the clinician-validated and
model-assisted subsets separately (Section~\ref{app:case_coverage}), so a reader can see
which conclusions hold on the fully adjudicated labels.


==> author_contributions.tex <==
Veronica Chatrath — benchmark execution lead (CB network, experiments) and primary manuscript lead

Bryan Zhu — healthcare lead, technical lead, and primary developer

George Pu — technical lead and primary developer

Jingxuan Fan — evidence grounding and metrics ideation and implementation

Apaar Shanker — policy grounding ideation

Varun Ursekar — policy grounding implementation

Anahita Sharma — policy and evidence grounding, CB network, and MIMIC env creation

Jason Qin — domain expertise and experimental ideation

Keqi Han — medical data, domain expertise, and related work

Soham Dinesh Tiwari — medical task release and domain contribution

Soham Dan — medical task release and domain contribution

Vijay Kalmath — manuscript iteration

Yuan (Christy) Li — manuscript iteration

Daniel Yue Zhang — benchmark release

Chenguang Wang — senior benchmark advisor

Zainab Doctor — medical data and domain expertise

Zhijun Yin — medical-domain guidance and related work

Nigam Shah — senior medical-domain advisor

Yuan (Emily) Xue — senior project lead, problem conception, vision, benchmark direction, manuscript leadership, and supervision


==> evaluation_bk_07252pst.tex <==
\section{Evaluation Framework}
\label{sec:eval}

\benchmarkname{} scores autonomous systems with a set of per-example metrics that are aggregated into cohort-level summaries. The per-example metrics extend beyond binary accuracy to capture grounding, appropriate abstention, and the quality of the agent's reasoning process; cohort-level aggregation then adds reliability and cost. Every metric is computed from the artifacts each trial records: the agent's final report, the tool calls and reasoning captured in its trajectory, and the case's Clinical Board--validated metadata.

\subsection{Outcome Metrics}

\begin{itemize}
    \item \textbf{Accuracy:} Measures the formal agreement between the agent's final classification (\textit{Yes}, \textit{No}, \textit{Indeterminate: Lack of Data}, or \textit{Indeterminate: Medically Ambiguous}) and the Clinical Board--validated gold label. We report overall accuracy together with a macro-averaged F1 and per-class precision, recall, and F1, so that performance on the less frequent, safety-critical \textit{Indeterminate} classes is not obscured by majority-class statistics.
    \item \textbf{Insight Grounding:} Evaluates whether the claims made by the agent are anchored in authentic medical records, reported as a list of substantiated claims paired with their cited sources. The framework assesses grounding along two complementary axes: \emph{citation precision}, whether the claims it states are faithful to that evidence, and \emph{evidence recall}, whether it surfaced the evidence the case requires.

\emph{Citation precision} is the proportion of the report's asserted facts that the
cited evidence accurately supports, penalizing fabricated or misattributed citations.
As a first guard against fabrication, every cited \textbf{record identifier} (patient,
admission, stay, order, or note) must appear in the evidence the agent retrieved;
because such an identifier can only be copied and never inferred, any cited identifier
absent from the evidence is necessarily invented, giving a record-level precision
$P_{\mathrm{record}} = |\mathcal{I}_{\mathrm{cited}} \cap \mathcal{I}_{\mathrm{evidence}}|
\,/\, |\mathcal{I}_{\mathrm{cited}}|$ over the cited identifiers $\mathcal{I}_{\mathrm{cited}}$. \jingxuan{The record identifier level every model is ~1 so we can also omitting reporting this part, this is more like a guardrail}
The reported precision is then measured at the level of \textbf{clinical claims}: the
report is decomposed into atomic factual assertions---measured values, doses, imaging
and procedure findings, and the presence or absence of an event---each judged
\emph{supported}, \emph{contradicted}, or \emph{unverifiable} against the evidence, and
precision is the supported fraction $P_{\mathrm{claim}} = N_{\mathrm{supported}} \,/\, N_{\mathrm{claims}}$.


\emph{Evidence recall} measures whether the agent gathered and reported the information needed for a correct answer. It complements precision: a report can be faithful to its citations yet still miss the findings that determine the clinical decision. We assess it at both ends of the agent's
process---the evidence it gathered while investigating, and the findings it ultimately
reported. At the gathering end, \textbf{retrieval recall} asks whether the agent
consulted the sources the case depends on. For each case, a medical expert annotates
the set of MIMIC-IV source tables $\mathcal{S}_{\mathrm{gold}}$ that a correct answer
must draw on, and retrieval recall is the
fraction of these the agent actually queried during its investigation,
$R_{\mathrm{retrieval}} = |\mathcal{S}_{\mathrm{gold}} \cap \mathcal{S}_{\mathrm{consulted}}|
\,/\, |\mathcal{S}_{\mathrm{gold}}|$.  At the reporting end, \textbf{insight
coverage} asks whether the report presents the findings the case calls for. For each case, the medical expert also annotates a set of required-evidence categories
$\mathcal{C}_{\mathrm{req}}$---the decisive pieces of evidence a sound answer must
establish, such as a creatinine timeline spanning the relevant window, dialysis
status, or confirmation of an imaging study's timing---and an LLM judge determines,
category by category, whether the report addresses each one, either by presenting the
evidence or by stating an explicit finding about it (including a documented absence).
Insight coverage is the fraction of categories judged covered,
$C_{\mathrm{insight}} = |\{c \in \mathcal{C}_{\mathrm{req}} : \mathrm{covered}(c)\}|
\,/\, |\mathcal{C}_{\mathrm{req}}|$.
%\textbf{Insight Grounding:} Evaluates whether the claims made by the agent are anchored in authentic medical records, reported as a list of substantiated claims paired with their cited sources. The framework calculates \textbf{citation precision} (the proportion of cited spans that accurately and factually support the assertion, penalizing fabricated or irrelevant citations) and \textbf{evidence recall} (the proportion of mandatory data streams specified in the case's grounding criteria that the agent successfully extracted) \cite{chung2026verifact, munnangi2024factehr}.
    \item 
    % \george{Technically implemented, we have precision/recall/F1 metrics on all classification labels. Maybe there's an easy way to tie confidence into these numbers, such as reporting calibration error (e.g., https://github.com/centerforaisafety/hle/blob/main/hle\_eval/run\_judge\_results.py\#L96-L127).}
    % \bryan{this is directly correlated with class accuracy, is this something we need to measure/compute separately? if so, calling it "calibration" adds confusion between this and the EFE concept of escalation/calibration, so I would propose a different name}
    \textbf{Abstention Behavior:} Quantifies \emph{how} a system handles the deferral decision, the behavior the benchmark is built to stress. It characterizes two directional errors: \emph{over-commitment}, returning a definitive \textit{Yes}/\textit{No} when the chart warrants deferral, and \emph{over-abstention}, returning \textit{Indeterminate} when the record in fact supports a definitive conclusion. It further scores whether the agent correctly separates \textit{Indeterminate: Lack of Data} from \textit{Indeterminate: Medically Ambiguous}, since mistaking a missing-evidence case for a genuinely ambiguous one, or the reverse, reflects a distinct reasoning failure with a different downstream remedy (retrieving more evidence versus escalating to expert judgment).
    % Quantifies an agent's capacity to recognize safety boundaries and abstain under uncertainty. The framework evaluates precision and recall against the two Indeterminate ground-truth classes, jointly, the abstention class (measuring rates of over-commitment and providing a definitive Yes or No when the chart warrants deferral) and over-abstention (returning Indeterminate when the available record contains sufficient evidence to form a definitive conclusion). It further scores whether the agent correctly separates Indeterminate: Lack of Data from Indeterminate: Medically Ambiguous, since mistaking a missing-evidence case for a genuinely ambiguous one, or the reverse, reflects a distinct reasoning failure with a different downstream remedy (retrieving more evidence versus escalating to expert judgment). Whether the agent actively retrieves the evidence a clinician would seek, issuing the right look-ups rather than answering from the first records returned, measured against the case's required-evidence set.
\end{itemize}

\subsection{Process Rubric Metric}
In addition to outcome-based scoring, every case carries a process rubric of \textbf{MUST-DO} and \textbf{MUST-NOT} criteria, each with a signed weight, that grades \emph{how} the agent reached its answer. An LLM judge marks each criterion met or not-met against both the agent's report and its tool-call trajectory, so that a methodology claimed in the report is credited only when the agent's actions corroborate it. The trial's process score is a weighted percentage of achievable credit: the denominator is the sum of the MUST-DO weights, and the numerator is the earned MUST-DO credit less the penalty of any MUST-NOT the agent violated (such as fabricating a laboratory value or inferring a clinical endpoint purely from an unvetted billing code), floored at zero. This decoupling of workflow process from final classification lets CliniCARE-Bench differentiate an agent that reached the correct answer through sound clinical reasoning from one that simply guessed correctly.

Because the process grade is LLM-adjudicated, we characterize its reliability directly: a panel of judge models grades each trajectory, and we report inter-judge agreement (Fleiss' $\kappa$) and the most-contested rubric dimensions, so that criteria the judges cannot grade consistently are surfaced and revised rather than trusted silently.

\subsection{Cohort-Level Aggregation}
% \george{Aggregation is not implemented yet, but is low lift. Maybe someone can add details on what the cohorts we care about -- is it by reasoning skill, clinical domain (table 2) or by user demographic/etc.}
Per-example metrics are aggregated both within each case (over its 30 cases) and across all 25 cases to characterize a system at the cohort level along two additional dimensions. Beyond these aggregate views, each metric can be aggregated by the reasoning skill and clinical domain a case exercises, following the case taxonomy in Appendix~\ref{app:case_coverage} (Table~\ref{tab:skill_domain_coverage}), so that a system's profile can be read per-skill and per-domain rather than only in aggregate.

% Per-example metrics are aggregated both within each case (over its 30 patients) and across all 25 cases to characterize a system at the cohort level
% along three additional dimensions.
\begin{itemize}
  \item \textbf{Reliability:} 
  % The consistency of a system's verdicts and grounding across the cases of a case and across repeated runs, distinguishing systems that are dependably correct from those that are only correct on average.
  The consistency of a system's verdicts and grounding across the 30 cases of a case and across repeated attempts. As the reliability metric we report \textnormal{pass\textasciicircum k} \cite{yao2024taubenchbenchmarktoolagentuserinteraction}, the fraction of items answered correctly on \emph{all} $k$ independent attempts: it credits a system only when every attempt agrees, rewarding dependable correctness rather than a single lucky run. Because clinical use cares about worst-case consistency, we report \textnormal{pass\textasciicircum k} rather than the best-of-$k$ $\mathrm{pass}@k$, along with $\mathrm{avg}@k$.
  \item \textbf{Cost and Efficiency:} The resource intensity of each agent trajectory---total tokens, tool calls, and turns. We also report the time subject-matter experts spend completing and validating a case, as a human-effort reference point for the same clinical work.
  % \item \textbf{Win-Rate vs.\ Human:} Using a clinician's case-completion time
  % as a cost proxy, CliniCARE-Bench frames a head-to-head comparison that asks not only
  % whether an agent is correct, but whether its output would be preferred to an
  % expert's at materially lower cost.
\end{itemize}

% \subsection{Policy Citation and Compliance}
% \label{sec:policy-eval}
% % Policy grounding (Section~\ref{sec:policy}) is scored \emph{separately} from the patient-evidence grounding above, along two axes:
% Policy grounding (Section~\ref{sec:policy}) is scored \emph{separately} from the patient-evidence grounding above. Both axes below are graded as three-class line items---\emph{followed}, \emph{partially followed}, or \emph{did not follow} (1.0 / 0.5 / 0.0)---in a single per-case policy rubric, and the policy score is their weighted mean (items with nothing to check, such as citation correctness when the agent emitted no citations, are excluded).
% \begin{itemize}
%   \item \textbf{Policy citation correctness:} whether each cited passage exists in the corpus and factually supports its associated claim, checked at the line level to separate genuine documentary attribution from fabricated or parametric justification.
%   \item \textbf{Policy relevance:} a rubric-based judgment, following the same \textbf{MUST DO} / \textbf{MUST NOT} structure used elsewhere, of whether the agent retrieved and applied the policy passages a domain expert would consider governing for the case.
% \end{itemize}
% Through measuring both the policy-on and policy-off conditions, this axis captures not only whether the agent cites policy, but whether access to the corpus changes its verdicts, evidence that a decision is documentary rather than latent recall. 

\subsection{Policy Citation and Compliance}
\label{sec:policy-eval}
Policy grounding (Section~\ref{sec:policy}) is scored \emph{separately} from the patient-evidence grounding above, as a per-case rubric of three line items graded on a common three-class scale---\emph{followed}, \emph{partially followed}, or \emph{did not follow} (1.0 / 0.5 / 0.0). The first two items constitute \textbf{citation correctness} and the third \textbf{policy relevance}; two are adjudicated deterministically and only one invokes an LLM judge. Grounding is expressed through inline citations of the form \texttt{[policy:~\textit{document}~L\textit{a}--L\textit{b}]}, which name a corpus document and a physical line span and which the verifier resolves against the same source files the agent read:
\begin{itemize}
  \item \textbf{Citation existence} (deterministic): every citation must resolve to a document present in the corpus and to a valid line span within it, separating real documentary anchors from fabricated, out-of-corpus, or invalid-span references.
  \item \textbf{Citation support} (LLM-judged): each cited passage is assessed for whether it factually entails the specific claim it is attached to, distinguishing genuine attribution from citations that are merely on-topic or confabulated.
  \item \textbf{Policy relevance} (deterministic): grounding is scored by set membership against a per-case list of governing authoritative documents curated by the clinical board. A response is \emph{followed} when it cites only governing documents, \emph{partially followed} when it cites at least one governing document alongside non-governing ones, and \emph{did not follow} when it cites none.
\end{itemize}

The policy score is the weighted mean of the applicable items. Relevance is always applicable: a response that cites no governing document, including one that cites nothing at all, is scored \emph{did not follow}. The two citation-correctness items are evaluated only when citations exist and are otherwise omitted, since the existence or support of a citation cannot be assessed when none was made. A non-citing response therefore receives a failing relevance score and no correctness credit, rather than escaping evaluation.

Confining LLM adjudication to the support check renders relevance and existence reproducible by construction and isolates judge variance to a single item, which we characterize with the same judge-panel protocol used for the process rubric---inter-judge agreement (Fleiss' $\kappa$) and the most-contested criteria.


% \paragraph{Example: post-CT acute kidney injury.}
% For the post-CT AKI scenario, the process rubric operationalizes the
% investigation required to apply the scenario criteria correctly.

% \emily{TODO: to review again. This list is not the same as what is included in the Figure 2 in the previous version. }
% \begin{itemize}

%     \item \textbf{\textsc{Must-do} criteria} include:

%     \begin{itemize}

%         \item Identify the qualifying CT examination and establish its
%         performed time, distinguishing it from the order time.

%         \item Retrieve all available serum-creatinine measurements within
%         the specified pre-CT baseline window.

%         \item Assess whether the pre-CT creatinine values support a stable
%         and interpretable baseline under the scenario criteria.

%         \item Compare the peak post-CT creatinine with the established
%         baseline using both the absolute and relative KDIGO thresholds.

%         \item Check whether chronic dialysis, end-stage renal disease, or
%         another specified exclusion makes the acute criteria inapplicable.

%     \end{itemize}

%     \item \textbf{\textsc{Must-not} criteria} include:

%     \begin{itemize}
%         \item Do not infer AKI solely from an AKI diagnosis code, problem-list
%         entry, or statement in a clinical note without independently
%         verifying the creatinine criteria.

%         \item Do not treat the CT order time as the performed scan time
%         without confirming that the examination occurred at that time.

%         \item Do not apply the acute creatinine thresholds without first
%         establishing an eligible and interpretable baseline.

%         \item Do not return a definitive \textit{No} when required baseline
%         or post-CT measurements are missing.

%         \item Do not infer that the CT scan or contrast administration caused
%         the AKI; the scenario asks whether AKI occurred following imaging,
%         not whether it was contrast-induced.

%     \end{itemize}

% \end{itemize}

==> not-used.tex <==

% \subsection{Calibration}
% \label{sec:calibration}

% Enterprise readiness is not maximal autonomy; it is the \emph{minimum total
% cost of meeting a reliability target}. We formalize this as a selective-prediction
% problem with deferral to a human, and derive a single per-case economic metric:
% the model (token) cost plus the human-oversight cost an agent still requires to
% reach a target reliability $Y$.

% \subsubsection{Per-case decision pipeline}

% For each case $i$ in an evaluation set of $N$ cases, the agent emits a raw
% confidence $s_i$ and a predicted verdict $\hat{y}_i$. A calibration map $g$
% (fit on held-out data) produces a \emph{calibrated} confidence
% \begin{equation}
%   c_i \;=\; g(s_i) \;\approx\; \Pr\!\big(\hat{y}_i = y_i \,\big|\, s_i\big),
% \end{equation}
% so that $c_i$ estimates the probability that the agent's verdict is correct.
% Given an escalation threshold $\tau \in [0,1]$, the agent acts autonomously when
% $c_i \ge \tau$ and \emph{escalates} the case to a human reviewer otherwise:
% \begin{equation}
%   a_\tau(c_i) \;=\;
%   \begin{cases}
%     \textsc{autonomous}, & c_i \ge \tau,\\[2pt]
%     \textsc{escalate},   & c_i < \tau.
%   \end{cases}
% \end{equation}

% \subsubsection{Notation}

% Let $c$ have cumulative distribution $F$ and density $f$ over the case
% population. We define
% \begin{align}
%   \phi(\tau)   &= \Pr(c \ge \tau) = 1 - F(\tau)             && \text{(coverage / autonomy rate),}\\
%   e(\tau)      &= 1 - \phi(\tau) = F(\tau)                   && \text{(escalation rate),}\\
%   \alpha(\tau) &= \mathbb{E}\!\left[\,c \,\middle|\, c \ge \tau\,\right] && \text{(selective accuracy).}
% \end{align}
% We write $a_H$ for the human reviewer's accuracy on escalated cases, $Y$ for the
% target system reliability, $k_m$ for the model cost per case, and $k_h$ for the
% cost of one human review (with $k_h \gg k_m$).

% \subsubsection{System reliability}

% Autonomous cases are correct with probability $c$; escalated cases are correct
% with probability $a_H$. Under calibration $\big(\Pr(\text{correct}\mid c)=c\big)$,
% the deployed system's reliability is
% \begin{equation}
%   R(\tau)
%   \;=\; \phi(\tau)\,\alpha(\tau) + \big(1-\phi(\tau)\big)\,a_H
%   \;=\; \underbrace{\int_{\tau}^{1} c\,f(c)\,dc}_{\text{autonomous correct mass}}
%         \;+\; \underbrace{a_H\,F(\tau)}_{\text{human-handled}}.
%   \label{eq:reliability}
% \end{equation}

% \begin{lemma}[Monotonicity]
% \label{lem:mono}
% $R(\tau)$ is nondecreasing in $\tau$ on $[0, a_H]$, since
% $\frac{d R}{d\tau} = (a_H - \tau)\,f(\tau) \ge 0$ for $\tau \le a_H$.
% \end{lemma}
% \noindent
% Intuitively, routing a borderline-confidence case to the more reliable human
% raises system reliability until the threshold exceeds the human's own accuracy.

% \subsubsection{Cost-optimal gating and the economic metric}

% The token cost $k_m$ is incurred on every case, whereas the human cost $k_h$ is
% incurred only on escalated cases. The expected cost per case is therefore
% \begin{equation}
%   c_{\mathrm{unit}}(\tau) \;=\; k_m \;+\; k_h\,e(\tau) \;=\; k_m + k_h\,F(\tau),
%   \label{eq:cunit}
% \end{equation}
% which is strictly increasing in $\tau$. Minimizing cost subject to the reliability
% constraint thus selects the \emph{smallest} feasible threshold:
% \begin{equation}
%   \tau^\star \;=\; \min\,\{\,\tau \in [0,1] : R(\tau) \ge Y\,\},
%   \qquad
%   C^\star \;=\; k_m + k_h\,F(\tau^\star).
%   \label{eq:opt}
% \end{equation}
% By Lemma~\ref{lem:mono}, $R$ is monotone, so $\tau^\star$ is well defined whenever
% the target is attainable. Two regimes bound the curve:
% \begin{itemize}
%   \item \textbf{Floor.} If the base accuracy $a_0 = \mathbb{E}[c] = R(0)$ already
%         satisfies $a_0 \ge Y$, then $\tau^\star = 0$ and $C^\star = k_m$:
%         no escalation is required.
%   \item \textbf{Ceiling.} Since $\sup_\tau R(\tau) = a_H$, the target is feasible
%         only if $Y \le a_H$: to promise reliability $Y$, the human review process
%         must itself attain at least $Y$.
% \end{itemize}

% It is convenient to report savings relative to the all-human baseline (reviewing
% every case at cost $k_h$) and the dimensionless cost ratio $\rho = k_h/k_m$:
% \begin{equation}
%   S \;=\; k_h - C^\star \;=\; k_h\,\phi(\tau^\star) - k_m,
%   \qquad
%   \frac{C^\star}{k_m} \;=\; 1 + \rho\,F(\tau^\star).
% \end{equation}

% \subsubsection{Closed form under a Beta confidence model}

% To instantiate the curve, we model the calibrated confidence as
% $c \sim \mathrm{Beta}(\alpha,\beta)$ with mean $\mu = \alpha/(\alpha+\beta)$ (the
% base accuracy) and concentration $\nu = \alpha+\beta$ (calibration sharpness).
% Writing $I_x(a,b)$ for the regularized incomplete beta function (the
% $\mathrm{Beta}$ CDF), the identity
% $\int_{\tau}^{1} c\,f(c;\alpha,\beta)\,dc = \mu\,\big(1 - I_\tau(\alpha+1,\beta)\big)$
% gives the closed forms
% \begin{align}
%   e(\tau) &= I_\tau(\alpha,\beta), \\
%   R(\tau) &= \mu\,\big(1 - I_\tau(\alpha+1,\beta)\big) + a_H\,I_\tau(\alpha,\beta).
% \end{align}
% Substituting $\tau^\star$ from \eqref{eq:opt} into \eqref{eq:cunit} yields the
% cost as a function of the target $Y$ for each model (Figure~\ref{fig:cost}).
% The resulting \emph{cost-of-reliability} curve is convex and diverges as
% $Y \to a_H$; a stronger, better-calibrated model (mass of $c$ concentrated near
% $1$) attains the same $Y$ with smaller $e(\tau^\star)$, shifting its curve
% downward. This quantifies the framework's central claim: \emph{as agent quality
% improves, the human-oversight cost required for a fixed reliability target
% declines}.

% \subsection{Empirical instantiation on PSEBench}
% \label{sec:econ-pse}

% We instantiate the model directly from measured benchmark results, using
% PSEBench's 15-model leaderboard. PSEBench reports, per model, a verdict accuracy
% $M_1$ and an uncertain-detection $F_1$ score $M_7$ that quantifies how well the
% model recognizes the cases it should escalate. We map these to the two ingredients
% the cost model needs: $M_1$ fixes the base accuracy and $M_7$ fixes the
% \emph{calibration quality} that governs how efficiently the model can defer.

% Concretely, we draw per-case correctness $p \sim \mathrm{Beta}(\mu, \nu_0)$ with
% $\mu = M_1$ and a fixed difficulty spread $\nu_0 = 8$. A perfectly calibrated agent
% ($q=1$) escalates its lowest-$p$ cases first, recovering the optimal gate
% $R_{\mathrm{opt}}$ above; an uncalibrated agent ($q=0$) escalates at random,
% $R_{\mathrm{rand}}(e) = (1-e)\mu + a_H e$. Setting the calibration quality to the
% measured $q = M_7$ interpolates the two:
% \begin{equation}
%   R_q(e) = q\,R_{\mathrm{opt}}(e) + (1-q)\,R_{\mathrm{rand}}(e),
%   \qquad e^\star = \min\{\,e : R_q(e) \ge Y\,\}.
%   \label{eq:rq}
% \end{equation}
% Per-case token cost is computed from a shared PSEBench profile, roughly $6{,}000$ input tokens plus $4{,}000$ output tokens for reasoning models ($1{,}500$ otherwise), priced at each model's tier. Anthropic rates are list prices; OpenAI, Google, open-weight, and medical-specialty rates are representative current per-tier rates. We take the human reviewer accuracy $a_H = 0.99$ and review cost $k_h = \$25$ per escalated case ($\approx$18 minutes of a patient-safety expert).

% \begin{figure}[t]
%   \centering
%   \input{figures/cost-reliability-figure}
%   \caption{Total cost per case versus target reliability $Y$ for representative
%     PSEBench models ($a_H=0.99$, $k_h=\$25$). Cost rises convexly with the target
%     and converges to the all-human baseline as $Y \to a_H$. GPT-5.5 and GPT-5 have
%     identical token cost, yet GPT-5's collapsed uncertainty calibration
%     ($M_7=12.8$ vs.\ $79.7$) forces far more escalation and a much higher curve.}
%   \label{fig:cost}
% \end{figure}

% \begin{table}[t]
%   \centering
%   \small
%   \input{pse-results}
%   \caption{PSEBench economic results. \emph{Token \$/case} is the per-case
%     inference cost at the shared token profile; \emph{esc.}\ is the escalation rate
%     at the cost-optimal gate \eqref{eq:rq}; \emph{\$/case} is the total
%     $c_{\mathrm{unit}} = k_m + k_h\,e^\star$ at $k_h=\$25$. The all-human baseline
%     is $\$25$/case.}
%   \label{tab:pse-econ}
% \end{table}

% Three results stand out (Table~\ref{tab:pse-econ}, Figure~\ref{fig:cost}).
% \begin{enumerate}
%   \item \textbf{Token cost is a rounding error.} Per-case inference cost spans
%     only \$0.000--\$0.130 across all 15 models, at most $0.5\%$ of a \$25 human review. Per-token price is therefore not the operative economic variable, and
%     the 40$\times$ spread in token rates barely perturbs the total.
%   \item \textbf{The cost driver is escalation rate (i.e.\ accuracy and
%     calibration).} GPT-5.5 and GPT-5 have \emph{identical} token cost (\$0.048), yet
%     at $Y=98\%$ they cost \$7.45 and \$21.80 per case. The gap is entirely
%     GPT-5's collapsed uncertainty awareness ($M_7$: $12.8$ vs.\ $79.7$), which
%     forces it to escalate $87\%$ of cases rather than $30\%$. The leaderboard's
%     $M_1$ and $M_7$ columns translate directly into dollars.
%   \item \textbf{The human ceiling binds near the target.} As $Y \to a_H = 0.99$
%     every model is pushed toward escalating everything; at $Y=98\%$ only the
%     strongest few (Gemini 3.1 Pro, GPT-5.5, Claude Opus 4.7) stay materially below
%     the all-human baseline, while the rest cluster at \$22--\$24. Relaxing the target to $95\%$ opens the frontier models dramatically. Gemini 3.1 Pro, whose $95.3\%$ base accuracy already clears the bar, needs \emph{zero} escalation at \$0.05/case. That gap is the measurable price of the reliability one demands.
% \end{enumerate}

% \subsubsection{Calibration and the escalate class}

% Two error types govern the cost. \emph{Under-escalation}, a confident, incorrect verdict on a case that should have been deferred (the \textsc{Escalate} / \textsc{Uncertain} class), is a reliability failure that forces $\tau^\star$ upward and raises cost globally. \emph{Over-escalation}, deferring cases the agent would have answered correctly, is wasted human cost. Good calibration collapses both: genuinely insufficient-evidence cases receive low $c$ and route to
% a human through the same gate. Calibration error $\varepsilon$ (e.g.\ expected calibration error) acts as a safety margin: the operator must inflate the threshold to $\tau^\star + \delta(\varepsilon)$ to remain robust, and that margin carries a measurable price in additional escalation.
